Coded Caching and Spatial Multiplexing Gain Trade-off in Dynamic MISO Networks

The global caching gain of multi-antenna coded caching techniques can be also mostly achieved in dynamic network setups, where the cache contents of users are dictated by a central server, and each user can freely join or leave the network at any moment. In the dynamic setup, users are assigned to a limited set of caching profiles and the non-uniformness in the number of users assigned to each profile is compensated during the delivery phase by either adding phantom users for multicasting or serving a subset of users with unicast transmissions. In this paper, we perform a thorough analysis and provide closed-form representations of the achievable degrees of freedom (DoF) in such hybrid schemes, and assess the inherent trade-off between the global caching and spatial multiplexing gains caused by either adding phantom users or serving parts of the data through unicasting.

==> Figs/3D_Data.tex <==
DOF40	ETA40	DOF30	ETA30	DOF20	ETA20	DOF10	ETA10	DOF0	ETA0
0.666666667	0	0.666666667	0	0.666666667	0	0.666666667	0	0.666666667	0
0.666666667	0.010526316	0.666666667	0.013157895	0.666666667	0.022222222	0.666666667	0.025641026	0.666666667	0.04
0.658227848	0.021052632	0.658227848	0.026315789	0.666666667	0.044444444	0.666666667	0.051282051	0.666666667	0.08
0.6443769	0.031578947	0.656346749	0.039473684	0.670886076	0.066666667	0.670886076	0.076923077	0.670886076	0.12
0.629737609	0.042105263	0.654545455	0.052631579	0.672897196	0.088888889	0.672897196	0.102564103	0.672897196	0.16
0.611111111	0.052631579	0.647058824	0.065789474	0.676923077	0.111111111	0.676923077	0.128205128	0.676923077	0.2
0.602150538	0.063157895	0.649275362	0.078947368	0.668656716	0.133333333	0.682926829	0.153846154	0.682926829	0.24
0.592207792	0.073684211	0.642253521	0.092105263	0.662790698	0.155555556	0.688821752	0.179487179	0.688821752	0.28
0.581453634	0.084210526	0.637362637	0.105263158	0.655367232	0.177777778	0.696696697	0.205128205	0.696696697	0.32
0.571428571	0.094736842	0.631016043	0.118421053	0.650137741	0.2	0.704477612	0.230769231	0.704477612	0.36
0.558139535	0.105263158	0.615384615	0.131578947	0.631578947	0.222222222	0.705882353	0.256410256	0.705882353	0.4
0.554545455	0.115789474	0.62244898	0.144736842	0.640419948	0.244444444	0.724035608	0.282051282	0.724035608	0.44
0.547461369	0.126315789	0.618453865	0.157894737	0.635897436	0.266666667	0.725146199	0.307692308	0.733727811	0.48
0.540772532	0.136842105	0.614634146	0.171052632	0.633165829	0.288888889	0.730434783	0.333333333	0.730434783	0.52
0.533333333	0.147368421	0.612440191	0.184210526	0.628992629	0.311111111	0.711111111	0.358974359	0.711111111	0.56
0.528455285	0.157894737	0.610328638	0.197368421	0.628019324	0.333333333	0.693333333	0.384615385	0.693333333	0.6
0.522772277	0.168421053	0.608294931	0.210526316	0.625592417	0.355555556	0.676923077	0.41025641	0.676923077	0.64
0.517374517	0.178947368	0.606334842	0.223684211	0.623255814	0.377777778	0.661728395	0.435897436	0.661728395	0.68
0.512241055	0.189473684	0.600441501	0.236842105	0.622425629	0.4	0.647619048	0.461538462	0.647619048	0.72
0.508287293	0.2	0.594827586	0.25	0.621621622	0.422222222	0.634482759	0.487179487	0.634482759	0.76
0.504504505	0.210526316	0.588235294	0.263157895	0.622222222	0.444444444	0.622222222	0.512820513	0.622222222	0.8
0.5	0.221052632	0.583162218	0.276315789	0.610752688	0.466666667	0.610752688	0.538461538	0.610752688	0.84
0.496551724	0.231578947	0.578313253	0.289473684	0.6	0.488888889	0.6	0.564102564	0.6	0.88
0.493243243	0.242105263	0.57367387	0.302631579	0.58989899	0.511111111	0.58989899	0.58974359	0.58989899	0.92
0.490066225	0.252631579	0.570327553	0.315789474	0.580392157	0.533333333	0.580392157	0.615384615	0.580392157	0.96
0.48	0.263157895	0.545454545	0.328947368	0.571428571	0.555555556	0.571428571	0.641025641	1	1
0.484848485	0.273684211	0.562962963	0.342105263	0.562962963	0.577777778	0.562962963	0.666666667		
0.48200313	0.284210526	0.554954955	0.355263158	0.554954955	0.6	0.554954955	0.692307692		
0.48	0.294736842	0.547368421	0.368421053	0.547368421	0.622222222	0.547368421	0.717948718		
0.47806354	0.305263158	0.54017094	0.381578947	0.54017094	0.644444444	0.54017094	0.743589744		
0.476190476	0.315789474	0.533333333	0.394736842	0.533333333	0.666666667	0.533333333	0.769230769		
0.473684211	0.326315789	0.526829268	0.407894737	0.526829268	0.688888889	0.526829268	0.794871795		
0.472622478	0.336842105	0.520634921	0.421052632	0.520634921	0.711111111	0.520634921	0.820512821		
0.470921986	0.347368421	0.514728682	0.434210526	0.514728682	0.733333333	0.514728682	0.846153846		
0.469273743	0.357894737	0.509090909	0.447368421	0.509090909	0.755555556	0.509090909	0.871794872		
0.468319559	0.368421053	0.503703704	0.460526316	0.503703704	0.777777778	0.503703704	0.897435897		
0.466757123	0.378947368	0.498550725	0.473684211	0.498550725	0.8	0.498550725	0.923076923		
0.465863454	0.389473684	0.493617021	0.486842105	0.493617021	0.822222222	0.493617021	0.948717949		
0.464993395	0.4	0.488888889	0.5	0.488888889	0.844444444	0.488888889	0.974358974		
0.463541667	0.410526316	0.484353741	0.513157895	0.484353741	0.866666667	0.760683761	1		
0.463320463	0.421052632	0.48	0.526315789	0.48	0.888888889				
0.462515883	0.431578947	0.475816993	0.539473684	0.475816993	0.911111111				
0.461731493	0.442105263	0.471794872	0.552631579	0.471794872	0.933333333				
0.460966543	0.452631579	0.467924528	0.565789474	0.467924528	0.955555556				
0.460784314	0.463157895	0.464197531	0.578947368	0.464197531	0.977777778				
0.460606061	0.473684211	0.460606061	0.592105263	0.703703704	1				
0.457142857	0.484210526	0.457142857	0.605263158						
0.45380117	0.494736842	0.45380117	0.618421053						
0.450574713	0.505263158	0.450574713	0.631578947						
0.447457627	0.515789474	0.447457627	0.644736842						
0.444444444	0.526315789	0.444444444	0.657894737						
0.441530055	0.536842105	0.441530055	0.671052632						
0.438709677	0.547368421	0.438709677	0.684210526						
0.435978836	0.557894737	0.435978836	0.697368421						
0.433333333	0.568421053	0.433333333	0.710526316						
0.430769231	0.578947368	0.430769231	0.723684211						
0.428282828	0.589473684	0.428282828	0.736842105						
0.425870647	0.6	0.425870647	0.75						
0.423529412	0.610526316	0.423529412	0.763157895						
0.421256039	0.621052632	0.421256039	0.776315789						
0.419047619	0.631578947	0.419047619	0.789473684						
0.416901408	0.642105263	0.416901408	0.802631579						
0.414814815	0.652631579	0.414814815	0.815789474						
0.412785388	0.663157895	0.412785388	0.828947368						
0.410810811	0.673684211	0.410810811	0.842105263						
0.408888889	0.684210526	0.408888889	0.855263158						
0.407017544	0.694736842	0.407017544	0.868421053						
0.405194805	0.705263158	0.405194805	0.881578947						
0.403418803	0.715789474	0.403418803	0.894736842						
0.401687764	0.726315789	0.401687764	0.907894737						
0.4	0.736842105	0.4	0.921052632						
0.398353909	0.747368421	0.398353909	0.934210526						
0.396747967	0.757894737	0.396747967	0.947368421						
0.395180723	0.768421053	0.395180723	0.960526316						
0.393650794	0.778947368	0.393650794	0.973684211						
0.392156863	0.789473684	0.392156863	0.986842105						
0.390697674	0.8	0.552631579	1						
0.389272031	0.810526316								
0.387878788	0.821052632								
0.386516854	0.831578947								
0.385185185	0.842105263								
0.383882784	0.852631579								
0.382608696	0.863157895								
0.381362007	0.873684211								
0.380141844	0.884210526								
0.378947368	0.894736842								
0.377777778	0.905263158								
0.376632302	0.915789474								
0.375510204	0.926315789								
0.374410774	0.936842105								
0.373333333	0.947368421								
0.372277228	0.957894737								
0.37124183	0.968421053								
0.370226537	0.978947368								
0.369230769	0.989473684								
0.50877193	1								


==> Figs/DoFV_Data.tex <==
DynamicX	DynamicY	UCX	UCY	MCX	MCY	Helper	DynamicXSD	UCXSD	MCXSD
1728	0.666666667	1728	0.666666667	1728	1	2	41.56921938	41.56921938	41.56921938
1634	0.666666667	1634	0.666666667	1634	1	6	40.42276586	40.42276586	40.42276586
1544	0.666666667	1544	0.666666667	1544	1	10	39.29376541	39.29376541	39.29376541
1458	0.666666667	1458	0.666666667	1458	1	14	38.18376618	38.18376618	38.18376618
1376	0.666666667	1376	0.666666667	1376	1	18	37.09447398	37.09447398	37.09447398
1298	0.666666667	1298	0.666666667	1298	1	22	36.02776707	36.02776707	36.02776707
1224	0.666666667	1224	0.666666667	1224	1	26	34.98571137	34.98571137	34.98571137
1154	0.666666667	1154	0.666666667	1154	1	30	33.9705755	33.9705755	33.9705755
1088	0.666666667	1088	0.666666667	1088	1	34	32.984845	32.984845	32.984845
1026	0.666666667	1026	0.666666667	1026	1	38	32.03123476	32.03123476	32.03123476
968	0.666666667	968	0.666666667	968	1	42	31.11269837	31.11269837	31.11269837
914	0.666666667	914	0.666666667	914	1	46	30.23243292	30.23243292	30.23243292
840.5	0.666666667	840.5	0.666666667	840.5	1	2	28.99137803	28.99137803	28.99137803
796.5	0.666666667	796.5	0.666666667	796.5	1	6	28.22233158	28.22233158	28.22233158
756.5	0.666666667	756.5	0.666666667	756.5	1	10	27.50454508	27.50454508	27.50454508
720.5	0.666666667	720.5	0.666666667	720.5	1	14	26.84213106	26.84213106	26.84213106
688.5	0.666666667	688.5	0.666666667	688.5	1	18	26.23928353	26.23928353	26.23928353
660.5	0.666666667	660.5	0.666666667	660.5	1	22	25.70019455	25.70019455	25.70019455
636.5	0.666666667	636.5	0.666666667	636.5	1	26	25.22895162	25.22895162	25.22895162
616.5	0.666666667	616.5	0.666666667	616.5	1	30	24.82941804	24.82941804	24.82941804
600.5	0.666666667	600.5	0.666666667	600.5	1	34	24.50510151	24.50510151	24.50510151
588.5	0.666666667	588.5	0.666666667	588.5	1	38	24.25901894	24.25901894	24.25901894
580.5	0.666666667	580.5	0.666666667	580.5	1	42	24.09356761	24.09356761	24.09356761
576.5	0.666666667	576.5	0.666666667	576.5	1	46	24.01041441	24.01041441	24.01041441
1587.5	0.666666667	1587.5	0.666666667	1587.5	1	2	39.84344363	39.84344363	39.84344363
1498.5	0.666666667	1498.5	0.666666667	1498.5	1	6	38.7104637	38.7104637	38.7104637
1413.5	0.666666667	1413.5	0.666666667	1413.5	1	10	37.59654239	37.59654239	37.59654239
1332.5	0.666666667	1332.5	0.666666667	1332.5	1	14	36.5034245	36.5034245	36.5034245
1255.5	0.666666667	1255.5	0.666666667	1255.5	1	18	35.43303543	35.43303543	35.43303543
1182.5	0.666666667	1182.5	0.666666667	1182.5	1	22	34.38749773	34.38749773	34.38749773
1113.5	0.666666667	1113.5	0.666666667	1113.5	1	26	33.36914743	33.36914743	33.36914743
1048.5	0.666666667	1048.5	0.666666667	1048.5	1	30	32.38054972	32.38054972	32.38054972
987.5	0.666666667	987.5	0.666666667	987.5	1	34	31.42451272	31.42451272	31.42451272
930.5	0.666666667	930.5	0.666666667	930.5	1	38	30.50409809	30.50409809	30.50409809
877.5	0.666666667	877.5	0.666666667	877.5	1	42	29.62262649	29.62262649	29.62262649
828.5	0.666666667	828.5	0.666666667	828.5	1	46	28.78367593	28.78367593	28.78367593
762.5	0.666666667	762.5	0.666666667	762.5	1	2	27.61340254	27.61340254	27.61340254
723.5	0.666666667	723.5	0.666666667	723.5	1	6	26.89795531	26.89795531	26.89795531
688.5	0.666666667	688.5	0.666666667	688.5	1	10	26.23928353	26.23928353	26.23928353
657.5	0.666666667	657.5	0.666666667	657.5	1	14	25.64176281	25.64176281	25.64176281
630.5	0.666666667	630.5	0.666666667	630.5	1	18	25.10975906	25.10975906	25.10975906
607.5	0.666666667	607.5	0.666666667	607.5	1	22	24.64751509	24.64751509	24.64751509
588.5	0.666666667	588.5	0.666666667	588.5	1	26	24.25901894	24.25901894	24.25901894
573.5	0.666666667	573.5	0.666666667	573.5	1	30	23.94786003	23.94786003	23.94786003
562.5	0.666666667	562.5	0.666666667	562.5	1	34	23.71708245	23.71708245	23.71708245
555.5	0.666666667	555.5	0.666666667	555.5	1	38	23.5690475	23.5690475	23.5690475
553.5	0.666666667	553.5	0.666666667	553.5	1	42	23.52658071	23.52658071	23.52658071
1497.5	0.666666667	1497.5	0.666666667	1497.5	1	46	38.69754514	38.69754514	38.69754514
1370	0.666666667	1370	0.666666667	1370	1	2	37.01351105	37.01351105	37.01351105
1290	0.666666667	1290	0.666666667	1290	1	6	35.91656999	35.91656999	35.91656999
1214	0.666666667	1214	0.666666667	1214	1	10	34.84250278	34.84250278	34.84250278
1142	0.666666667	1142	0.666666667	1142	1	14	33.7934905	33.7934905	33.7934905
1074	0.666666667	1074	0.666666667	1074	1	18	32.77193922	32.77193922	32.77193922
1010	0.666666667	1010	0.666666667	1010	1	22	31.78049716	31.78049716	31.78049716
950	0.666666667	950	0.666666667	950	1	26	30.82207001	30.82207001	30.82207001
894	0.666666667	894	0.666666667	894	1	30	29.89983278	29.89983278	29.89983278
842	0.666666667	842	0.666666667	842	1	34	29.01723626	29.01723626	29.01723626
794	0.666666667	794	0.666666667	794	1	38	28.17800561	28.17800561	28.17800561
750	0.666666667	750	0.666666667	750	1	42	27.38612788	27.38612788	27.38612788
710	0.666666667	710	0.666666667	710	1	46	26.64582519	26.64582519	26.64582519
657.5	0.666666667	657.5	0.666666667	657.5	1	2	25.64176281	25.64176281	25.64176281
627.5	0.666666667	627.5	0.666666667	627.5	1	6	25.0499501	25.0499501	25.0499501
601.5	0.666666667	601.5	0.666666667	601.5	1	10	24.52549694	24.52549694	24.52549694
579.5	0.666666667	579.5	0.666666667	579.5	1	14	24.07280623	24.07280623	24.07280623
561.5	0.666666667	561.5	0.666666667	561.5	1	18	23.69599122	23.69599122	23.69599122
547.5	0.666666667	547.5	0.666666667	547.5	1	22	23.39871791	23.39871791	23.39871791
537.5	0.666666667	537.5	0.666666667	537.5	1	26	23.18404624	23.18404624	23.18404624
531.5	0.666666667	531.5	0.666666667	531.5	1	30	23.05428377	23.05428377	23.05428377
529.5	0.680555556	529.5	0.666666667	529.5	1	34	23.010867	23.010867	23.010867
1410.5	0.666666667	1410.5	0.666666667	1410.5	1	38	37.55662392	37.55662392	37.55662392
1327.5	0.666666667	1327.5	0.666666667	1327.5	1	42	36.4348734	36.4348734	36.4348734
1248.5	0.666666667	1248.5	0.666666667	1248.5	1	46	35.33411949	35.33411949	35.33411949
1137.5	0.666666667	1137.5	0.666666667	1137.5	1	2	33.72684391	33.72684391	33.72684391
1068.5	0.666666667	1068.5	0.666666667	1068.5	1	6	32.68791826	32.68791826	32.68791826
1003.5	0.666666667	1003.5	0.666666667	1003.5	1	10	31.67806812	31.67806812	31.67806812
942.5	0.666666667	942.5	0.666666667	942.5	1	14	30.70016287	30.70016287	30.70016287
885.5	0.666666667	885.5	0.666666667	885.5	1	18	29.75735203	29.75735203	29.75735203
832.5	0.666666667	832.5	0.666666667	832.5	1	22	28.85307609	28.85307609	28.85307609
783.5	0.666666667	783.5	0.666666667	783.5	1	26	27.99107	27.99107	27.99107
738.5	0.666666667	738.5	0.666666667	738.5	1	30	27.17535648	27.17535648	27.17535648
697.5	0.666666667	697.5	0.666666667	697.5	1	34	26.41022529	26.41022529	26.41022529
660.5	0.666666667	660.5	0.666666667	660.5	1	38	25.70019455	25.70019455	25.70019455
627.5	0.666666667	627.5	0.666666667	627.5	1	42	25.0499501	25.0499501	25.0499501
598.5	0.666666667	598.5	0.666666667	598.5	1	46	24.46425965	24.46425965	24.46425965
562.5	0.666666667	562.5	0.666666667	562.5	1	2	23.71708245	23.71708245	23.71708245
543.5	0.666666667	543.5	0.666666667	543.5	1	6	23.31308645	23.31308645	23.31308645
528.5	0.666666667	528.5	0.666666667	528.5	1	10	22.98912787	22.98912787	22.98912787
517.5	0.666666667	517.5	0.666666667	517.5	1	14	22.74862633	22.74862633	22.74862633
510.5	0.666666667	510.5	0.666666667	510.5	1	18	22.59424706	22.59424706	22.59424706
1368	0.666666667	1368	0.666666667	1368	1	22	36.98648402	36.98648402	36.98648402
1286	0.666666667	1286	0.666666667	1286	1	26	35.86084215	35.86084215	35.86084215
1208	0.666666667	1208	0.666666667	1208	1	30	34.75629439	34.75629439	34.75629439
1134	0.666666667	1134	0.666666667	1134	1	34	33.67491648	33.67491648	33.67491648
1064	0.666666667	1064	0.666666667	1064	1	38	32.61901286	32.61901286	32.61901286
998	0.666666667	998	0.666666667	998	1	42	31.591138	31.591138	31.591138
936	0.666666667	936	0.666666667	936	1	46	30.59411708	30.59411708	30.59411708
850.5	0.666666667	850.5	0.666666667	850.5	1	2	29.16333314	29.16333314	29.16333314
798.5	0.666666667	798.5	0.666666667	798.5	1	6	28.2577423	28.2577423	28.2577423
750.5	0.666666667	750.5	0.666666667	750.5	1	10	27.39525506	27.39525506	27.39525506
706.5	0.666666667	706.5	0.666666667	706.5	1	14	26.58006772	26.58006772	26.58006772
666.5	0.666666667	666.5	0.666666667	666.5	1	18	25.81666129	25.81666129	25.81666129
630.5	0.666666667	630.5	0.666666667	630.5	1	22	25.10975906	25.10975906	25.10975906
598.5	0.666666667	598.5	0.666666667	598.5	1	26	24.46425965	24.46425965	24.46425965
570.5	0.666666667	570.5	0.666666667	570.5	1	30	23.88514182	23.88514182	23.88514182
546.5	0.666666667	546.5	0.666666667	546.5	1	34	23.37733946	23.37733946	23.37733946
526.5	0.666666667	526.5	0.666666667	526.5	1	38	22.94558781	22.94558781	22.94558781
510.5	0.666666667	510.5	0.666666667	510.5	1	42	22.59424706	22.59424706	22.59424706
498.5	0.666666667	498.5	0.666666667	498.5	1	46	22.32711356	22.32711356	22.32711356
490.5	0.666666667	490.5	0.666666667	490.5	1	2	22.14723459	22.14723459	22.14723459
1285.5	0.666666667	1285.5	0.666666667	1285.5	1	6	35.85387008	35.85387008	35.85387008
1206.5	0.666666667	1206.5	0.666666667	1206.5	1	10	34.73470887	34.73470887	34.73470887
1131.5	0.666666667	1131.5	0.666666667	1131.5	1	14	33.63777638	33.63777638	33.63777638
1060.5	0.666666667	1060.5	0.666666667	1060.5	1	18	32.56531898	32.56531898	32.56531898
993.5	0.666666667	993.5	0.666666667	993.5	1	22	31.51983502	31.51983502	31.51983502
930.5	0.666666667	930.5	0.666666667	930.5	1	26	30.50409809	30.50409809	30.50409809
871.5	0.666666667	871.5	0.666666667	871.5	1	30	29.52117884	29.52117884	29.52117884
816.5	0.666666667	816.5	0.666666667	816.5	1	34	28.57446412	28.57446412	28.57446412
765.5	0.666666667	765.5	0.666666667	765.5	1	38	27.66767066	27.66767066	27.66767066
718.5	0.666666667	718.5	0.666666667	718.5	1	42	26.80485031	26.80485031	26.80485031
675.5	0.666666667	675.5	0.666666667	675.5	1	46	25.99038284	25.99038284	25.99038284
618.5	0.666666667	618.5	0.666666667	618.5	1	2	24.86966023	24.86966023	24.86966023
585.5	0.666666667	585.5	0.666666667	585.5	1	6	24.19710727	24.19710727	24.19710727
556.5	0.666666667	556.5	0.666666667	556.5	1	10	23.59025222	23.59025222	23.59025222
531.5	0.666666667	531.5	0.666666667	531.5	1	14	23.05428377	23.05428377	23.05428377
510.5	0.666666667	510.5	0.666666667	510.5	1	18	22.59424706	22.59424706	22.59424706
493.5	0.666666667	493.5	0.666666667	493.5	1	22	22.21485989	22.21485989	22.21485989
480.5	0.666666667	480.5	0.666666667	480.5	1	26	21.92031022	21.92031022	21.92031022
471.5	0.666666667	471.5	0.666666667	471.5	1	30	21.71405075	21.71405075	21.71405075
466.5	0.680555556	466.5	0.666666667	466.5	1	34	21.59861107	21.59861107	21.59861107
1167.5	0.666666667	1167.5	0.666666667	1167.5	1	38	34.16869913	34.16869913	34.16869913
1093.5	0.666666667	1093.5	0.666666667	1093.5	1	42	33.06811153	33.06811153	33.06811153
1023.5	0.666666667	1023.5	0.666666667	1023.5	1	46	31.99218655	31.99218655	31.99218655
926	0.666666667	926	0.666666667	926	1	2	30.43024811	30.43024811	30.43024811
866	0.666666667	866	0.666666667	866	1	6	29.42787794	29.42787794	29.42787794
810	0.666666667	810	0.666666667	810	1	10	28.46049894	28.46049894	28.46049894
758	0.666666667	758	0.666666667	758	1	14	27.5317998	27.5317998	27.5317998
710	0.666666667	710	0.666666667	710	1	18	26.64582519	26.64582519	26.64582519
666	0.666666667	666	0.666666667	666	1	22	25.8069758	25.8069758	25.8069758
626	0.666666667	626	0.666666667	626	1	26	25.01999201	25.01999201	25.01999201
590	0.666666667	590	0.666666667	590	1	30	24.2899156	24.2899156	24.2899156
558	0.666666667	558	0.666666667	558	1	34	23.62202362	23.62202362	23.62202362
530	0.666666667	530	0.666666667	530	1	38	23.02172887	23.02172887	23.02172887
506	0.666666667	506	0.666666667	506	1	42	22.49444376	22.49444376	22.49444376
486	0.666666667	486	0.666666667	486	1	46	22.04540769	22.04540769	22.04540769
463.5	0.666666667	463.5	0.666666667	463.5	1	2	21.52905014	21.52905014	21.52905014
453.5	0.666666667	453.5	0.666666667	453.5	1	6	21.29553944	21.29553944	21.29553944
447.5	0.680555556	447.5	0.666666667	447.5	1	10	21.1541958	21.1541958	21.1541958
1129.5	0.666666667	1129.5	0.666666667	1129.5	1	14	33.60803475	33.60803475	33.60803475
1056.5	0.666666667	1056.5	0.666666667	1056.5	1	18	32.50384593	32.50384593	32.50384593
987.5	0.666666667	987.5	0.666666667	987.5	1	22	31.42451272	31.42451272	31.42451272
922.5	0.666666667	922.5	0.666666667	922.5	1	26	30.3726851	30.3726851	30.3726851
861.5	0.666666667	861.5	0.666666667	861.5	1	30	29.35132024	29.35132024	29.35132024
804.5	0.666666667	804.5	0.666666667	804.5	1	34	28.36370921	28.36370921	28.36370921
751.5	0.666666667	751.5	0.666666667	751.5	1	38	27.41350032	27.41350032	27.41350032
702.5	0.666666667	702.5	0.666666667	702.5	1	42	26.50471656	26.50471656	26.50471656
657.5	0.666666667	657.5	0.666666667	657.5	1	46	25.64176281	25.64176281	25.64176281
597.5	0.666666667	597.5	0.666666667	597.5	1	2	24.44381312	24.44381312	24.44381312
562.5	0.666666667	562.5	0.666666667	562.5	1	6	23.71708245	23.71708245	23.71708245
531.5	0.666666667	531.5	0.666666667	531.5	1	10	23.05428377	23.05428377	23.05428377
504.5	0.666666667	504.5	0.666666667	504.5	1	14	22.46107745	22.46107745	22.46107745
481.5	0.666666667	481.5	0.666666667	481.5	1	18	21.94310826	21.94310826	21.94310826
462.5	0.666666667	462.5	0.666666667	462.5	1	22	21.50581317	21.50581317	21.50581317
447.5	0.666666667	447.5	0.666666667	447.5	1	26	21.1541958	21.1541958	21.1541958
436.5	0.666666667	436.5	0.666666667	436.5	1	30	20.89258242	20.89258242	20.89258242
427.5	0.687943262	427.5	0.666666667	427.5	1	34	20.67607313	20.67607313	20.67607313
1020.5	0.666666667	1020.5	0.666666667	1020.5	1	38	31.94526569	31.94526569	31.94526569
952.5	0.666666667	952.5	0.666666667	952.5	1	42	30.86259872	30.86259872	30.86259872
888.5	0.666666667	888.5	0.666666667	888.5	1	46	29.80771712	29.80771712	29.80771712
800	0.666666667	800	0.666666667	800	1	2	28.28427125	28.28427125	28.28427125
746	0.666666667	746	0.666666667	746	1	6	27.31300057	27.31300057	27.31300057
696	0.666666667	696	0.666666667	696	1	10	26.38181192	26.38181192	26.38181192
650	0.666666667	650	0.666666667	650	1	14	25.49509757	25.49509757	25.49509757
608	0.666666667	608	0.666666667	608	1	18	24.65765601	24.65765601	24.65765601
570	0.666666667	570	0.666666667	570	1	22	23.87467277	23.87467277	23.87467277
536	0.666666667	536	0.666666667	536	1	26	23.15167381	23.15167381	23.15167381
506	0.666666667	506	0.666666667	506	1	30	22.49444376	22.49444376	22.49444376
480	0.666666667	480	0.666666667	480	1	34	21.9089023	21.9089023	21.9089023
458	0.666666667	458	0.666666667	458	1	38	21.40093456	21.40093456	21.40093456
440	0.666666667	440	0.666666667	440	1	42	20.97617696	20.97617696	20.97617696
426	0.666666667	426	0.666666667	426	1	46	20.63976744	20.63976744	20.63976744
412.5	0.680555556	412.5	0.666666667	412.5	1	2	20.31009601	20.31009601	20.31009601
985.5	0.666666667	985.5	0.666666667	985.5	1	6	31.3926743	31.3926743	31.3926743
918.5	0.666666667	918.5	0.666666667	918.5	1	10	30.30676492	30.30676492	30.30676492
855.5	0.666666667	855.5	0.666666667	855.5	1	14	29.2489316	29.2489316	29.2489316
796.5	0.666666667	796.5	0.666666667	796.5	1	18	28.22233158	28.22233158	28.22233158
741.5	0.666666667	741.5	0.666666667	741.5	1	22	27.23049761	27.23049761	27.23049761
690.5	0.666666667	690.5	0.666666667	690.5	1	26	26.27736669	26.27736669	26.27736669
643.5	0.666666667	643.5	0.666666667	643.5	1	30	25.36730179	25.36730179	25.36730179
600.5	0.666666667	600.5	0.666666667	600.5	1	34	24.50510151	24.50510151	24.50510151
561.5	0.666666667	561.5	0.666666667	561.5	1	38	23.69599122	23.69599122	23.69599122
526.5	0.666666667	526.5	0.666666667	526.5	1	42	22.94558781	22.94558781	22.94558781
495.5	0.666666667	495.5	0.666666667	495.5	1	46	22.25982929	22.25982929	22.25982929
456.5	0.666666667	456.5	0.666666667	456.5	1	2	21.36586062	21.36586062	21.36586062
435.5	0.666666667	435.5	0.666666667	435.5	1	6	20.86863675	20.86863675	20.86863675
418.5	0.666666667	418.5	0.666666667	418.5	1	10	20.45727255	20.45727255	20.45727255
405.5	0.666666667	405.5	0.666666667	405.5	1	14	20.13703057	20.13703057	20.13703057
396.5	0.680555556	396.5	0.666666667	396.5	1	18	19.91230775	19.91230775	19.91230775
918	0.666666667	918	0.666666667	918	1	22	30.29851482	30.29851482	30.29851482
854	0.666666667	854	0.666666667	854	1	26	29.22327839	29.22327839	29.22327839
794	0.666666667	794	0.666666667	794	1	30	28.17800561	28.17800561	28.17800561
738	0.666666667	738	0.666666667	738	1	34	27.16615541	27.16615541	27.16615541
686	0.666666667	686	0.666666667	686	1	38	26.19160171	26.19160171	26.19160171
638	0.666666667	638	0.666666667	638	1	42	25.25866188	25.25866188	25.25866188
594	0.666666667	594	0.666666667	594	1	46	24.37211521	24.37211521	24.37211521
535.5	0.666666667	535.5	0.666666667	535.5	1	2	23.14087293	23.14087293	23.14087293
501.5	0.666666667	501.5	0.666666667	501.5	1	6	22.39419568	22.39419568	22.39419568
471.5	0.666666667	471.5	0.666666667	471.5	1	10	21.71405075	21.71405075	21.71405075
445.5	0.666666667	445.5	0.666666667	445.5	1	14	21.10687092	21.10687092	21.10687092
423.5	0.666666667	423.5	0.666666667	423.5	1	18	20.57911563	20.57911563	20.57911563
405.5	0.666666667	405.5	0.666666667	405.5	1	22	20.13703057	20.13703057	20.13703057
391.5	0.666666667	391.5	0.666666667	391.5	1	26	19.78635894	19.78635894	19.78635894
381.5	0.680555556	381.5	0.666666667	381.5	1	30	19.53202498	19.53202498	19.53202498
373.5	0.712121212	373.5	0.666666667	373.5	1	34	19.32614809	19.32614809	19.32614809
822.5	0.666666667	822.5	0.666666667	822.5	1	38	28.6792608	28.6792608	28.6792608
763.5	0.666666667	763.5	0.666666667	763.5	1	42	27.63150376	27.63150376	27.63150376
708.5	0.666666667	708.5	0.666666667	708.5	1	46	26.61766331	26.61766331	26.61766331
633.5	0.666666667	633.5	0.666666667	633.5	1	2	25.1694259	25.1694259	25.1694259
588.5	0.666666667	588.5	0.666666667	588.5	1	6	24.25901894	24.25901894	24.25901894
547.5	0.666666667	547.5	0.666666667	547.5	1	10	23.39871791	23.39871791	23.39871791
510.5	0.666666667	510.5	0.666666667	510.5	1	14	22.59424706	22.59424706	22.59424706
477.5	0.666666667	477.5	0.666666667	477.5	1	18	21.85177338	21.85177338	21.85177338
448.5	0.666666667	448.5	0.666666667	448.5	1	22	21.17781858	21.17781858	21.17781858
423.5	0.666666667	423.5	0.666666667	423.5	1	26	20.57911563	20.57911563	20.57911563
402.5	0.666666667	402.5	0.666666667	402.5	1	30	20.06240265	20.06240265	20.06240265
385.5	0.666666667	385.5	0.666666667	385.5	1	34	19.63415392	19.63415392	19.63415392
372.5	0.673469388	372.5	0.666666667	372.5	1	38	19.30025907	19.30025907	19.30025907
358.5	0.703703704	358.5	0.666666667	358.5	1	42	18.93409623	18.93409623	18.93409623
762.5	0.666666667	762.5	0.666666667	762.5	1	46	27.61340254	27.61340254	27.61340254
680	0.666666667	680	0.666666667	680	1	2	26.07680962	26.07680962	26.07680962
630	0.666666667	630	0.666666667	630	1	6	25.0998008	25.0998008	25.0998008
584	0.666666667	584	0.666666667	584	1	10	24.16609195	24.16609195	24.16609195
542	0.666666667	542	0.666666667	542	1	14	23.28089345	23.28089345	23.28089345
504	0.666666667	504	0.666666667	504	1	18	22.44994432	22.44994432	22.44994432
470	0.666666667	470	0.666666667	470	1	22	21.67948339	21.67948339	21.67948339
440	0.666666667	440	0.666666667	440	1	26	20.97617696	20.97617696	20.97617696
414	0.666666667	414	0.666666667	414	1	30	20.34698995	20.34698995	20.34698995
392	0.666666667	392	0.666666667	392	1	34	19.79898987	19.79898987	19.79898987
374	0.666666667	374	0.666666667	374	1	38	19.33907961	19.33907961	19.33907961
366.5	0.666666667	366.5	0.666666667	366.5	1	42	19.14418972	19.14418972	19.14418972
346.5	0.695652174	346.5	0.666666667	346.5	1	46	18.61451047	18.61451047	18.61451047
705.5	0.666666667	705.5	0.666666667	705.5	1	2	26.56124997	26.56124997	26.56124997
652.5	0.666666667	652.5	0.666666667	652.5	1	6	25.54407955	25.54407955	25.54407955
603.5	0.666666667	603.5	0.666666667	603.5	1	10	24.56623699	24.56623699	24.56623699
558.5	0.666666667	558.5	0.666666667	558.5	1	14	23.6326046	23.6326046	23.6326046
517.5	0.666666667	517.5	0.666666667	517.5	1	18	22.74862633	22.74862633	22.74862633
480.5	0.666666667	480.5	0.666666667	480.5	1	22	21.92031022	21.92031022	21.92031022
447.5	0.666666667	447.5	0.666666667	447.5	1	26	21.1541958	21.1541958	21.1541958
418.5	0.666666667	418.5	0.666666667	418.5	1	30	20.45727255	20.45727255	20.45727255
393.5	0.666666667	393.5	0.666666667	393.5	1	34	19.83683442	19.83683442	19.83683442
372.5	0.666666667	372.5	0.666666667	372.5	1	38	19.30025907	19.30025907	19.30025907
355.5	0.666666667	355.5	0.666666667	355.5	1	42	18.85470763	18.85470763	18.85470763
342.5	0.680555556	342.5	0.666666667	342.5	1	46	18.50675552	18.50675552	18.50675552
678	0.666666667	678	0.666666667	678	1	2	26.03843313	26.03843313	26.03843313
626	0.666666667	626	0.666666667	626	1	6	25.01999201	25.01999201	25.01999201
578	0.666666667	578	0.666666667	578	1	10	24.04163056	24.04163056	24.04163056
534	0.666666667	534	0.666666667	534	1	14	23.10844002	23.10844002	23.10844002
494	0.666666667	494	0.666666667	494	1	18	22.22611077	22.22611077	22.22611077
458	0.666666667	458	0.666666667	458	1	22	21.40093456	21.40093456	21.40093456
426	0.666666667	426	0.666666667	426	1	26	20.63976744	20.63976744	20.63976744
398	0.666666667	398	0.666666667	398	1	30	19.94993734	19.94993734	19.94993734
374	0.666666667	374	0.666666667	374	1	34	19.33907961	19.33907961	19.33907961
354	0.666666667	354	0.666666667	354	1	38	18.81488772	18.81488772	18.81488772
345.5	0.666666667	345.5	0.666666667	345.5	1	42	18.5876303	18.5876303	18.5876303
321.5	0.695652174	321.5	0.666666667	321.5	1	46	17.93042108	17.93042108	17.93042108
600.5	0.670050761	600.5	0.666666667	600.5	1	2	24.50510151	24.50510151	24.50510151
510.5	0.670050761	510.5	0.666666667	510.5	1	6	22.59424706	22.59424706	22.59424706
436.5	0.670050761	436.5	0.666666667	436.5	1	10	20.89258242	20.89258242	20.89258242
378.5	0.670050761	378.5	0.666666667	378.5	1	14	19.45507646	19.45507646	19.45507646
336.5	0.670050761	336.5	0.666666667	336.5	1	18	18.34393633	18.34393633	18.34393633
310.5	0.695652174	310.5	0.666666667	310.5	1	22	17.62101019	17.62101019	17.62101019
300.5	0.73015873	300.5	0.666666667	300.5	1	26	17.33493582	17.33493582	17.33493582
508.5	0.670050761	508.5	0.666666667	508.5	1	30	22.54994457	22.54994457	22.54994457
432.5	0.670050761	432.5	0.666666667	432.5	1	34	20.79663434	20.79663434	20.79663434
372.5	0.670050761	372.5	0.666666667	372.5	1	38	19.30025907	19.30025907	19.30025907
328.5	0.670050761	328.5	0.666666667	328.5	1	42	18.12456896	18.12456896	18.12456896
300.5	0.695652174	300.5	0.666666667	300.5	1	46	17.33493582	17.33493582	17.33493582
529.5	0.670050761	529.5	0.666666667	529.5	1	2	23.010867	23.010867	23.010867
447.5	0.670050761	447.5	0.666666667	447.5	1	6	21.1541958	21.1541958	21.1541958
381.5	0.670050761	381.5	0.666666667	381.5	1	10	19.53202498	19.53202498	19.53202498
331.5	0.670050761	331.5	0.666666667	331.5	1	14	18.20714146	18.20714146	18.20714146
297.5	0.687943262	297.5	0.666666667	297.5	1	18	17.24818831	17.24818831	17.24818831
279.5	0.720930233	279.5	0.666666667	279.5	1	22	16.7182535	16.7182535	16.7182535
465.5	0.670050761	465.5	0.666666667	465.5	1	26	21.57544901	21.57544901	21.57544901
393.5	0.670050761	393.5	0.666666667	393.5	1	30	19.83683442	19.83683442	19.83683442
337.5	0.670050761	337.5	0.666666667	337.5	1	34	18.37117307	18.37117307	18.37117307
297.5	0.680555556	297.5	0.666666667	297.5	1	38	17.24818831	17.24818831	17.24818831
273.5	0.712121212	273.5	0.666666667	273.5	1	42	16.53783541	16.53783541	16.53783541
265.5	0.75	265.5	0.666666667	265.5	1	46	16.29417074	16.29417074	16.29417074
360.5	0.670050761	360.5	0.666666667	360.5	1	2	18.98683755	18.98683755	18.98683755
310.5	0.670050761	310.5	0.666666667	310.5	1	6	17.62101019	17.62101019	17.62101019
276.5	0.695652174	276.5	0.666666667	276.5	1	10	16.62828915	16.62828915	16.62828915
258.5	0.73015873	258.5	0.666666667	258.5	1	14	16.07793519	16.07793519	16.07793519
390.5	0.670050761	390.5	0.666666667	390.5	1	18	19.76107285	19.76107285	19.76107285
330.5	0.670050761	330.5	0.666666667	330.5	1	22	18.17965896	18.17965896	18.17965896
286.5	0.680555556	286.5	0.666666667	286.5	1	26	16.92631088	16.92631088	16.92631088
258.5	0.712121212	258.5	0.666666667	258.5	1	30	16.07793519	16.07793519	16.07793519
246.5	0.75	246.5	0.666666667	246.5	1	34	15.70031847	15.70031847	15.70031847
342.5	0.670050761	342.5	0.666666667	342.5	1	38	18.50675552	18.50675552	18.50675552
292.5	0.673469388	292.5	0.666666667	292.5	1	42	17.10263138	17.10263138	17.10263138
258.5	0.703703704	258.5	0.666666667	258.5	1	46	16.07793519	16.07793519	16.07793519
237.5	0.760683761	237.5	0.666666667	237.5	1	2	15.41103501	15.41103501	15.41103501
301.5	0.670050761	301.5	0.666666667	301.5	1	6	17.36375535	17.36375535	17.36375535
261.5	0.695652174	261.5	0.666666667	261.5	1	10	16.17096163	16.17096163	16.17096163
237.5	0.73015873	237.5	0.666666667	237.5	1	14	15.41103501	15.41103501	15.41103501
229.5	0.771929825	229.5	0.666666667	229.5	1	18	15.14925741	15.14925741	15.14925741
277.5	0.680555556	277.5	0.666666667	277.5	1	22	16.65833125	16.65833125	16.65833125
243.5	0.712121212	243.5	0.666666667	243.5	1	26	15.60448653	15.60448653	15.60448653
225.5	0.75	225.5	0.666666667	225.5	1	30	15.01665742	15.01665742	15.01665742
276.5	0.680555556	276.5	0.666666667	276.5	1	34	16.62828915	16.62828915	16.62828915
240.5	0.712121212	240.5	0.666666667	240.5	1	38	15.50806242	15.50806242	15.50806242
220.5	0.75	220.5	0.666666667	220.5	1	42	14.8492424	14.8492424	14.8492424
265.5	0.687943262	265.5	0.666666667	265.5	1	46	16.29417074	16.29417074	16.29417074
220.5	0.739837398	220.5	0.666666667	220.5	1	2	14.8492424	14.8492424	14.8492424
210.5	0.783783784	210.5	0.666666667	210.5	1	6	14.50861813	14.50861813	14.50861813
223.5	0.73015873	223.5	0.666666667	223.5	1	10	14.94991639	14.94991639	14.94991639
207.5	0.771929825	207.5	0.666666667	207.5	1	14	14.40486029	14.40486029	14.40486029
222.5	0.73015873	222.5	0.666666667	222.5	1	18	14.91643389	14.91643389	14.91643389
204.5	0.771929825	204.5	0.666666667	204.5	1	22	14.30034965	14.30034965	14.30034965
210.5	0.75	210.5	0.666666667	210.5	1	26	14.50861813	14.50861813	14.50861813
198.5	0.796296296	198.5	0.666666667	198.5	1	30	14.0890028	14.0890028	14.0890028
198.5	0.783783784	198.5	0.666666667	198.5	1	34	14.0890028	14.0890028	14.0890028
195.5	0.796296296	195.5	0.666666667	195.5	1	38	13.98213145	13.98213145	13.98213145
192.5	0.823529412	192.5	0.666666667	192.5	1	42	13.87443693	13.87443693	13.87443693
1587	0.666666667	1587	0.666666667	1587	1	46	39.83716857	39.83716857	39.83716857
1497	0.666666667	1497	0.666666667	1497	1	2	38.69108424	38.69108424	38.69108424
1411	0.666666667	1411	0.666666667	1411	1	6	37.56327994	37.56327994	37.56327994
1369.5	0.666666667	1369.5	0.666666667	1369.5	1	10	37.00675614	37.00675614	37.00675614
1329	0.666666667	1329	0.666666667	1329	1	14	36.45545227	36.45545227	36.45545227
1251	0.666666667	1251	0.666666667	1251	1	18	35.36947837	35.36947837	35.36947837
1213.5	0.666666667	1213.5	0.666666667	1213.5	1	22	34.8353269	34.8353269	34.8353269
1177	0.666666667	1177	0.666666667	1177	1	26	34.3074336	34.3074336	34.3074336
1107	0.666666667	1107	0.666666667	1107	1	30	33.27160952	33.27160952	33.27160952
1073.5	0.666666667	1073.5	0.666666667	1073.5	1	34	32.76430985	32.76430985	32.76430985
1041	0.666666667	1041	0.666666667	1041	1	38	32.26453161	32.26453161	32.26453161
979	0.666666667	979	0.666666667	979	1	42	31.28897569	31.28897569	31.28897569
949.5	0.666666667	949.5	0.666666667	949.5	1	46	30.81395788	30.81395788	30.81395788
893.5	0.666666667	893.5	0.666666667	893.5	1	2	29.89147036	29.89147036	29.89147036
867	0.666666667	867	0.666666667	867	1	6	29.44486373	29.44486373	29.44486373
817	0.666666667	817	0.666666667	817	1	10	28.58321186	28.58321186	28.58321186
793.5	0.666666667	793.5	0.666666667	793.5	1	14	28.16913204	28.16913204	28.16913204
771	0.666666667	771	0.666666667	771	1	18	27.76688675	27.76688675	27.76688675
729	0.666666667	729	0.666666667	729	1	22	27	27	27
709.5	0.666666667	709.5	0.666666667	709.5	1	26	26.6364412	26.6364412	26.6364412
691	0.666666667	691	0.666666667	691	1	30	26.28687886	26.28687886	26.28687886
657	0.666666667	657	0.666666667	657	1	34	25.63201124	25.63201124	25.63201124
641.5	0.666666667	641.5	0.666666667	641.5	1	38	25.32785028	25.32785028	25.32785028
627	0.666666667	627	0.666666667	627	1	42	25.03996805	25.03996805	25.03996805
601	0.666666667	601	0.666666667	601	1	46	24.51530134	24.51530134	24.51530134
579	0.666666667	579	0.666666667	579	1	2	24.06241883	24.06241883	24.06241883
569.5	0.666666667	569.5	0.666666667	569.5	1	6	23.86419913	23.86419913	23.86419913
561	0.666666667	561	0.666666667	561	1	10	23.68543856	23.68543856	23.68543856
547	0.666666667	547	0.666666667	547	1	14	23.38803113	23.38803113	23.38803113
541.5	0.666666667	541.5	0.666666667	541.5	1	18	23.27015256	23.27015256	23.27015256
537	0.666666667	537	0.666666667	537	1	22	23.17326045	23.17326045	23.17326045
531	0.666666667	531	0.666666667	531	1	26	23.04343724	23.04343724	23.04343724
529.5	0.673469388	529.5	0.666666667	529.5	1	30	23.010867	23.010867	23.010867
1496.5	0.666666667	1496.5	0.666666667	1496.5	1	34	38.68462227	38.68462227	38.68462227
1409.5	0.666666667	1409.5	0.666666667	1409.5	1	38	37.54330833	37.54330833	37.54330833
1367.5	0.666666667	1367.5	0.666666667	1367.5	1	42	36.97972417	36.97972417	36.97972417
1326.5	0.666666667	1326.5	0.666666667	1326.5	1	46	36.4211477	36.4211477	36.4211477
1247.5	0.666666667	1247.5	0.666666667	1247.5	1	2	35.31996602	35.31996602	35.31996602
1172.5	0.666666667	1172.5	0.666666667	1172.5	1	6	34.24178734	34.24178734	34.24178734
1136.5	0.666666667	1136.5	0.666666667	1136.5	1	10	33.71201566	33.71201566	33.71201566
1101.5	0.666666667	1101.5	0.666666667	1101.5	1	14	33.18885355	33.18885355	33.18885355
1034.5	0.666666667	1034.5	0.666666667	1034.5	1	18	32.16364407	32.16364407	32.16364407
1002.5	0.666666667	1002.5	0.666666667	1002.5	1	22	31.6622804	31.6622804	31.6622804
971.5	0.666666667	971.5	0.666666667	971.5	1	26	31.16889475	31.16889475	31.16889475
912.5	0.666666667	912.5	0.666666667	912.5	1	30	30.20761493	30.20761493	30.20761493
884.5	0.666666667	884.5	0.666666667	884.5	1	34	29.74054472	29.74054472	29.74054472
857.5	0.666666667	857.5	0.666666667	857.5	1	38	29.28310093	29.28310093	29.28310093
806.5	0.666666667	806.5	0.666666667	806.5	1	42	28.39894364	28.39894364	28.39894364
782.5	0.666666667	782.5	0.666666667	782.5	1	46	27.97320146	27.97320146	27.97320146
737.5	0.666666667	737.5	0.666666667	737.5	1	2	27.15695123	27.15695123	27.15695123
716.5	0.666666667	716.5	0.666666667	716.5	1	6	26.76751763	26.76751763	26.76751763
677.5	0.666666667	677.5	0.666666667	677.5	1	10	26.02883017	26.02883017	26.02883017
659.5	0.666666667	659.5	0.666666667	659.5	1	14	25.68073208	25.68073208	25.68073208
642.5	0.666666667	642.5	0.666666667	642.5	1	18	25.34758371	25.34758371	25.34758371
611.5	0.666666667	611.5	0.666666667	611.5	1	22	24.72852604	24.72852604	24.72852604
597.5	0.666666667	597.5	0.666666667	597.5	1	26	24.44381312	24.44381312	24.44381312
584.5	0.666666667	584.5	0.666666667	584.5	1	30	24.17643481	24.17643481	24.17643481
561.5	0.666666667	561.5	0.666666667	561.5	1	34	23.69599122	23.69599122	23.69599122
551.5	0.666666667	551.5	0.666666667	551.5	1	38	23.48403713	23.48403713	23.48403713
542.5	0.666666667	542.5	0.666666667	542.5	1	42	23.2916294	23.2916294	23.2916294
527.5	0.666666667	527.5	0.666666667	527.5	1	46	22.96736816	22.96736816	22.96736816
516.5	0.666666667	516.5	0.666666667	516.5	1	2	22.72663635	22.72663635	22.72663635
512.5	0.666666667	512.5	0.666666667	512.5	1	6	22.63846285	22.63846285	22.63846285
509.5	0.666666667	509.5	0.666666667	509.5	1	10	22.57210668	22.57210668	22.57210668
1409	0.666666667	1409	0.666666667	1409	1	14	37.53664876	37.53664876	37.53664876
1366.5	0.666666667	1366.5	0.666666667	1366.5	1	18	36.96620078	36.96620078	36.96620078
1325	0.666666667	1325	0.666666667	1325	1	22	36.40054945	36.40054945	36.40054945
1245	0.666666667	1245	0.666666667	1245	1	26	35.28455753	35.28455753	35.28455753
1206.5	0.666666667	1206.5	0.666666667	1206.5	1	30	34.73470887	34.73470887	34.73470887
1169	0.666666667	1169	0.666666667	1169	1	34	34.19064199	34.19064199	34.19064199
1097	0.666666667	1097	0.666666667	1097	1	38	33.12099032	33.12099032	33.12099032
1062.5	0.666666667	1062.5	0.666666667	1062.5	1	42	32.59601203	32.59601203	32.59601203
1029	0.666666667	1029	0.666666667	1029	1	46	32.07802986	32.07802986	32.07802986
965	0.666666667	965	0.666666667	965	1	2	31.06444913	31.06444913	31.06444913
905	0.666666667	905	0.666666667	905	1	6	30.08321791	30.08321791	30.08321791
876.5	0.666666667	876.5	0.666666667	876.5	1	10	29.60574269	29.60574269	29.60574269
849	0.666666667	849	0.666666667	849	1	14	29.13760457	29.13760457	29.13760457
797	0.666666667	797	0.666666667	797	1	18	28.23118843	28.23118843	28.23118843
772.5	0.666666667	772.5	0.666666667	772.5	1	22	27.79388422	27.79388422	27.79388422
749	0.666666667	749	0.666666667	749	1	26	27.36786437	27.36786437	27.36786437
705	0.666666667	705	0.666666667	705	1	30	26.55183609	26.55183609	26.55183609
684.5	0.666666667	684.5	0.666666667	684.5	1	34	26.1629509	26.1629509	26.1629509
665	0.666666667	665	0.666666667	665	1	38	25.78759392	25.78759392	25.78759392
629	0.666666667	629	0.666666667	629	1	42	25.07987241	25.07987241	25.07987241
612.5	0.666666667	612.5	0.666666667	612.5	1	46	24.74873734	24.74873734	24.74873734
582.5	0.666666667	582.5	0.666666667	582.5	1	2	24.13503677	24.13503677	24.13503677
569	0.666666667	569	0.666666667	569	1	6	23.85372088	23.85372088	23.85372088
545	0.666666667	545	0.666666667	545	1	10	23.34523506	23.34523506	23.34523506
534.5	0.666666667	534.5	0.666666667	534.5	1	14	23.11925604	23.11925604	23.11925604
525	0.666666667	525	0.666666667	525	1	18	22.91287847	22.91287847	22.91287847
509	0.666666667	509	0.666666667	509	1	22	22.56102835	22.56102835	22.56102835
502.5	0.666666667	502.5	0.666666667	502.5	1	26	22.41651177	22.41651177	22.41651177
497	0.666666667	497	0.666666667	497	1	30	22.29349681	22.29349681	22.29349681
489	0.666666667	489	0.666666667	489	1	34	22.11334439	22.11334439	22.11334439
486.5	0.673469388	486.5	0.666666667	486.5	1	38	22.056745	22.056745	22.056745
1324.5	0.666666667	1324.5	0.666666667	1324.5	1	42	36.39368077	36.39368077	36.39368077
1283.5	0.666666667	1283.5	0.666666667	1283.5	1	46	35.82596824	35.82596824	35.82596824
1204.5	0.666666667	1204.5	0.666666667	1204.5	1	2	34.70590728	34.70590728	34.70590728
1129.5	0.666666667	1129.5	0.666666667	1129.5	1	6	33.60803475	33.60803475	33.60803475
1093.5	0.666666667	1093.5	0.666666667	1093.5	1	10	33.06811153	33.06811153	33.06811153
1058.5	0.666666667	1058.5	0.666666667	1058.5	1	14	32.53459697	32.53459697	32.53459697
991.5	0.666666667	991.5	0.666666667	991.5	1	18	31.48809299	31.48809299	31.48809299
959.5	0.666666667	959.5	0.666666667	959.5	1	22	30.975797	30.975797	30.975797
928.5	0.666666667	928.5	0.666666667	928.5	1	26	30.47129797	30.47129797	30.47129797
869.5	0.666666667	869.5	0.666666667	869.5	1	30	29.4872854	29.4872854	29.4872854
841.5	0.666666667	841.5	0.666666667	841.5	1	34	29.00861941	29.00861941	29.00861941
814.5	0.666666667	814.5	0.666666667	814.5	1	38	28.53944639	28.53944639	28.53944639
763.5	0.666666667	763.5	0.666666667	763.5	1	42	27.63150376	27.63150376	27.63150376
739.5	0.666666667	739.5	0.666666667	739.5	1	46	27.19374928	27.19374928	27.19374928
694.5	0.666666667	694.5	0.666666667	694.5	1	2	26.35336791	26.35336791	26.35336791
673.5	0.666666667	673.5	0.666666667	673.5	1	6	25.95187854	25.95187854	25.95187854
634.5	0.666666667	634.5	0.666666667	634.5	1	10	25.18928344	25.18928344	25.18928344
616.5	0.666666667	616.5	0.666666667	616.5	1	14	24.82941804	24.82941804	24.82941804
599.5	0.666666667	599.5	0.666666667	599.5	1	18	24.48468909	24.48468909	24.48468909
568.5	0.666666667	568.5	0.666666667	568.5	1	22	23.84323804	23.84323804	23.84323804
554.5	0.666666667	554.5	0.666666667	554.5	1	26	23.54782368	23.54782368	23.54782368
541.5	0.666666667	541.5	0.666666667	541.5	1	30	23.27015256	23.27015256	23.27015256
518.5	0.666666667	518.5	0.666666667	518.5	1	34	22.77059507	22.77059507	22.77059507
508.5	0.666666667	508.5	0.666666667	508.5	1	38	22.54994457	22.54994457	22.54994457
499.5	0.666666667	499.5	0.666666667	499.5	1	42	22.34949664	22.34949664	22.34949664
484.5	0.666666667	484.5	0.666666667	484.5	1	46	22.0113607	22.0113607	22.0113607
473.5	0.666666667	473.5	0.666666667	473.5	1	2	21.76005515	21.76005515	21.76005515
469.5	0.666666667	469.5	0.666666667	469.5	1	6	21.66794868	21.66794868	21.66794868
464.5	0.680555556	464.5	0.666666667	464.5	1	10	21.55226206	21.55226206	21.55226206
1243	0.666666667	1243	0.666666667	1243	1	14	35.25620513	35.25620513	35.25620513
1165	0.666666667	1165	0.666666667	1165	1	18	34.13209633	34.13209633	34.13209633
1127.5	0.666666667	1127.5	0.666666667	1127.5	1	22	33.57826678	33.57826678	33.57826678
1091	0.666666667	1091	0.666666667	1091	1	26	33.03028913	33.03028913	33.03028913
1021	0.666666667	1021	0.666666667	1021	1	30	31.95309062	31.95309062	31.95309062
987.5	0.666666667	987.5	0.666666667	987.5	1	34	31.42451272	31.42451272	31.42451272
955	0.666666667	955	0.666666667	955	1	38	30.90307428	30.90307428	30.90307428
893	0.666666667	893	0.666666667	893	1	42	29.88310559	29.88310559	29.88310559
863.5	0.666666667	863.5	0.666666667	863.5	1	46	29.38537051	29.38537051	29.38537051
807.5	0.666666667	807.5	0.666666667	807.5	1	2	28.41654448	28.41654448	28.41654448
781	0.666666667	781	0.666666667	781	1	6	27.94637722	27.94637722	27.94637722
731	0.666666667	731	0.666666667	731	1	10	27.03701167	27.03701167	27.03701167
707.5	0.666666667	707.5	0.666666667	707.5	1	14	26.59887216	26.59887216	26.59887216
685	0.666666667	685	0.666666667	685	1	18	26.17250466	26.17250466	26.17250466
643	0.666666667	643	0.666666667	643	1	22	25.35744467	25.35744467	25.35744467
623.5	0.666666667	623.5	0.666666667	623.5	1	26	24.96998198	24.96998198	24.96998198
605	0.666666667	605	0.666666667	605	1	30	24.59674775	24.59674775	24.59674775
571	0.666666667	571	0.666666667	571	1	34	23.89560629	23.89560629	23.89560629
555.5	0.666666667	555.5	0.666666667	555.5	1	38	23.5690475	23.5690475	23.5690475
541	0.666666667	541	0.666666667	541	1	42	23.2594067	23.2594067	23.2594067
515	0.666666667	515	0.666666667	515	1	46	22.69361144	22.69361144	22.69361144
493	0.666666667	493	0.666666667	493	1	2	22.20360331	22.20360331	22.20360331
483.5	0.666666667	483.5	0.666666667	483.5	1	6	21.98863343	21.98863343	21.98863343
475	0.666666667	475	0.666666667	475	1	10	21.79449472	21.79449472	21.79449472
461	0.666666667	461	0.666666667	461	1	14	21.47091055	21.47091055	21.47091055
455.5	0.666666667	455.5	0.666666667	455.5	1	18	21.34244597	21.34244597	21.34244597
451	0.666666667	451	0.666666667	451	1	22	21.23676058	21.23676058	21.23676058
443.5	0.687943262	443.5	0.666666667	443.5	1	26	21.05943969	21.05943969	21.05943969
1164.5	0.666666667	1164.5	0.666666667	1164.5	1	30	34.12477106	34.12477106	34.12477106
1089.5	0.666666667	1089.5	0.666666667	1089.5	1	34	33.00757489	33.00757489	33.00757489
1053.5	0.666666667	1053.5	0.666666667	1053.5	1	38	32.45766473	32.45766473	32.45766473
1018.5	0.666666667	1018.5	0.666666667	1018.5	1	42	31.91394679	31.91394679	31.91394679
951.5	0.666666667	951.5	0.666666667	951.5	1	46	30.84639363	30.84639363	30.84639363
888.5	0.666666667	888.5	0.666666667	888.5	1	2	29.80771712	29.80771712	29.80771712
858.5	0.666666667	858.5	0.666666667	858.5	1	6	29.30017065	29.30017065	29.30017065
829.5	0.666666667	829.5	0.666666667	829.5	1	10	28.80104165	28.80104165	28.80104165
774.5	0.666666667	774.5	0.666666667	774.5	1	14	27.8298401	27.8298401	27.8298401
748.5	0.666666667	748.5	0.666666667	748.5	1	18	27.35872804	27.35872804	27.35872804
723.5	0.666666667	723.5	0.666666667	723.5	1	22	26.89795531	26.89795531	26.89795531
676.5	0.666666667	676.5	0.666666667	676.5	1	26	26.00961361	26.00961361	26.00961361
654.5	0.666666667	654.5	0.666666667	654.5	1	30	25.58319761	25.58319761	25.58319761
633.5	0.666666667	633.5	0.666666667	633.5	1	34	25.1694259	25.1694259	25.1694259
594.5	0.666666667	594.5	0.666666667	594.5	1	38	24.38237068	24.38237068	24.38237068
576.5	0.666666667	576.5	0.666666667	576.5	1	42	24.01041441	24.01041441	24.01041441
559.5	0.666666667	559.5	0.666666667	559.5	1	46	23.65375235	23.65375235	23.65375235
528.5	0.666666667	528.5	0.666666667	528.5	1	2	22.98912787	22.98912787	22.98912787
501.5	0.666666667	501.5	0.666666667	501.5	1	6	22.39419568	22.39419568	22.39419568
489.5	0.666666667	489.5	0.666666667	489.5	1	10	22.12464689	22.12464689	22.12464689
478.5	0.666666667	478.5	0.666666667	478.5	1	14	21.87464285	21.87464285	21.87464285
459.5	0.666666667	459.5	0.666666667	459.5	1	18	21.43595111	21.43595111	21.43595111
451.5	0.666666667	451.5	0.666666667	451.5	1	22	21.24852936	21.24852936	21.24852936
444.5	0.666666667	444.5	0.666666667	444.5	1	26	21.08316864	21.08316864	21.08316864
433.5	0.666666667	433.5	0.666666667	433.5	1	30	20.82066281	20.82066281	20.82066281
429.5	0.673469388	429.5	0.666666667	429.5	1	34	20.72438178	20.72438178	20.72438178
1089	0.666666667	1089	0.666666667	1089	1	38	33	33	33
1052.5	0.666666667	1052.5	0.666666667	1052.5	1	42	32.4422564	32.4422564	32.4422564
1017	0.666666667	1017	0.666666667	1017	1	46	31.89043744	31.89043744	31.89043744
949	0.666666667	949	0.666666667	949	1	2	30.8058436	30.8058436	30.8058436
885	0.666666667	885	0.666666667	885	1	6	29.74894956	29.74894956	29.74894956
854.5	0.666666667	854.5	0.666666667	854.5	1	10	29.23183196	29.23183196	29.23183196
825	0.666666667	825	0.666666667	825	1	14	28.72281323	28.72281323	28.72281323
769	0.666666667	769	0.666666667	769	1	18	27.73084925	27.73084925	27.73084925
742.5	0.666666667	742.5	0.666666667	742.5	1	22	27.24885319	27.24885319	27.24885319
717	0.666666667	717	0.666666667	717	1	26	26.77685568	26.77685568	26.77685568
669	0.666666667	669	0.666666667	669	1	30	25.86503431	25.86503431	25.86503431
646.5	0.666666667	646.5	0.666666667	646.5	1	34	25.42636427	25.42636427	25.42636427
625	0.666666667	625	0.666666667	625	1	38	25	25	25
585	0.666666667	585	0.666666667	585	1	42	24.18677324	24.18677324	24.18677324
566.5	0.666666667	566.5	0.666666667	566.5	1	46	23.80126047	23.80126047	23.80126047
532.5	0.666666667	532.5	0.666666667	532.5	1	2	23.07596152	23.07596152	23.07596152
517	0.666666667	517	0.666666667	517	1	6	22.737634	22.737634	22.737634
489	0.666666667	489	0.666666667	489	1	10	22.11334439	22.11334439	22.11334439
476.5	0.666666667	476.5	0.666666667	476.5	1	14	21.82887995	21.82887995	21.82887995
465	0.666666667	465	0.666666667	465	1	18	21.56385865	21.56385865	21.56385865
445	0.666666667	445	0.666666667	445	1	22	21.09502311	21.09502311	21.09502311
436.5	0.666666667	436.5	0.666666667	436.5	1	26	20.89258242	20.89258242	20.89258242
429	0.666666667	429	0.666666667	429	1	30	20.71231518	20.71231518	20.71231518
417	0.666666667	417	0.666666667	417	1	34	20.42057786	20.42057786	20.42057786
412.5	0.673469388	412.5	0.666666667	412.5	1	38	20.31009601	20.31009601	20.31009601
404.5	0.703703704	404.5	0.666666667	404.5	1	42	20.11218536	20.11218536	20.11218536
981.5	0.666666667	981.5	0.666666667	981.5	1	46	31.3289004	31.3289004	31.3289004
914.5	0.666666667	914.5	0.666666667	914.5	1	2	30.24070105	30.24070105	30.24070105
882.5	0.666666667	882.5	0.666666667	882.5	1	6	29.70690156	29.70690156	29.70690156
851.5	0.666666667	851.5	0.666666667	851.5	1	10	29.18047292	29.18047292	29.18047292
792.5	0.666666667	792.5	0.666666667	792.5	1	14	28.15137652	28.15137652	28.15137652
764.5	0.666666667	764.5	0.666666667	764.5	1	18	27.64959313	27.64959313	27.64959313
737.5	0.666666667	737.5	0.666666667	737.5	1	22	27.15695123	27.15695123	27.15695123
686.5	0.666666667	686.5	0.666666667	686.5	1	26	26.20114501	26.20114501	26.20114501
662.5	0.666666667	662.5	0.666666667	662.5	1	30	25.73907535	25.73907535	25.73907535
639.5	0.666666667	639.5	0.666666667	639.5	1	34	25.28833723	25.28833723	25.28833723
596.5	0.666666667	596.5	0.666666667	596.5	1	38	24.42334948	24.42334948	24.42334948
576.5	0.666666667	576.5	0.666666667	576.5	1	42	24.01041441	24.01041441	24.01041441
557.5	0.666666667	557.5	0.666666667	557.5	1	46	23.61143791	23.61143791	23.61143791
522.5	0.666666667	522.5	0.666666667	522.5	1	2	22.8582589	22.8582589	22.8582589
491.5	0.666666667	491.5	0.666666667	491.5	1	6	22.16979928	22.16979928	22.16979928
477.5	0.666666667	477.5	0.666666667	477.5	1	10	21.85177338	21.85177338	21.85177338
464.5	0.666666667	464.5	0.666666667	464.5	1	14	21.55226206	21.55226206	21.55226206
441.5	0.666666667	441.5	0.666666667	441.5	1	18	21.01190139	21.01190139	21.01190139
431.5	0.666666667	431.5	0.666666667	431.5	1	22	20.77257808	20.77257808	20.77257808
422.5	0.666666667	422.5	0.666666667	422.5	1	26	20.55480479	20.55480479	20.55480479
407.5	0.666666667	407.5	0.666666667	407.5	1	30	20.18662924	20.18662924	20.18662924
401.5	0.666666667	401.5	0.666666667	401.5	1	34	20.03746491	20.03746491	20.03746491
392.5	0.680555556	392.5	0.666666667	392.5	1	38	19.81161276	19.81161276	19.81161276
947	0.666666667	947	0.666666667	947	1	42	30.77336511	30.77336511	30.77336511
913.5	0.666666667	913.5	0.666666667	913.5	1	46	30.22416252	30.22416252	30.22416252
849.5	0.666666667	849.5	0.666666667	849.5	1	2	29.14618328	29.14618328	29.14618328
819	0.666666667	819	0.666666667	819	1	6	28.61817604	28.61817604	28.61817604
761	0.666666667	761	0.666666667	761	1	10	27.58622845	27.58622845	27.58622845
733.5	0.666666667	733.5	0.666666667	733.5	1	14	27.08320513	27.08320513	27.08320513
707	0.666666667	707	0.666666667	707	1	18	26.5894716	26.5894716	26.5894716
657	0.666666667	657	0.666666667	657	1	22	25.63201124	25.63201124	25.63201124
633.5	0.666666667	633.5	0.666666667	633.5	1	26	25.1694259	25.1694259	25.1694259
611	0.666666667	611	0.666666667	611	1	30	24.71841419	24.71841419	24.71841419
569	0.666666667	569	0.666666667	569	1	34	23.85372088	23.85372088	23.85372088
549.5	0.666666667	549.5	0.666666667	549.5	1	38	23.44141634	23.44141634	23.44141634
531	0.666666667	531	0.666666667	531	1	42	23.04343724	23.04343724	23.04343724
497	0.666666667	497	0.666666667	497	1	46	22.29349681	22.29349681	22.29349681
467	0.666666667	467	0.666666667	467	1	2	21.61018278	21.61018278	21.61018278
453.5	0.666666667	453.5	0.666666667	453.5	1	6	21.29553944	21.29553944	21.29553944
441	0.666666667	441	0.666666667	441	1	10	21	21	21
419	0.666666667	419	0.666666667	419	1	14	20.46948949	20.46948949	20.46948949
409.5	0.666666667	409.5	0.666666667	409.5	1	18	20.23610634	20.23610634	20.23610634
401	0.666666667	401	0.666666667	401	1	22	20.02498439	20.02498439	20.02498439
387	0.666666667	387	0.666666667	387	1	26	19.67231557	19.67231557	19.67231557
381.5	0.673469388	381.5	0.666666667	381.5	1	30	19.53202498	19.53202498	19.53202498
369.5	0.703703704	369.5	0.666666667	369.5	1	34	19.22238279	19.22238279	19.22238279
880.5	0.666666667	880.5	0.666666667	880.5	1	38	29.67322025	29.67322025	29.67322025
817.5	0.666666667	817.5	0.666666667	817.5	1	42	28.59195691	28.59195691	28.59195691
787.5	0.666666667	787.5	0.666666667	787.5	1	46	28.0624304	28.0624304	28.0624304
730.5	0.666666667	730.5	0.666666667	730.5	1	2	27.0277635	27.0277635	27.0277635
703.5	0.666666667	703.5	0.666666667	703.5	1	6	26.52357442	26.52357442	26.52357442
652.5	0.666666667	652.5	0.666666667	652.5	1	10	25.54407955	25.54407955	25.54407955
628.5	0.666666667	628.5	0.666666667	628.5	1	14	25.06990227	25.06990227	25.06990227
605.5	0.666666667	605.5	0.666666667	605.5	1	18	24.6069096	24.6069096	24.6069096
562.5	0.666666667	562.5	0.666666667	562.5	1	22	23.71708245	23.71708245	23.71708245
542.5	0.666666667	542.5	0.666666667	542.5	1	26	23.2916294	23.2916294	23.2916294
523.5	0.666666667	523.5	0.666666667	523.5	1	30	22.88012238	22.88012238	22.88012238
488.5	0.666666667	488.5	0.666666667	488.5	1	34	22.10203611	22.10203611	22.10203611
472.5	0.666666667	472.5	0.666666667	472.5	1	38	21.73706512	21.73706512	21.73706512
457.5	0.666666667	457.5	0.666666667	457.5	1	42	21.38924964	21.38924964	21.38924964
430.5	0.666666667	430.5	0.666666667	430.5	1	46	20.74849392	20.74849392	20.74849392
407.5	0.666666667	407.5	0.666666667	407.5	1	2	20.18662924	20.18662924	20.18662924
397.5	0.666666667	397.5	0.666666667	397.5	1	6	19.93740204	19.93740204	19.93740204
388.5	0.666666667	388.5	0.666666667	388.5	1	10	19.71040334	19.71040334	19.71040334
373.5	0.666666667	373.5	0.666666667	373.5	1	14	19.32614809	19.32614809	19.32614809
367.5	0.673469388	367.5	0.666666667	367.5	1	18	19.17028951	19.17028951	19.17028951
353.5	0.703703704	353.5	0.666666667	353.5	1	22	18.80159568	18.80159568	18.80159568
817	0.666666667	817	0.666666667	817	1	26	28.58321186	28.58321186	28.58321186
757	0.666666667	757	0.666666667	757	1	30	27.51363298	27.51363298	27.51363298
728.5	0.666666667	728.5	0.666666667	728.5	1	34	26.99073915	26.99073915	26.99073915
701	0.666666667	701	0.666666667	701	1	38	26.47640459	26.47640459	26.47640459
649	0.666666667	649	0.666666667	649	1	42	25.47547841	25.47547841	25.47547841
624.5	0.666666667	624.5	0.666666667	624.5	1	46	24.989998	24.989998	24.989998
578.5	0.666666667	578.5	0.666666667	578.5	1	2	24.05202694	24.05202694	24.05202694
557	0.666666667	557	0.666666667	557	1	6	23.60084744	23.60084744	23.60084744
517	0.666666667	517	0.666666667	517	1	10	22.737634	22.737634	22.737634
498.5	0.666666667	498.5	0.666666667	498.5	1	14	22.32711356	22.32711356	22.32711356
481	0.666666667	481	0.666666667	481	1	18	21.9317122	21.9317122	21.9317122
449	0.666666667	449	0.666666667	449	1	22	21.1896201	21.1896201	21.1896201
434.5	0.666666667	434.5	0.666666667	434.5	1	26	20.84466359	20.84466359	20.84466359
421	0.666666667	421	0.666666667	421	1	30	20.51828453	20.51828453	20.51828453
397	0.666666667	397	0.666666667	397	1	34	19.92485885	19.92485885	19.92485885
386.5	0.666666667	386.5	0.666666667	386.5	1	38	19.65960325	19.65960325	19.65960325
377	0.666666667	377	0.666666667	377	1	42	19.41648784	19.41648784	19.41648784
361	0.666666667	361	0.666666667	361	1	46	19	19	19
344.5	0.687943262	344.5	0.666666667	344.5	1	2	18.56071119	18.56071119	18.56071119
336.5	0.720930233	336.5	0.666666667	336.5	1	6	18.34393633	18.34393633	18.34393633
727.5	0.666666667	727.5	0.666666667	727.5	1	10	26.97220792	26.97220792	26.97220792
699.5	0.666666667	699.5	0.666666667	699.5	1	14	26.44806231	26.44806231	26.44806231
672.5	0.666666667	672.5	0.666666667	672.5	1	18	25.93260496	25.93260496	25.93260496
621.5	0.666666667	621.5	0.666666667	621.5	1	22	24.92990172	24.92990172	24.92990172
597.5	0.666666667	597.5	0.666666667	597.5	1	26	24.44381312	24.44381312	24.44381312
574.5	0.666666667	574.5	0.666666667	574.5	1	30	23.96872963	23.96872963	23.96872963
531.5	0.666666667	531.5	0.666666667	531.5	1	34	23.05428377	23.05428377	23.05428377
511.5	0.666666667	511.5	0.666666667	511.5	1	38	22.61636576	22.61636576	22.61636576
492.5	0.666666667	492.5	0.666666667	492.5	1	42	22.19234102	22.19234102	22.19234102
457.5	0.666666667	457.5	0.666666667	457.5	1	46	21.38924964	21.38924964	21.38924964
426.5	0.666666667	426.5	0.666666667	426.5	1	2	20.65187643	20.65187643	20.65187643
412.5	0.666666667	412.5	0.666666667	412.5	1	6	20.31009601	20.31009601	20.31009601
399.5	0.666666667	399.5	0.666666667	399.5	1	10	19.98749609	19.98749609	19.98749609
376.5	0.666666667	376.5	0.666666667	376.5	1	14	19.40360791	19.40360791	19.40360791
366.5	0.666666667	366.5	0.666666667	366.5	1	18	19.14418972	19.14418972	19.14418972
357.5	0.666666667	357.5	0.666666667	357.5	1	22	18.9076704	18.9076704	18.9076704
349.5	0.666666667	349.5	0.666666667	349.5	1	26	18.6949191	18.6949191	18.6949191
327.5	0.695652174	327.5	0.666666667	327.5	1	30	18.09696107	18.09696107	18.09696107
699	0.666666667	699	0.666666667	699	1	34	26.43860813	26.43860813	26.43860813
671.5	0.666666667	671.5	0.666666667	671.5	1	38	25.91331704	25.91331704	25.91331704
645	0.666666667	645	0.666666667	645	1	42	25.3968502	25.3968502	25.3968502
619.5	0.666666667	619.5	0.666666667	619.5	1	46	24.88975693	24.88975693	24.88975693
595	0.666666667	595	0.666666667	595	1	2	24.39262184	24.39262184	24.39262184
571.5	0.666666667	571.5	0.666666667	571.5	1	6	23.90606618	23.90606618	23.90606618
549	0.666666667	549	0.666666667	549	1	10	23.43074903	23.43074903	23.43074903
527.5	0.666666667	527.5	0.666666667	527.5	1	14	22.96736816	22.96736816	22.96736816
507	0.666666667	507	0.666666667	507	1	18	22.5166605	22.5166605	22.5166605
487.5	0.666666667	487.5	0.666666667	487.5	1	22	22.07940217	22.07940217	22.07940217
469	0.666666667	469	0.666666667	469	1	26	21.65640783	21.65640783	21.65640783
451.5	0.666666667	451.5	0.666666667	451.5	1	30	21.24852936	21.24852936	21.24852936
435	0.666666667	435	0.666666667	435	1	34	20.85665361	20.85665361	20.85665361
419.5	0.666666667	419.5	0.666666667	419.5	1	38	20.48169915	20.48169915	20.48169915
405	0.666666667	405	0.666666667	405	1	42	20.1246118	20.1246118	20.1246118
391.5	0.666666667	391.5	0.666666667	391.5	1	46	19.78635894	19.78635894	19.78635894
367.5	0.666666667	367.5	0.666666667	367.5	1	2	19.17028951	19.17028951	19.17028951
357	0.666666667	357	0.666666667	357	1	6	18.89444363	18.89444363	18.89444363
347.5	0.666666667	347.5	0.666666667	347.5	1	10	18.64135188	18.64135188	18.64135188
339	0.666666667	339	0.666666667	339	1	14	18.41195264	18.41195264	18.41195264
339	0.666666667	339	0.666666667	339	1	18	18.41195264	18.41195264	18.41195264
315	0.695652174	315	0.666666667	315	1	22	17.74823935	17.74823935	17.74823935
307	0.73015873	307	0.666666667	307	1	26	17.52141547	17.52141547	17.52141547
569.5	0.671834625	569.5	0.666666667	569.5	1	30	23.86419913	23.86419913	23.86419913
483.5	0.671834625	483.5	0.666666667	483.5	1	34	21.98863343	21.98863343	21.98863343
413.5	0.671834625	413.5	0.666666667	413.5	1	38	20.33469941	20.33469941	20.33469941
359.5	0.671834625	359.5	0.666666667	359.5	1	42	18.96048523	18.96048523	18.96048523
321.5	0.673469388	321.5	0.666666667	321.5	1	46	17.93042108	17.93042108	17.93042108
294.5	0.720930233	294.5	0.666666667	294.5	1	2	17.1610023	17.1610023	17.1610023
545	0.676923077	545	0.666666667	545	1	6	23.34523506	23.34523506	23.34523506
461	0.676923077	461	0.666666667	461	1	10	21.47091055	21.47091055	21.47091055
393	0.676923077	393	0.666666667	393	1	14	19.8242276	19.8242276	19.8242276
341	0.676923077	341	0.666666667	341	1	18	18.46618531	18.46618531	18.46618531
305	0.680555556	305	0.666666667	305	1	22	17.4642492	17.4642492	17.4642492
285	0.712121212	285	0.666666667	285	1	26	16.88194302	16.88194302	16.88194302
544.5	0.676923077	544.5	0.666666667	544.5	1	30	23.33452378	23.33452378	23.33452378
458.5	0.676923077	458.5	0.666666667	458.5	1	34	21.41261311	21.41261311	21.41261311
388.5	0.676923077	388.5	0.666666667	388.5	1	38	19.71040334	19.71040334	19.71040334
334.5	0.676923077	334.5	0.666666667	334.5	1	42	18.28934116	18.28934116	18.28934116
296.5	0.680555556	296.5	0.666666667	296.5	1	46	17.21917536	17.21917536	17.21917536
269.5	0.73015873	269.5	0.666666667	269.5	1	2	16.41645516	16.41645516	16.41645516
457	0.676923077	457	0.666666667	457	1	6	21.37755833	21.37755833	21.37755833
385	0.676923077	385	0.666666667	385	1	10	19.62141687	19.62141687	19.62141687
329	0.676923077	329	0.666666667	329	1	14	18.13835715	18.13835715	18.13835715
289	0.680555556	289	0.666666667	289	1	18	17	17	17
265	0.712121212	265	0.666666667	265	1	22	16.2788206	16.2788206	16.2788206
257	0.75	257	0.666666667	257	1	26	16.03121954	16.03121954	16.03121954
399.5	0.676923077	399.5	0.666666667	399.5	1	30	19.98749609	19.98749609	19.98749609
337.5	0.676923077	337.5	0.666666667	337.5	1	34	18.37117307	18.37117307	18.37117307
291.5	0.676923077	291.5	0.666666667	291.5	1	38	17.07337108	17.07337108	17.07337108
261.5	0.703703704	261.5	0.666666667	261.5	1	42	16.17096163	16.17096163	16.17096163
247.5	0.739837398	247.5	0.666666667	247.5	1	46	15.73213272	15.73213272	15.73213272
349	0.676923077	349	0.666666667	349	1	2	18.68154169	18.68154169	18.68154169
297	0.676923077	297	0.666666667	297	1	6	17.23368794	17.23368794	17.23368794
261	0.695652174	261	0.666666667	261	1	10	16.15549442	16.15549442	16.15549442
241	0.73015873	241	0.666666667	241	1	14	15.5241747	15.5241747	15.5241747
380.5	0.676923077	380.5	0.666666667	380.5	1	18	19.5064092	19.5064092	19.5064092
318.5	0.676923077	318.5	0.666666667	318.5	1	22	17.8465683	17.8465683	17.8465683
272.5	0.680555556	272.5	0.666666667	272.5	1	26	16.50757402	16.50757402	16.50757402
242.5	0.712121212	242.5	0.666666667	242.5	1	30	15.5724115	15.5724115	15.5724115
228.5	0.75	228.5	0.666666667	228.5	1	34	15.11621646	15.11621646	15.11621646
317	0.676923077	317	0.666666667	317	1	38	17.80449381	17.80449381	17.80449381
269	0.680555556	269	0.666666667	269	1	42	16.40121947	16.40121947	16.40121947
237	0.712121212	237	0.666666667	237	1	46	15.39480432	15.39480432	15.39480432
219	0.771929825	219	0.666666667	219	1	2	14.79864859	14.79864859	14.79864859
277.5	0.676923077	277.5	0.666666667	277.5	1	6	16.65833125	16.65833125	16.65833125
239.5	0.703703704	239.5	0.666666667	239.5	1	10	15.47578754	15.47578754	15.47578754
217.5	0.739837398	217.5	0.666666667	217.5	1	14	14.7478812	14.7478812	14.7478812
289	0.676923077	289	0.666666667	289	1	18	17	17	17
245	0.695652174	245	0.666666667	245	1	22	15.65247584	15.65247584	15.65247584
217	0.73015873	217	0.666666667	217	1	26	14.73091986	14.73091986	14.73091986
205	0.771929825	205	0.666666667	205	1	30	14.31782106	14.31782106	14.31782106
243.5	0.695652174	243.5	0.666666667	243.5	1	34	15.60448653	15.60448653	15.60448653
213.5	0.73015873	213.5	0.666666667	213.5	1	38	14.6116392	14.6116392	14.6116392
199.5	0.771929825	199.5	0.666666667	199.5	1	42	14.12444689	14.12444689	14.12444689
225	0.712121212	225	0.666666667	225	1	46	15	15	15
195	0.771929825	195	0.666666667	195	1	2	13.96424004	13.96424004	13.96424004
216.5	0.720930233	216.5	0.666666667	216.5	1	6	14.71393897	14.71393897	14.71393897
194.5	0.760683761	194.5	0.666666667	194.5	1	10	13.94632568	13.94632568	13.94632568
209	0.73015873	209	0.666666667	209	1	14	14.45683229	14.45683229	14.45683229
189	0.771929825	189	0.666666667	189	1	18	13.74772708	13.74772708	13.74772708
196.5	0.75	196.5	0.666666667	196.5	1	22	14.01784577	14.01784577	14.01784577
182.5	0.796296296	182.5	0.666666667	182.5	1	26	13.50925609	13.50925609	13.50925609
181	0.796296296	181	0.666666667	181	1	30	13.45362405	13.45362405	13.45362405
178.5	0.80952381	178.5	0.666666667	178.5	1	34	13.36038922	13.36038922	13.36038922
1452	0.670886076	1452	0.666666667	1452	1	38	38.10511777	38.10511777	38.10511777
1284	0.670886076	1284	0.666666667	1284	1	42	35.83294573	35.83294573	35.83294573
1132	0.670886076	1132	0.666666667	1132	1	46	33.64520768	33.64520768	33.64520768
934	0.670886076	934	0.666666667	934	1	2	30.56141358	30.56141358	30.56141358
822	0.670886076	822	0.666666667	822	1	6	28.67054237	28.67054237	28.67054237
726	0.670886076	726	0.666666667	726	1	10	26.94438717	26.94438717	26.94438717
646	0.670886076	646	0.666666667	646	1	14	25.41653005	25.41653005	25.41653005
582	0.670886076	582	0.666666667	582	1	18	24.12467616	24.12467616	24.12467616
534	0.670886076	534	0.666666667	534	1	22	23.10844002	23.10844002	23.10844002
502	0.670886076	502	0.666666667	502	1	26	22.4053565	22.4053565	22.4053565
486	0.673469388	486	0.666666667	486	1	30	22.04540769	22.04540769	22.04540769
1323.5	0.670886076	1323.5	0.666666667	1323.5	1	34	36.37993953	36.37993953	36.37993953
1165.5	0.670886076	1165.5	0.666666667	1165.5	1	38	34.13942003	34.13942003	34.13942003
1023.5	0.670886076	1023.5	0.666666667	1023.5	1	42	31.99218655	31.99218655	31.99218655
897.5	0.670886076	897.5	0.666666667	897.5	1	46	29.95830436	29.95830436	29.95830436
738.5	0.670886076	738.5	0.666666667	738.5	1	2	27.17535648	27.17535648	27.17535648
652.5	0.670886076	652.5	0.666666667	652.5	1	6	25.54407955	25.54407955	25.54407955
582.5	0.670886076	582.5	0.666666667	582.5	1	10	24.13503677	24.13503677	24.13503677
528.5	0.670886076	528.5	0.666666667	528.5	1	14	22.98912787	22.98912787	22.98912787
490.5	0.670886076	490.5	0.666666667	490.5	1	18	22.14723459	22.14723459	22.14723459
468.5	0.670886076	468.5	0.666666667	468.5	1	22	21.64486082	21.64486082	21.64486082
1282	0.670886076	1282	0.666666667	1282	1	26	35.80502758	35.80502758	35.80502758
1126	0.670886076	1126	0.666666667	1126	1	30	33.55592347	33.55592347	33.55592347
986	0.670886076	986	0.666666667	986	1	34	31.40063694	31.40063694	31.40063694
862	0.670886076	862	0.666666667	862	1	38	29.35983651	29.35983651	29.35983651
754	0.670886076	754	0.666666667	754	1	42	27.45906044	27.45906044	27.45906044
662	0.670886076	662	0.666666667	662	1	46	25.72936066	25.72936066	25.72936066
554	0.670886076	554	0.666666667	554	1	2	23.53720459	23.53720459	23.53720459
502	0.670886076	502	0.666666667	502	1	6	22.4053565	22.4053565	22.4053565
466	0.670886076	466	0.666666667	466	1	10	21.58703314	21.58703314	21.58703314
446	0.673469388	446	0.666666667	446	1	14	21.11871208	21.11871208	21.11871208
1201.5	0.670886076	1201.5	0.666666667	1201.5	1	18	34.66266002	34.66266002	34.66266002
1051.5	0.670886076	1051.5	0.666666667	1051.5	1	22	32.42684073	32.42684073	32.42684073
917.5	0.670886076	917.5	0.666666667	917.5	1	26	30.29026246	30.29026246	30.29026246
799.5	0.670886076	799.5	0.666666667	799.5	1	30	28.27543103	28.27543103	28.27543103
697.5	0.670886076	697.5	0.666666667	697.5	1	34	26.41022529	26.41022529	26.41022529
611.5	0.670886076	611.5	0.666666667	611.5	1	38	24.72852604	24.72852604	24.72852604
541.5	0.670886076	541.5	0.666666667	541.5	1	42	23.27015256	23.27015256	23.27015256
487.5	0.670886076	487.5	0.666666667	487.5	1	46	22.07940217	22.07940217	22.07940217
436.5	0.670886076	436.5	0.666666667	436.5	1	2	20.89258242	20.89258242	20.89258242
422.5	0.687943262	422.5	0.666666667	422.5	1	6	20.55480479	20.55480479	20.55480479
1050	0.670886076	1050	0.666666667	1050	1	10	32.40370349	32.40370349	32.40370349
914	0.670886076	914	0.666666667	914	1	14	30.23243292	30.23243292	30.23243292
794	0.670886076	794	0.666666667	794	1	18	28.17800561	28.17800561	28.17800561
690	0.670886076	690	0.666666667	690	1	22	26.26785107	26.26785107	26.26785107
602	0.670886076	602	0.666666667	602	1	26	24.53568829	24.53568829	24.53568829
530	0.670886076	530	0.666666667	530	1	30	23.02172887	23.02172887	23.02172887
474	0.670886076	474	0.666666667	474	1	34	21.77154106	21.77154106	21.77154106
434	0.670886076	434	0.666666667	434	1	38	20.83266666	20.83266666	20.83266666
410	0.673469388	410	0.666666667	410	1	42	20.24845673	20.24845673	20.24845673
402	0.703703704	402	0.666666667	402	1	46	20.04993766	20.04993766	20.04993766
879.5	0.670886076	879.5	0.666666667	879.5	1	2	29.65636525	29.65636525	29.65636525
761.5	0.670886076	761.5	0.666666667	761.5	1	6	27.59528945	27.59528945	27.59528945
659.5	0.670886076	659.5	0.666666667	659.5	1	10	25.68073208	25.68073208	25.68073208
573.5	0.670886076	573.5	0.666666667	573.5	1	14	23.94786003	23.94786003	23.94786003
503.5	0.670886076	503.5	0.666666667	503.5	1	18	22.43880567	22.43880567	22.43880567
449.5	0.670886076	449.5	0.666666667	449.5	1	22	21.20141505	21.20141505	21.20141505
411.5	0.670886076	411.5	0.666666667	411.5	1	26	20.28546278	20.28546278	20.28546278
389.5	0.680555556	389.5	0.666666667	389.5	1	30	19.73575436	19.73575436	19.73575436
978	0.670886076	978	0.666666667	978	1	34	31.27299154	31.27299154	31.27299154
846	0.670886076	846	0.666666667	846	1	38	29.08607914	29.08607914	29.08607914
730	0.670886076	730	0.666666667	730	1	42	27.01851217	27.01851217	27.01851217
630	0.670886076	630	0.666666667	630	1	46	25.0998008	25.0998008	25.0998008
510	0.670886076	510	0.666666667	510	1	2	22.58317958	22.58317958	22.58317958
450	0.670886076	450	0.666666667	450	1	6	21.21320344	21.21320344	21.21320344
406	0.670886076	406	0.666666667	406	1	10	20.14944168	20.14944168	20.14944168
378	0.673469388	378	0.666666667	378	1	14	19.4422221	19.4422221	19.4422221
366	0.703703704	366	0.666666667	366	1	18	19.13112647	19.13112647	19.13112647
844.5	0.670886076	844.5	0.666666667	844.5	1	22	29.06028217	29.06028217	29.06028217
726.5	0.670886076	726.5	0.666666667	726.5	1	26	26.95366394	26.95366394	26.95366394
624.5	0.670886076	624.5	0.666666667	624.5	1	30	24.989998	24.989998	24.989998
538.5	0.670886076	538.5	0.666666667	538.5	1	34	23.20560277	23.20560277	23.20560277
468.5	0.670886076	468.5	0.666666667	468.5	1	38	21.64486082	21.64486082	21.64486082
414.5	0.670886076	414.5	0.666666667	414.5	1	42	20.35927307	20.35927307	20.35927307
376.5	0.670886076	376.5	0.666666667	376.5	1	46	19.40360791	19.40360791	19.40360791
349.5	0.703703704	349.5	0.666666667	349.5	1	2	18.6949191	18.6949191	18.6949191
782	0.670886076	782	0.666666667	782	1	6	27.96426291	27.96426291	27.96426291
670	0.670886076	670	0.666666667	670	1	10	25.88435821	25.88435821	25.88435821
574	0.670886076	574	0.666666667	574	1	14	23.9582971	23.9582971	23.9582971
494	0.670886076	494	0.666666667	494	1	18	22.22611077	22.22611077	22.22611077
430	0.670886076	430	0.666666667	430	1	22	20.73644135	20.73644135	20.73644135
382	0.670886076	382	0.666666667	382	1	26	19.54482029	19.54482029	19.54482029
350	0.673469388	350	0.666666667	350	1	30	18.70828693	18.70828693	18.70828693
334	0.703703704	334	0.666666667	334	1	34	18.27566688	18.27566688	18.27566688
751.5	0.670886076	751.5	0.666666667	751.5	1	38	27.41350032	27.41350032	27.41350032
641.5	0.670886076	641.5	0.666666667	641.5	1	42	25.32785028	25.32785028	25.32785028
547.5	0.670886076	547.5	0.666666667	547.5	1	46	23.39871791	23.39871791	23.39871791
436.5	0.670886076	436.5	0.666666667	436.5	1	2	20.89258242	20.89258242	20.89258242
382.5	0.670886076	382.5	0.666666667	382.5	1	6	19.55760722	19.55760722	19.55760722
344.5	0.670886076	344.5	0.666666667	344.5	1	10	18.56071119	18.56071119	18.56071119
322.5	0.695652174	322.5	0.666666667	322.5	1	14	17.958285	17.958285	17.958285
722	0.670886076	722	0.666666667	722	1	18	26.87005769	26.87005769	26.87005769
614	0.670886076	614	0.666666667	614	1	22	24.77902339	24.77902339	24.77902339
522	0.670886076	522	0.666666667	522	1	26	22.84731932	22.84731932	22.84731932
446	0.670886076	446	0.666666667	446	1	30	21.11871208	21.11871208	21.11871208
386	0.670886076	386	0.666666667	386	1	34	19.6468827	19.6468827	19.6468827
342	0.670886076	342	0.666666667	342	1	38	18.49324201	18.49324201	18.49324201
314	0.687943262	314	0.666666667	314	1	42	17.72004515	17.72004515	17.72004515
302	0.720930233	302	0.666666667	302	1	46	17.3781472	17.3781472	17.3781472
563.5	0.673684211	563.5	0.666666667	563.5	1	2	23.73815494	23.73815494	23.73815494
477.5	0.673684211	477.5	0.666666667	477.5	1	6	21.85177338	21.85177338	21.85177338
407.5	0.673684211	407.5	0.666666667	407.5	1	10	20.18662924	20.18662924	20.18662924
353.5	0.673684211	353.5	0.666666667	353.5	1	14	18.80159568	18.80159568	18.80159568
315.5	0.673684211	315.5	0.666666667	315.5	1	18	17.76231967	17.76231967	17.76231967
293.5	0.703703704	293.5	0.666666667	293.5	1	22	17.1318417	17.1318417	17.1318417
612	0.678851175	612	0.666666667	612	1	26	24.73863375	24.73863375	24.73863375
516	0.678851175	516	0.666666667	516	1	30	22.71563338	22.71563338	22.71563338
436	0.678851175	436	0.666666667	436	1	34	20.88061302	20.88061302	20.88061302
372	0.678851175	372	0.666666667	372	1	38	19.28730152	19.28730152	19.28730152
324	0.678851175	324	0.666666667	324	1	42	18	18	18
292	0.687943262	292	0.666666667	292	1	46	17.08800749	17.08800749	17.08800749
274	0.739837398	274	0.666666667	274	1	2	16.55294536	16.55294536	16.55294536
492.5	0.678851175	492.5	0.666666667	492.5	1	6	22.19234102	22.19234102	22.19234102
414.5	0.678851175	414.5	0.666666667	414.5	1	10	20.35927307	20.35927307	20.35927307
352.5	0.678851175	352.5	0.666666667	352.5	1	14	18.77498336	18.77498336	18.77498336
306.5	0.678851175	306.5	0.666666667	306.5	1	18	17.5071414	17.5071414	17.5071414
276.5	0.695652174	276.5	0.666666667	276.5	1	22	16.62828915	16.62828915	16.62828915
262.5	0.73015873	262.5	0.666666667	262.5	1	26	16.20185175	16.20185175	16.20185175
470	0.678851175	470	0.666666667	470	1	30	21.67948339	21.67948339	21.67948339
394	0.678851175	394	0.666666667	394	1	34	19.84943324	19.84943324	19.84943324
334	0.678851175	334	0.666666667	334	1	38	18.27566688	18.27566688	18.27566688
290	0.678851175	290	0.666666667	290	1	42	17.02938637	17.02938637	17.02938637
262	0.703703704	262	0.666666667	262	1	46	16.18641406	16.18641406	16.18641406
469.5	0.678851175	469.5	0.666666667	469.5	1	2	21.66794868	21.66794868	21.66794868
391.5	0.678851175	391.5	0.666666667	391.5	1	6	19.78635894	19.78635894	19.78635894
329.5	0.678851175	329.5	0.666666667	329.5	1	10	18.15213486	18.15213486	18.15213486
283.5	0.678851175	283.5	0.666666667	283.5	1	14	16.83745824	16.83745824	16.83745824
253.5	0.703703704	253.5	0.666666667	253.5	1	18	15.92168333	15.92168333	15.92168333
239.5	0.739837398	239.5	0.666666667	239.5	1	22	15.47578754	15.47578754	15.47578754
390	0.678851175	390	0.666666667	390	1	26	19.74841766	19.74841766	19.74841766
326	0.678851175	326	0.666666667	326	1	30	18.05547009	18.05547009	18.05547009
278	0.678851175	278	0.666666667	278	1	34	16.673332	16.673332	16.673332
246	0.703703704	246	0.666666667	246	1	38	15.68438714	15.68438714	15.68438714
230	0.739837398	230	0.666666667	230	1	42	15.16575089	15.16575089	15.16575089
371.5	0.678851175	371.5	0.666666667	371.5	1	46	19.27433527	19.27433527	19.27433527
284.5	0.678851175	284.5	0.666666667	284.5	1	2	16.86712779	16.86712779	16.86712779
246.5	0.695652174	246.5	0.666666667	246.5	1	6	15.70031847	15.70031847	15.70031847
224.5	0.73015873	224.5	0.666666667	224.5	1	10	14.98332406	14.98332406	14.98332406
354	0.678851175	354	0.666666667	354	1	14	18.81488772	18.81488772	18.81488772
294	0.678851175	294	0.666666667	294	1	18	17.1464282	17.1464282	17.1464282
250	0.687943262	250	0.666666667	250	1	22	15.8113883	15.8113883	15.8113883
222	0.720930233	222	0.666666667	222	1	26	14.89966443	14.89966443	14.89966443
210	0.760683761	210	0.666666667	210	1	30	14.49137675	14.49137675	14.49137675
292.5	0.678851175	292.5	0.666666667	292.5	1	34	17.10263138	17.10263138	17.10263138
246.5	0.687943262	246.5	0.666666667	246.5	1	38	15.70031847	15.70031847	15.70031847
216.5	0.720930233	216.5	0.666666667	216.5	1	42	14.71393897	14.71393897	14.71393897
202.5	0.760683761	202.5	0.666666667	202.5	1	46	14.23024947	14.23024947	14.23024947
244	0.687943262	244	0.666666667	244	1	2	15.62049935	15.62049935	15.62049935
212	0.720930233	212	0.666666667	212	1	6	14.56021978	14.56021978	14.56021978
196	0.760683761	196	0.666666667	196	1	10	14	14	14
253.5	0.680555556	253.5	0.666666667	253.5	1	14	15.92168333	15.92168333	15.92168333
215.5	0.712121212	215.5	0.666666667	215.5	1	18	14.67991826	14.67991826	14.67991826
193.5	0.75	193.5	0.666666667	193.5	1	22	13.91042774	13.91042774	13.91042774
242	0.687943262	242	0.666666667	242	1	26	15.55634919	15.55634919	15.55634919
206	0.720930233	206	0.666666667	206	1	30	14.35270009	14.35270009	14.35270009
186	0.760683761	186	0.666666667	186	1	34	13.6381817	13.6381817	13.6381817
221.5	0.703703704	221.5	0.666666667	221.5	1	38	14.88287607	14.88287607	14.88287607
191.5	0.739837398	191.5	0.666666667	191.5	1	42	13.8383525	13.8383525	13.8383525
177.5	0.783783784	177.5	0.666666667	177.5	1	46	13.32291259	13.32291259	13.32291259
180	0.760683761	180	0.666666667	180	1	2	13.41640786	13.41640786	13.41640786
172	0.80952381	172	0.666666667	172	1	6	13.11487705	13.11487705	13.11487705
174.5	0.771929825	174.5	0.666666667	174.5	1	10	13.20984481	13.20984481	13.20984481
178	0.760683761	178	0.666666667	178	1	14	13.34166406	13.34166406	13.34166406
166	0.80952381	166	0.666666667	166	1	18	12.88409873	12.88409873	12.88409873
164.5	0.80952381	164.5	0.666666667	164.5	1	22	12.82575534	12.82575534	12.82575534
162	0.838383838	162	0.666666667	162	1	26	12.72792206	12.72792206	12.72792206
1241	0.672897196	1241	0.666666667	1241	1	30	35.22782991	35.22782991	35.22782991
1089	0.672897196	1089	0.666666667	1089	1	34	33	33	33
953	0.672897196	953	0.666666667	953	1	38	30.87069808	30.87069808	30.87069808
833	0.672897196	833	0.666666667	833	1	42	28.86173938	28.86173938	28.86173938
729	0.672897196	729	0.666666667	729	1	46	27	27	27
603	0.672897196	603	0.666666667	603	1	2	24.55605832	24.55605832	24.55605832
539	0.672897196	539	0.666666667	539	1	6	23.21637353	23.21637353	23.21637353
491	0.672897196	491	0.666666667	491	1	10	22.15851981	22.15851981	22.15851981
459	0.672897196	459	0.666666667	459	1	14	21.42428529	21.42428529	21.42428529
443	0.680555556	443	0.666666667	443	1	18	21.04756518	21.04756518	21.04756518
1200.5	0.672897196	1200.5	0.666666667	1200.5	1	22	34.64823228	34.64823228	34.64823228
1050.5	0.672897196	1050.5	0.666666667	1050.5	1	26	32.41141774	32.41141774	32.41141774
916.5	0.672897196	916.5	0.666666667	916.5	1	30	30.27375101	30.27375101	30.27375101
798.5	0.672897196	798.5	0.666666667	798.5	1	34	28.2577423	28.2577423	28.2577423
696.5	0.672897196	696.5	0.666666667	696.5	1	38	26.39128644	26.39128644	26.39128644
610.5	0.672897196	610.5	0.666666667	610.5	1	42	24.7082982	24.7082982	24.7082982
540.5	0.672897196	540.5	0.666666667	540.5	1	46	23.24865588	23.24865588	23.24865588
465.5	0.672897196	465.5	0.666666667	465.5	1	2	21.57544901	21.57544901	21.57544901
435.5	0.672897196	435.5	0.666666667	435.5	1	6	20.86863675	20.86863675	20.86863675
421.5	0.687943262	421.5	0.666666667	421.5	1	10	20.53046517	20.53046517	20.53046517
1085	0.672897196	1085	0.666666667	1085	1	14	32.93933818	32.93933818	32.93933818
945	0.672897196	945	0.666666667	945	1	18	30.7408523	30.7408523	30.7408523
821	0.672897196	821	0.666666667	821	1	22	28.65309756	28.65309756	28.65309756
713	0.672897196	713	0.666666667	713	1	26	26.70205985	26.70205985	26.70205985
621	0.672897196	621	0.666666667	621	1	30	24.91987159	24.91987159	24.91987159
545	0.672897196	545	0.666666667	545	1	34	23.34523506	23.34523506	23.34523506
485	0.672897196	485	0.666666667	485	1	38	22.02271555	22.02271555	22.02271555
441	0.672897196	441	0.666666667	441	1	42	21	21	21
413	0.672897196	413	0.666666667	413	1	46	20.32240143	20.32240143	20.32240143
1084.5	0.672897196	1084.5	0.666666667	1084.5	1	2	32.9317476	32.9317476	32.9317476
942.5	0.672897196	942.5	0.666666667	942.5	1	6	30.70016287	30.70016287	30.70016287
816.5	0.672897196	816.5	0.666666667	816.5	1	10	28.57446412	28.57446412	28.57446412
706.5	0.672897196	706.5	0.666666667	706.5	1	14	26.58006772	26.58006772	26.58006772
612.5	0.672897196	612.5	0.666666667	612.5	1	18	24.74873734	24.74873734	24.74873734
534.5	0.672897196	534.5	0.666666667	534.5	1	22	23.11925604	23.11925604	23.11925604
472.5	0.672897196	472.5	0.666666667	472.5	1	26	21.73706512	21.73706512	21.73706512
426.5	0.672897196	426.5	0.666666667	426.5	1	30	20.65187643	20.65187643	20.65187643
396.5	0.672897196	396.5	0.666666667	396.5	1	34	19.91230775	19.91230775	19.91230775
382.5	0.695652174	382.5	0.666666667	382.5	1	38	19.55760722	19.55760722	19.55760722
941	0.672897196	941	0.666666667	941	1	42	30.6757233	30.6757233	30.6757233
813	0.672897196	813	0.666666667	813	1	46	28.51315486	28.51315486	28.51315486
651	0.672897196	651	0.666666667	651	1	2	25.51470164	25.51470164	25.51470164
563	0.672897196	563	0.666666667	563	1	6	23.72762104	23.72762104	23.72762104
491	0.672897196	491	0.666666667	491	1	10	22.15851981	22.15851981	22.15851981
435	0.672897196	435	0.666666667	435	1	14	20.85665361	20.85665361	20.85665361
395	0.672897196	395	0.666666667	395	1	18	19.87460691	19.87460691	19.87460691
371	0.680555556	371	0.666666667	371	1	22	19.26136028	19.26136028	19.26136028
363	0.712121212	363	0.666666667	363	1	26	19.05255888	19.05255888	19.05255888
841.5	0.672897196	841.5	0.666666667	841.5	1	30	29.00861941	29.00861941	29.00861941
723.5	0.672897196	723.5	0.666666667	723.5	1	34	26.89795531	26.89795531	26.89795531
621.5	0.672897196	621.5	0.666666667	621.5	1	38	24.92990172	24.92990172	24.92990172
535.5	0.672897196	535.5	0.666666667	535.5	1	42	23.14087293	23.14087293	23.14087293
465.5	0.672897196	465.5	0.666666667	465.5	1	46	21.57544901	21.57544901	21.57544901
390.5	0.672897196	390.5	0.666666667	390.5	1	2	19.76107285	19.76107285	19.76107285
360.5	0.673469388	360.5	0.666666667	360.5	1	6	18.98683755	18.98683755	18.98683755
346.5	0.703703704	346.5	0.666666667	346.5	1	10	18.61451047	18.61451047	18.61451047
809	0.672897196	809	0.666666667	809	1	14	28.44292531	28.44292531	28.44292531
693	0.672897196	693	0.666666667	693	1	18	26.32489316	26.32489316	26.32489316
593	0.672897196	593	0.666666667	593	1	22	24.35159132	24.35159132	24.35159132
509	0.672897196	509	0.666666667	509	1	26	22.56102835	22.56102835	22.56102835
441	0.672897196	441	0.666666667	441	1	30	21	21	21
389	0.672897196	389	0.666666667	389	1	34	19.72308292	19.72308292	19.72308292
353	0.672897196	353	0.666666667	353	1	38	18.78829423	18.78829423	18.78829423
333	0.695652174	333	0.666666667	333	1	42	18.24828759	18.24828759	18.24828759
808.5	0.672897196	808.5	0.666666667	808.5	1	46	28.43413442	28.43413442	28.43413442
637.5	0.672897196	637.5	0.666666667	637.5	1	2	25.24876235	25.24876235	25.24876235
543.5	0.672897196	543.5	0.666666667	543.5	1	6	23.31308645	23.31308645	23.31308645
465.5	0.672897196	465.5	0.666666667	465.5	1	10	21.57544901	21.57544901	21.57544901
403.5	0.672897196	403.5	0.666666667	403.5	1	14	20.08730943	20.08730943	20.08730943
357.5	0.672897196	357.5	0.666666667	357.5	1	18	18.9076704	18.9076704	18.9076704
327.5	0.680555556	327.5	0.666666667	327.5	1	22	18.09696107	18.09696107	18.09696107
313.5	0.712121212	313.5	0.666666667	313.5	1	26	17.70593121	17.70593121	17.70593121
689	0.673913043	689	0.666666667	689	1	30	26.2488095	26.2488095	26.2488095
585	0.673913043	585	0.666666667	585	1	34	24.18677324	24.18677324	24.18677324
497	0.673913043	497	0.666666667	497	1	38	22.29349681	22.29349681	22.29349681
425	0.673913043	425	0.666666667	425	1	42	20.61552813	20.61552813	20.61552813
369	0.673913043	369	0.666666667	369	1	46	19.20937271	19.20937271	19.20937271
315	0.680555556	315	0.666666667	315	1	2	17.74823935	17.74823935	17.74823935
299	0.712121212	301.5	0.666666667	301.5	1	6	17.29161647	17.36375535	17.36375535
660.5	0.677419355	688.5	0.666666667	688.5	1	10	25.70019455	26.23928353	26.23928353
558.5	0.677419355	582.5	0.666666667	582.5	1	14	23.6326046	24.13503677	24.13503677
472.5	0.677419355	492.5	0.666666667	492.5	1	18	21.73706512	22.19234102	22.19234102
402.5	0.677419355	418.5	0.666666667	418.5	1	22	20.06240265	20.45727255	20.45727255
348.5	0.677419355	360.5	0.666666667	360.5	1	26	18.6681547	18.98683755	18.98683755
310.5	0.677419355	318.5	0.666666667	318.5	1	30	17.62101019	17.8465683	17.8465683
288.5	0.703703704	292.5	0.666666667	292.5	1	34	16.98528775	17.10263138	17.10263138
633	0.680851064	282.5	0.666666667	282.5	1	38	25.15949125	16.80773631	16.80773631
533	0.680851064	556.5	0.666666667	556.5	1	42	23.08679276	23.59025222	23.59025222
449	0.680851064	468.5	0.666666667	468.5	1	46	21.1896201	21.64486082	21.64486082
353	0.680851064	366.5	0.666666667	366.5	1	2	18.78829423	19.14418972	19.14418972
309	0.680851064	318.5	0.666666667	318.5	1	6	17.57839583	17.8465683	17.8465683
281	0.695652174	286.5	0.666666667	286.5	1	10	16.76305461	16.92631088	16.92631088
269	0.73015873	270.5	0.666666667	270.5	1	14	16.40121947	16.4468842	16.4468842
531.5	0.686015831	555.5	0.666666667	555.5	1	18	23.05428377	23.5690475	23.5690475
445.5	0.686015831	465.5	0.666666667	465.5	1	22	21.10687092	21.57544901	21.57544901
375.5	0.686015831	391.5	0.666666667	391.5	1	26	19.37782238	19.78635894	19.78635894
321.5	0.686015831	333.5	0.666666667	333.5	1	30	17.93042108	18.26198237	18.26198237
283.5	0.686015831	291.5	0.666666667	291.5	1	34	16.83745824	17.07337108	17.07337108
261.5	0.712121212	265.5	0.666666667	265.5	1	38	16.17096163	16.29417074	16.29417074
531	0.686015831	255.5	0.666666667	255.5	1	42	23.04343724	15.98436736	15.98436736
443	0.686015831	463.5	0.666666667	463.5	1	46	21.04756518	21.52905014	21.52905014
341	0.686015831	355.5	0.666666667	355.5	1	2	18.46618531	18.85470763	18.85470763
293	0.686015831	303.5	0.666666667	303.5	1	6	17.11724277	17.42125139	17.42125139
261	0.695652174	267.5	0.666666667	267.5	1	10	16.15549442	16.35542723	16.35542723
245	0.73015873	247.5	0.666666667	247.5	1	14	15.65247584	15.73213272	15.73213272
462.5	0.686015831	484.5	0.666666667	484.5	1	18	21.50581317	22.0113607	22.0113607
384.5	0.686015831	402.5	0.666666667	402.5	1	22	19.60867155	20.06240265	20.06240265
322.5	0.686015831	336.5	0.666666667	336.5	1	26	17.958285	18.34393633	18.34393633
276.5	0.686015831	286.5	0.666666667	286.5	1	30	16.62828915	16.92631088	16.92631088
246.5	0.703703704	252.5	0.666666667	252.5	1	34	15.70031847	15.89024858	15.89024858
232.5	0.739837398	234.5	0.666666667	234.5	1	38	15.24795068	15.31339283	15.31339283
401	0.686015831	420.5	0.666666667	420.5	1	42	20.02498439	20.50609665	20.50609665
333	0.686015831	348.5	0.666666667	348.5	1	46	18.24828759	18.6681547	18.6681547
261	0.686015831	270.5	0.666666667	270.5	1	2	16.15549442	16.4468842	16.4468842
233	0.712121212	238.5	0.666666667	238.5	1	6	15.26433752	15.44344521	15.44344521
221	0.75	222.5	0.666666667	222.5	1	10	14.86606875	14.91643389	14.91643389
363.5	0.686015831	381.5	0.666666667	381.5	1	14	19.06567596	19.53202498	19.53202498
301.5	0.686015831	315.5	0.666666667	315.5	1	18	17.36375535	17.76231967	17.76231967
255.5	0.686015831	265.5	0.666666667	265.5	1	22	15.98436736	16.29417074	16.29417074
225.5	0.712121212	231.5	0.666666667	231.5	1	26	15.01665742	15.21512405	15.21512405
211.5	0.75	213.5	0.666666667	213.5	1	30	14.54303957	14.6116392	14.6116392
329	0.686015831	345.5	0.666666667	345.5	1	34	18.13835715	18.5876303	18.5876303
273	0.686015831	285.5	0.666666667	285.5	1	38	16.52271164	16.89674525	16.89674525
233	0.695652174	241.5	0.666666667	241.5	1	42	15.26433752	15.54027027	15.54027027
209	0.73015873	213.5	0.666666667	213.5	1	46	14.45683229	14.6116392	14.6116392
312.5	0.686015831	328.5	0.666666667	328.5	1	2	17.67766953	18.12456896	18.12456896
258.5	0.686015831	270.5	0.666666667	270.5	1	6	16.07793519	16.4468842	16.4468842
220.5	0.703703704	228.5	0.666666667	228.5	1	10	14.8492424	15.11621646	15.11621646
198.5	0.739837398	202.5	0.666666667	202.5	1	14	14.0890028	14.23024947	14.23024947
297	0.686015831	192.5	0.666666667	192.5	1	18	17.23368794	13.87443693	13.87443693
245	0.686015831	256.5	0.666666667	256.5	1	22	15.65247584	16.01561738	16.01561738
209	0.712121212	216.5	0.666666667	216.5	1	26	14.45683229	14.71393897	14.71393897
189	0.75	192.5	0.666666667	192.5	1	30	13.74772708	13.87443693	13.87443693
268.5	0.686015831	184.5	0.666666667	184.5	1	34	16.38596961	13.58307771	13.58307771
222.5	0.695652174	232.5	0.666666667	232.5	1	38	14.91643389	15.24795068	15.24795068
192.5	0.73015873	198.5	0.666666667	198.5	1	42	13.87443693	14.0890028	14.0890028
178.5	0.771929825	180.5	0.666666667	180.5	1	46	13.36038922	13.43502884	13.43502884
203	0.712121212	211.5	0.666666667	211.5	1	2	14.24780685	14.54303957	14.54303957
179	0.75	183.5	0.666666667	183.5	1	6	13.37908816	13.54621718	13.54621718
171	0.796296296	171.5	0.666666667	171.5	1	10	13.07669683	13.09580085	13.09580085
193.5	0.720930233	201.5	0.666666667	201.5	1	14	13.91042774	14.19506957	14.19506957
171.5	0.760683761	175.5	0.666666667	175.5	1	18	13.09580085	13.2476413	13.2476413
201	0.712121212	165.5	0.666666667	165.5	1	22	14.17744688	12.86468033	12.86468033
173	0.75	178.5	0.666666667	178.5	1	26	13.15294644	13.36038922	13.36038922
161	0.796296296	162.5	0.666666667	162.5	1	30	12.68857754	12.74754878	12.74754878
171.5	0.75	177.5	0.666666667	177.5	1	34	13.09580085	13.32291259	13.32291259
157.5	0.796296296	159.5	0.666666667	159.5	1	38	12.5499004	12.62933094	12.62933094
161	0.771929825	165.5	0.666666667	165.5	1	42	12.68857754	12.86468033	12.86468033
153	0.823529412	153.5	0.666666667	153.5	1	46	12.36931688	12.38951169	12.38951169
153	0.796296296	150.5	0.666666667	150.5	1	2	12.36931688	12.26784415	12.26784415
148.5	0.823529412	148.5	0.666666667	148.5	1	6	12.18605761	12.18605761	12.18605761
1160.5	0.676923077	1200	0.666666667	1200	1	10	34.06611219	34.64101615	34.64101615
1012.5	0.676923077	1048	0.666666667	1048	1	14	31.81980515	32.37282811	32.37282811
880.5	0.676923077	912	0.666666667	912	1	18	29.67322025	30.19933774	30.19933774
764.5	0.676923077	792	0.666666667	792	1	22	27.64959313	28.14249456	28.14249456
664.5	0.676923077	688	0.666666667	688	1	26	25.77789751	26.2297541	26.2297541
580.5	0.676923077	600	0.666666667	600	1	30	24.09356761	24.49489743	24.49489743
512.5	0.676923077	528	0.666666667	528	1	34	22.63846285	22.97825059	22.97825059
460.5	0.676923077	472	0.666666667	472	1	38	21.45926373	21.72556098	21.72556098
424.5	0.676923077	432	0.666666667	432	1	42	20.60339778	20.78460969	20.78460969
404.5	0.680555556	408	0.666666667	408	1	46	20.11218536	20.19900988	20.19900988
1046.5	0.676923077	1083.5	0.666666667	1083.5	1	2	32.34965224	32.91656118	32.91656118
908.5	0.676923077	941.5	0.666666667	941.5	1	6	30.14133375	30.68387199	30.68387199
786.5	0.676923077	815.5	0.666666667	815.5	1	10	28.04460732	28.55696062	28.55696062
680.5	0.676923077	705.5	0.666666667	705.5	1	14	26.08639492	26.56124997	26.56124997
590.5	0.676923077	611.5	0.666666667	611.5	1	18	24.30020576	24.72852604	24.72852604
516.5	0.676923077	533.5	0.666666667	533.5	1	22	22.72663635	23.09761892	23.09761892
458.5	0.676923077	471.5	0.666666667	471.5	1	26	21.41261311	21.71405075	21.71405075
416.5	0.676923077	425.5	0.666666667	425.5	1	30	20.40833163	20.62765134	20.62765134
390.5	0.676923077	395.5	0.666666667	395.5	1	34	19.76107285	19.8871818	19.8871818
380.5	0.703703704	381.5	0.666666667	381.5	1	38	19.5064092	19.53202498	19.53202498
939.5	0.676923077	974	0.666666667	974	1	42	30.65126425	31.20897307	31.20897307
811.5	0.676923077	842	0.666666667	842	1	46	28.48683907	29.01723626	29.01723626
649.5	0.676923077	674	0.666666667	674	1	2	25.48528987	25.96150997	25.96150997
561.5	0.676923077	582	0.666666667	582	1	6	23.69599122	24.12467616	24.12467616
489.5	0.676923077	506	0.666666667	506	1	10	22.12464689	22.49444376	22.49444376
433.5	0.676923077	446	0.666666667	446	1	14	20.82066281	21.11871208	21.11871208
393.5	0.676923077	402	0.666666667	402	1	18	19.83683442	20.04993766	20.04993766
369.5	0.680555556	374	0.666666667	374	1	22	19.22238279	19.33907961	19.33907961
361.5	0.712121212	362	0.666666667	362	1	26	19.01315334	19.02629759	19.02629759
871.5	0.676923077	904.5	0.666666667	904.5	1	30	29.52117884	30.07490648	30.07490648
749.5	0.676923077	778.5	0.666666667	778.5	1	34	27.37699764	27.90161286	27.90161286
643.5	0.676923077	668.5	0.666666667	668.5	1	38	25.36730179	25.85536695	25.85536695
553.5	0.676923077	574.5	0.666666667	574.5	1	42	23.52658071	23.96872963	23.96872963
479.5	0.676923077	496.5	0.666666667	496.5	1	46	21.89748844	22.28227996	22.28227996
398.5	0.676923077	409.5	0.666666667	409.5	1	2	19.96246478	20.23610634	20.23610634
364.5	0.676923077	371.5	0.666666667	371.5	1	6	19.09188309	19.27433527	19.27433527
346.5	0.695652174	349.5	0.666666667	349.5	1	10	18.61451047	18.6949191	18.6949191
870.5	0.676923077	904	0.666666667	904	1	14	29.50423698	30.06659276	30.06659276
746.5	0.676923077	776	0.666666667	776	1	18	27.32215218	27.85677655	27.85677655
638.5	0.676923077	664	0.666666667	664	1	22	25.26855754	25.76819745	25.76819745
546.5	0.676923077	568	0.666666667	568	1	26	23.37733946	23.83275058	23.83275058
470.5	0.676923077	488	0.666666667	488	1	30	21.69101196	22.09072203	22.09072203
410.5	0.676923077	424	0.666666667	424	1	34	20.26079959	20.59126028	20.59126028
366.5	0.676923077	376	0.666666667	376	1	38	19.14418972	19.39071943	19.39071943
338.5	0.680555556	344	0.666666667	344	1	42	18.39836949	18.54723699	18.54723699
326.5	0.712121212	328	0.666666667	328	1	46	18.069311	18.11077028	18.11077028
715.5	0.676923077	744.5	0.666666667	744.5	1	2	26.74883175	27.2855273	27.2855273
609.5	0.676923077	634.5	0.666666667	634.5	1	6	24.68805379	25.18928344	25.18928344
519.5	0.676923077	540.5	0.666666667	540.5	1	10	22.79254264	23.24865588	23.24865588
445.5	0.676923077	462.5	0.666666667	462.5	1	14	21.10687092	21.50581317	21.50581317
387.5	0.676923077	400.5	0.666666667	400.5	1	18	19.68501969	20.0124961	20.0124961
345.5	0.676923077	354.5	0.666666667	354.5	1	22	18.5876303	18.82817038	18.82817038
319.5	0.687943262	324.5	0.666666667	324.5	1	26	17.87456293	18.01388353	18.01388353
309.5	0.720930233	310.5	0.666666667	310.5	1	30	17.59261209	17.62101019	17.62101019
685.5	0.679665738	714	0.666666667	714	1	34	26.18205492	26.72077843	26.72077843
581.5	0.679665738	606	0.666666667	606	1	38	24.1143111	24.61706725	24.61706725
493.5	0.679665738	514	0.666666667	514	1	42	22.21485989	22.6715681	22.6715681
421.5	0.679665738	438	0.666666667	438	1	46	20.53046517	20.92844954	20.92844954
343.5	0.679665738	354	0.666666667	354	1	2	18.53375299	18.81488772	18.81488772
311.5	0.680555556	318	0.666666667	318	1	6	17.64936259	17.8325545	17.8325545
295.5	0.712121212	298	0.666666667	298	1	10	17.19011344	17.2626765	17.2626765
684.5	0.681318681	713.5	0.666666667	713.5	1	14	26.1629509	26.71142078	26.71142078
578.5	0.681318681	603.5	0.666666667	603.5	1	18	24.05202694	24.56623699	24.56623699
488.5	0.681318681	509.5	0.666666667	509.5	1	22	22.10203611	22.57210668	22.57210668
414.5	0.681318681	431.5	0.666666667	431.5	1	26	20.35927307	20.77257808	20.77257808
356.5	0.681318681	369.5	0.666666667	369.5	1	30	18.88120759	19.22238279	19.22238279
314.5	0.681318681	323.5	0.666666667	323.5	1	34	17.73414785	17.98610575	17.98610575
288.5	0.695652174	293.5	0.666666667	293.5	1	38	16.98528775	17.1318417	17.1318417
278.5	0.73015873	279.5	0.666666667	279.5	1	42	16.68831927	16.7182535	16.7182535
576.5	0.684782609	602	0.666666667	602	1	46	24.01041441	24.53568829	24.53568829
444.5	0.684782609	464	0.666666667	464	1	2	21.08316864	21.54065923	21.54065923
376.5	0.684782609	392	0.666666667	392	1	6	19.40360791	19.79898987	19.79898987
324.5	0.684782609	336	0.666666667	336	1	10	18.01388353	18.33030278	18.33030278
288.5	0.684782609	296	0.666666667	296	1	14	16.98528775	17.20465053	17.20465053
268.5	0.712121212	272	0.666666667	272	1	18	16.38596961	16.4924225	16.4924225
601.5	0.688172043	264	0.666666667	264	1	22	24.52549694	16.24807681	16.24807681
503.5	0.688172043	526.5	0.666666667	526.5	1	26	22.43880567	22.94558781	22.94558781
421.5	0.688172043	440.5	0.666666667	440.5	1	30	20.53046517	20.98809186	20.98809186
355.5	0.688172043	370.5	0.666666667	370.5	1	34	18.85470763	19.24837655	19.24837655
305.5	0.688172043	316.5	0.666666667	316.5	1	38	17.47855829	17.79044687	17.79044687
271.5	0.688172043	278.5	0.666666667	278.5	1	42	16.47725705	16.68831927	16.68831927
253.5	0.720930233	256.5	0.666666667	256.5	1	46	15.92168333	16.01561738	16.01561738
479.5	0.693333333	502	0.666666667	502	1	2	21.89748844	22.4053565	22.4053565
399.5	0.693333333	418	0.666666667	418	1	6	19.98749609	20.4450483	20.4450483
335.5	0.693333333	350	0.666666667	350	1	10	18.31665908	18.70828693	18.70828693
287.5	0.693333333	298	0.666666667	298	1	14	16.95582496	17.2626765	17.2626765
255.5	0.695652174	262	0.666666667	262	1	18	15.98436736	16.18641406	16.18641406
239.5	0.73015873	242	0.666666667	242	1	22	15.47578754	15.55634919	15.55634919
478.5	0.693333333	501.5	0.666666667	501.5	1	26	21.87464285	22.39419568	22.39419568
396.5	0.693333333	415.5	0.666666667	415.5	1	30	19.91230775	20.38381711	20.38381711
330.5	0.693333333	345.5	0.666666667	345.5	1	34	18.17965896	18.5876303	18.5876303
280.5	0.693333333	291.5	0.666666667	291.5	1	38	16.74813422	17.07337108	17.07337108
246.5	0.695652174	253.5	0.666666667	253.5	1	42	15.70031847	15.92168333	15.92168333
228.5	0.73015873	231.5	0.666666667	231.5	1	46	15.11621646	15.21512405	15.21512405
394.5	0.693333333	414	0.666666667	414	1	2	19.86202407	20.34698995	20.34698995
326.5	0.693333333	342	0.666666667	342	1	6	18.069311	18.49324201	18.49324201
274.5	0.693333333	286	0.666666667	286	1	10	16.56804153	16.91153453	16.91153453
238.5	0.695652174	246	0.666666667	246	1	14	15.44344521	15.68438714	15.68438714
218.5	0.73015873	222	0.666666667	222	1	18	14.7817455	14.89966443	14.89966443
413.5	0.693333333	214	0.666666667	214	1	22	20.33469941	14.62873884	14.62873884
339.5	0.693333333	356.5	0.666666667	356.5	1	26	18.42552577	18.88120759	18.88120759
281.5	0.693333333	294.5	0.666666667	294.5	1	30	16.77796174	17.1610023	17.1610023
239.5	0.693333333	248.5	0.666666667	248.5	1	34	15.47578754	15.76388277	15.76388277
213.5	0.720930233	218.5	0.666666667	218.5	1	38	14.6116392	14.7817455	14.7817455
203.5	0.760683761	204.5	0.666666667	204.5	1	42	14.26534262	14.30034965	14.30034965
321.5	0.693333333	338	0.666666667	338	1	46	17.93042108	18.38477631	18.38477631
243.5	0.693333333	254	0.666666667	254	1	2	15.60448653	15.93737745	15.93737745
211.5	0.712121212	218	0.666666667	218	1	6	14.54303957	14.76482306	14.76482306
195.5	0.75	198	0.666666667	198	1	10	13.98213145	14.07124728	14.07124728
320.5	0.693333333	337.5	0.666666667	337.5	1	14	17.90251379	18.37117307	18.37117307
262.5	0.693333333	275.5	0.666666667	275.5	1	18	16.20185175	16.59819267	16.59819267
220.5	0.695652174	229.5	0.666666667	229.5	1	22	14.8492424	15.14925741	15.14925741
194.5	0.73015873	199.5	0.666666667	199.5	1	26	13.94632568	14.12444689	14.12444689
184.5	0.771929825	185.5	0.666666667	185.5	1	30	13.58307771	13.61983847	13.61983847
260.5	0.693333333	274	0.666666667	274	1	34	16.14001239	16.55294536	16.55294536
216.5	0.695652174	226	0.666666667	226	1	38	14.71393897	15.03329638	15.03329638
188.5	0.73015873	194	0.666666667	194	1	42	13.72953022	13.92838828	13.92838828
176.5	0.771929825	178	0.666666667	178	1	46	13.28533026	13.34166406	13.34166406
223.5	0.693333333	234.5	0.666666667	234.5	1	2	14.94991639	15.31339283	15.31339283
189.5	0.720930233	196.5	0.666666667	196.5	1	6	13.7658999	14.01784577	14.01784577
171.5	0.760683761	174.5	0.666666667	174.5	1	10	13.09580085	13.20984481	13.20984481
233.5	0.693333333	246	0.666666667	246	1	14	15.28070679	15.68438714	15.68438714
193.5	0.712121212	202	0.666666667	202	1	18	13.91042774	14.2126704	14.2126704
169.5	0.75	174	0.666666667	174	1	22	13.01921657	13.19090596	13.19090596
161.5	0.796296296	162	0.666666667	162	1	26	12.70826503	12.72792206	12.72792206
191.5	0.712121212	200.5	0.666666667	200.5	1	30	13.8383525	14.15980226	14.15980226
165.5	0.75	170.5	0.666666667	170.5	1	34	12.86468033	13.05756486	13.05756486
155.5	0.796296296	156.5	0.666666667	156.5	1	38	12.46996391	12.509996	12.509996
174.5	0.73015873	182	0.666666667	182	1	42	13.20984481	13.49073756	13.49073756
154.5	0.771929825	158	0.666666667	158	1	46	12.42980289	12.56980509	12.56980509
166.5	0.739837398	173.5	0.666666667	173.5	1	2	12.9034879	13.17193987	13.17193987
148.5	0.783783784	151.5	0.666666667	151.5	1	6	12.18605761	12.30853363	12.30853363
159.5	0.75	166	0.666666667	166	1	10	12.62933094	12.88409873	12.88409873
143.5	0.796296296	146	0.666666667	146	1	14	11.97914855	12.08304597	12.08304597
148.5	0.771929825	153.5	0.666666667	153.5	1	18	12.18605761	12.38951169	12.38951169
138.5	0.823529412	139.5	0.666666667	139.5	1	22	11.7686023	11.81101181	11.81101181
136.5	0.823529412	138	0.666666667	138	1	26	11.68332145	11.74734012	11.74734012
134.5	0.838383838	135.5	0.666666667	135.5	1	30	11.5974135	11.64044673	11.64044673
1045.5	0.682926829	1083	0.666666667	1083	1	34	32.33419243	32.90896534	32.90896534
905.5	0.682926829	939	0.666666667	939	1	38	30.09152705	30.64310689	30.64310689
781.5	0.682926829	811	0.666666667	811	1	42	27.9553215	28.47806173	28.47806173
673.5	0.682926829	699	0.666666667	699	1	46	25.95187854	26.43860813	26.43860813
541.5	0.682926829	561	0.666666667	561	1	2	23.27015256	23.68543856	23.68543856
473.5	0.682926829	489	0.666666667	489	1	6	21.76005515	22.11334439	22.11334439
421.5	0.682926829	433	0.666666667	433	1	10	20.53046517	20.80865205	20.80865205
385.5	0.682926829	393	0.666666667	393	1	14	19.63415392	19.8242276	19.8242276
365.5	0.687943262	369	0.666666667	369	1	18	19.11805429	19.20937271	19.20937271
1008.5	0.682926829	361	0.666666667	361	1	22	31.75688902	19	19
870.5	0.682926829	903.5	0.666666667	903.5	1	26	29.50423698	30.05827673	30.05827673
748.5	0.682926829	777.5	0.666666667	777.5	1	30	27.35872804	27.88368699	27.88368699
642.5	0.682926829	667.5	0.666666667	667.5	1	34	25.34758371	25.83602137	25.83602137
552.5	0.682926829	573.5	0.666666667	573.5	1	38	23.50531855	23.94786003	23.94786003
478.5	0.682926829	495.5	0.666666667	495.5	1	42	21.87464285	22.25982929	22.25982929
420.5	0.682926829	433.5	0.666666667	433.5	1	46	20.50609665	20.82066281	20.82066281
363.5	0.682926829	370.5	0.666666667	370.5	1	2	19.06567596	19.24837655	19.24837655
345.5	0.695652174	348.5	0.666666667	348.5	1	6	18.5876303	18.6681547	18.6681547
902.5	0.682926829	937	0.666666667	937	1	10	30.04163777	30.61045573	30.61045573
774.5	0.682926829	805	0.666666667	805	1	14	27.8298401	28.37252192	28.37252192
662.5	0.682926829	689	0.666666667	689	1	18	25.73907535	26.2488095	26.2488095
566.5	0.682926829	589	0.666666667	589	1	22	23.80126047	24.2693222	24.2693222
486.5	0.682926829	505	0.666666667	505	1	26	22.056745	22.47220505	22.47220505
422.5	0.682926829	437	0.666666667	437	1	30	20.55480479	20.90454496	20.90454496
374.5	0.682926829	385	0.666666667	385	1	34	19.35200248	19.62141687	19.62141687
342.5	0.682926829	349	0.666666667	349	1	38	18.50675552	18.68154169	18.68154169
326.5	0.703703704	329	0.666666667	329	1	42	18.069311	18.13835715	18.13835715
835.5	0.682926829	868.5	0.666666667	868.5	1	46	28.90501687	29.47032406	29.47032406
658.5	0.682926829	685.5	0.666666667	685.5	1	2	25.66125484	26.18205492	26.18205492
560.5	0.682926829	583.5	0.666666667	583.5	1	6	23.6748812	24.15574466	24.15574466
478.5	0.682926829	497.5	0.666666667	497.5	1	10	21.87464285	22.30470802	22.30470802
412.5	0.682926829	427.5	0.666666667	427.5	1	14	20.31009601	20.67607313	20.67607313
362.5	0.682926829	373.5	0.666666667	373.5	1	18	19.03943276	19.32614809	19.32614809
328.5	0.682926829	335.5	0.666666667	335.5	1	22	18.12456896	18.31665908	18.31665908
310.5	0.703703704	313.5	0.666666667	313.5	1	26	17.62101019	17.70593121	17.70593121
771.5	0.682926829	803	0.666666667	803	1	30	27.77588882	28.33725463	28.33725463
655.5	0.682926829	683	0.666666667	683	1	34	25.60273423	26.13426869	26.13426869
555.5	0.682926829	579	0.666666667	579	1	38	23.5690475	24.06241883	24.06241883
471.5	0.682926829	491	0.666666667	491	1	42	21.71405075	22.15851981	22.15851981
403.5	0.682926829	419	0.666666667	419	1	46	20.08730943	20.46948949	20.46948949
331.5	0.682926829	341	0.666666667	341	1	2	18.20714146	18.46618531	18.46618531
303.5	0.687943262	309	0.666666667	309	1	6	17.42125139	17.57839583	17.57839583
291.5	0.720930233	293	0.666666667	293	1	10	17.07337108	17.11724277	17.11724277
681.5	0.685393258	710.5	0.666666667	710.5	1	14	26.10555496	26.65520587	26.65520587
575.5	0.685393258	600.5	0.666666667	600.5	1	18	23.98958107	24.50510151	24.50510151
485.5	0.685393258	506.5	0.666666667	506.5	1	22	22.03406454	22.50555487	22.50555487
411.5	0.685393258	428.5	0.666666667	428.5	1	26	20.28546278	20.70024154	20.70024154
353.5	0.685393258	366.5	0.666666667	366.5	1	30	18.80159568	19.14418972	19.14418972
311.5	0.685393258	320.5	0.666666667	320.5	1	34	17.64936259	17.90251379	17.90251379
285.5	0.695652174	290.5	0.666666667	290.5	1	38	16.89674525	17.04406055	17.04406055
275.5	0.73015873	276.5	0.666666667	276.5	1	42	16.59819267	16.62828915	16.62828915
598.5	0.688888889	625	0.666666667	625	1	46	24.46425965	25	25
460.5	0.688888889	481	0.666666667	481	1	2	21.45926373	21.9317122	21.9317122
388.5	0.688888889	405	0.666666667	405	1	6	19.71040334	20.1246118	20.1246118
332.5	0.688888889	345	0.666666667	345	1	10	18.23458253	18.57417562	18.57417562
292.5	0.688888889	301	0.666666667	301	1	14	17.10263138	17.34935157	17.34935157
268.5	0.703703704	273	0.666666667	273	1	18	16.38596961	16.52271164	16.52271164
260.5	0.739837398	261	0.666666667	261	1	22	16.14001239	16.15549442	16.15549442
546.5	0.692307692	571.5	0.666666667	571.5	1	26	23.37733946	23.90606618	23.90606618
456.5	0.692307692	477.5	0.666666667	477.5	1	30	21.36586062	21.85177338	21.85177338
382.5	0.692307692	399.5	0.666666667	399.5	1	34	19.55760722	19.98749609	19.98749609
324.5	0.692307692	337.5	0.666666667	337.5	1	38	18.01388353	18.37117307	18.37117307
282.5	0.692307692	291.5	0.666666667	291.5	1	42	16.80773631	17.07337108	17.07337108
256.5	0.703703704	261.5	0.666666667	261.5	1	46	16.01561738	16.17096163	16.17096163
545.5	0.695652174	571	0.666666667	571	1	2	23.35594143	23.89560629	23.89560629
453.5	0.695652174	475	0.666666667	475	1	6	21.29553944	21.79449472	21.79449472
377.5	0.695652174	395	0.666666667	395	1	10	19.42935923	19.87460691	19.87460691
317.5	0.695652174	331	0.666666667	331	1	14	17.81852968	18.1934054	18.1934054
273.5	0.695652174	283	0.666666667	283	1	18	16.53783541	16.82260384	16.82260384
251	0.695652174	251	0.666666667	251	1	22	15.84297952	15.84297952	15.84297952
235	0.73015873	237.5	0.666666667	237.5	1	26	15.32970972	15.41103501	15.41103501
496.5	0.695652174	520.5	0.666666667	520.5	1	30	22.28227996	22.81446909	22.81446909
410.5	0.695652174	430.5	0.666666667	430.5	1	34	20.26079959	20.74849392	20.74849392
340.5	0.695652174	356.5	0.666666667	356.5	1	38	18.45264209	18.88120759	18.88120759
286.5	0.695652174	298.5	0.666666667	298.5	1	42	16.92631088	17.27715254	17.27715254
248.5	0.695652174	256.5	0.666666667	256.5	1	46	15.76388277	16.01561738	16.01561738
223.5	0.73015873	226.5	0.666666667	226.5	1	2	14.94991639	15.04991694	15.04991694
450.5	0.695652174	473	0.666666667	473	1	6	21.22498528	21.74856317	21.74856317
370.5	0.695652174	389	0.666666667	389	1	10	19.24837655	19.72308292	19.72308292
306.5	0.695652174	321	0.666666667	321	1	14	17.5071414	17.91647287	17.91647287
258.5	0.695652174	269	0.666666667	269	1	18	16.07793519	16.40121947	16.40121947
233	0.695652174	233	0.666666667	233	1	22	15.26433752	15.26433752	15.26433752
213	0.73015873	216.5	0.666666667	216.5	1	26	14.59451952	14.71393897	14.71393897
428.5	0.695652174	208.5	0.666666667	208.5	1	30	20.70024154	14.43952908	14.43952908
350.5	0.695652174	368.5	0.666666667	368.5	1	34	18.72164523	19.19635382	19.19635382
288.5	0.695652174	302.5	0.666666667	302.5	1	38	16.98528775	17.39252713	17.39252713
242.5	0.695652174	252.5	0.666666667	252.5	1	42	15.5724115	15.89024858	15.89024858
218.5	0.703703704	225.5	0.666666667	225.5	1	46	14.7817455	15.01665742	15.01665742
197.5	0.760683761	198.5	0.666666667	198.5	1	2	14.05346932	14.0890028	14.0890028
331.5	0.695652174	349	0.666666667	349	1	6	18.20714146	18.68154169	18.68154169
271.5	0.695652174	285	0.666666667	285	1	10	16.47725705	16.88194302	16.88194302
227.5	0.695652174	237	0.666666667	237	1	14	15.08310313	15.39480432	15.39480432
205	0.712121212	211.5	0.666666667	211.5	1	18	14.31782106	14.54303957	14.54303957
189	0.75	191.5	0.666666667	191.5	1	22	13.74772708	13.8383525	13.8383525
330.5	0.695652174	348.5	0.666666667	348.5	1	26	18.17965896	18.6681547	18.6681547
268.5	0.695652174	282.5	0.666666667	282.5	1	30	16.38596961	16.80773631	16.80773631
222.5	0.695652174	232.5	0.666666667	232.5	1	34	14.91643389	15.24795068	15.24795068
198.5	0.712121212	205.5	0.666666667	205.5	1	38	14.0890028	14.33527119	14.33527119
180.5	0.75	183.5	0.666666667	183.5	1	42	13.43502884	13.54621718	13.54621718
296.5	0.695652174	313	0.666666667	313	1	46	17.21917536	17.69180601	17.69180601
218.5	0.695652174	229	0.666666667	229	1	2	14.7817455	15.13274595	15.13274595
193	0.712121212	200.5	0.666666667	200.5	1	6	13.89244399	14.15980226	14.15980226
173	0.75	176.5	0.666666667	176.5	1	10	13.15294644	13.28533026	13.28533026
280.5	0.695652174	168.5	0.666666667	168.5	1	14	16.74813422	12.98075499	12.98075499
226.5	0.695652174	238.5	0.666666667	238.5	1	18	15.04991694	15.44344521	15.44344521
196.5	0.703703704	205.5	0.666666667	205.5	1	22	14.01784577	14.33527119	14.33527119
170.5	0.739837398	175.5	0.666666667	175.5	1	26	13.05756486	13.2476413	13.2476413
160.5	0.783783784	161.5	0.666666667	161.5	1	30	12.66885946	12.70826503	12.70826503
213.5	0.695652174	225	0.666666667	225	1	34	14.6116392	15	15
185	0.712121212	193.5	0.666666667	193.5	1	38	13.60147051	13.91042774	13.91042774
161	0.75	165.5	0.666666667	165.5	1	42	12.68857754	12.86468033	12.86468033
153	0.796296296	153.5	0.666666667	153.5	1	46	12.36931688	12.38951169	12.38951169
182.5	0.712121212	191.5	0.666666667	191.5	1	2	13.50925609	13.8383525	13.8383525
156.5	0.75	161.5	0.666666667	161.5	1	6	12.509996	12.70826503	12.70826503
146.5	0.796296296	147.5	0.666666667	147.5	1	10	12.10371844	12.1449578	12.1449578
181	0.712121212	190.5	0.666666667	190.5	1	14	13.45362405	13.80217374	13.80217374
153	0.75	158.5	0.666666667	158.5	1	18	12.36931688	12.58967831	12.58967831
141	0.796296296	142.5	0.666666667	142.5	1	22	11.87434209	11.93733639	11.93733639
163.5	0.73015873	171.5	0.666666667	171.5	1	26	12.78671185	13.09580085	13.09580085
141.5	0.771929825	145.5	0.666666667	145.5	1	30	11.89537725	12.06233808	12.06233808
163	0.73015873	135.5	0.666666667	135.5	1	34	12.76714533	11.64044673	11.64044673
139	0.771929825	143.5	0.666666667	143.5	1	38	11.78982612	11.97914855	11.97914855
131	0.823529412	131.5	0.666666667	131.5	1	42	11.44552314	11.46734494	11.46734494
133.5	0.783783784	137.5	0.666666667	137.5	1	46	11.55422001	11.7260394	11.7260394
129	0.796296296	132.5	0.666666667	132.5	1	2	11.35781669	11.51086443	11.51086443
128.5	0.796296296	124.5	0.666666667	124.5	1	6	11.33578405	11.1579568	11.1579568
123	0.823529412	122.5	0.666666667	122.5	1	10	11.09053651	11.06797181	11.06797181
972	0.688821752	120.5	0.666666667	120.5	1	14	31.17691454	10.9772492	10.9772492
836	0.688821752	868.5	0.666666667	868.5	1	18	28.91366459	29.47032406	29.47032406
716	0.688821752	744.5	0.666666667	744.5	1	22	26.75817632	27.2855273	27.2855273
612	0.688821752	636.5	0.666666667	636.5	1	26	24.73863375	25.22895162	25.22895162
524	0.688821752	544.5	0.666666667	544.5	1	30	22.89104628	23.33452378	23.33452378
452	0.688821752	468.5	0.666666667	468.5	1	34	21.26029163	21.64486082	21.64486082
396	0.688821752	408.5	0.666666667	408.5	1	38	19.89974874	20.21138293	20.21138293
356	0.688821752	364.5	0.666666667	364.5	1	42	18.86796226	19.09188309	19.09188309
332	0.688821752	336.5	0.666666667	336.5	1	46	18.22086716	18.34393633	18.34393633
867.5	0.688821752	901.5	0.666666667	901.5	1	2	29.45335295	30.02498959	30.02498959
741.5	0.688821752	771.5	0.666666667	771.5	1	6	27.23049761	27.77588882	27.77588882
631.5	0.688821752	657.5	0.666666667	657.5	1	10	25.12966375	25.64176281	25.64176281
537.5	0.688821752	559.5	0.666666667	559.5	1	14	23.18404624	23.65375235	23.65375235
459.5	0.688821752	477.5	0.666666667	477.5	1	18	21.43595111	21.85177338	21.85177338
397.5	0.688821752	411.5	0.666666667	411.5	1	22	19.93740204	20.28546278	20.28546278
351.5	0.688821752	361.5	0.666666667	361.5	1	26	18.74833326	19.01315334	19.01315334
321.5	0.688821752	327.5	0.666666667	327.5	1	30	17.93042108	18.09696107	18.09696107
307.5	0.712121212	309.5	0.666666667	309.5	1	34	17.53567792	17.59261209	17.59261209
770	0.69005848	801.5	0.666666667	801.5	1	38	27.74887385	28.31077533	28.31077533
654	0.69005848	681.5	0.666666667	681.5	1	42	25.57342371	26.10555496	26.10555496
554	0.69005848	577.5	0.666666667	577.5	1	46	23.53720459	24.03122968	24.03122968
434	0.69005848	451.5	0.666666667	451.5	1	2	20.83266666	21.24852936	21.24852936
374	0.69005848	387.5	0.666666667	387.5	1	6	19.33907961	19.68501969	19.68501969
330	0.69005848	339.5	0.666666667	339.5	1	10	18.16590212	18.42552577	18.42552577
302	0.69005848	307.5	0.666666667	307.5	1	14	17.3781472	17.53567792	17.53567792
290	0.720930233	291.5	0.666666667	291.5	1	18	17.02938637	17.07337108	17.07337108
708.5	0.69005848	738.5	0.666666667	738.5	1	22	26.61766331	27.17535648	27.17535648
598.5	0.69005848	624.5	0.666666667	624.5	1	26	24.46425965	24.989998	24.989998
504.5	0.69005848	526.5	0.666666667	526.5	1	30	22.46107745	22.94558781	22.94558781
426.5	0.69005848	444.5	0.666666667	444.5	1	34	20.65187643	21.08316864	21.08316864
364.5	0.69005848	378.5	0.666666667	378.5	1	38	19.09188309	19.45507646	19.45507646
318.5	0.69005848	328.5	0.666666667	328.5	1	42	17.8465683	18.12456896	18.12456896
288.5	0.69005848	294.5	0.666666667	294.5	1	46	16.98528775	17.1610023	17.1610023
708	0.693181818	273.5	0.666666667	273.5	1	2	26.60826939	16.53783541	16.53783541
596	0.693181818	622.5	0.666666667	622.5	1	6	24.41311123	24.9499499	24.9499499
500	0.693181818	522.5	0.666666667	522.5	1	10	22.36067977	22.8582589	22.8582589
420	0.693181818	438.5	0.666666667	438.5	1	14	20.49390153	20.94039159	20.94039159
356	0.693181818	370.5	0.666666667	370.5	1	18	18.86796226	19.24837655	19.24837655
308	0.693181818	318.5	0.666666667	318.5	1	22	17.54992877	17.8465683	17.8465683
276	0.693181818	282.5	0.666666667	282.5	1	26	16.61324773	16.80773631	16.80773631
260	0.720930233	262.5	0.666666667	262.5	1	30	16.1245155	16.20185175	16.20185175
621.5	0.694677871	649.5	0.666666667	649.5	1	34	24.92990172	25.48528987	25.48528987
519.5	0.694677871	543.5	0.666666667	543.5	1	38	22.79254264	23.31308645	23.31308645
433.5	0.694677871	453.5	0.666666667	453.5	1	42	20.82066281	21.29553944	21.29553944
363.5	0.694677871	379.5	0.666666667	379.5	1	46	19.06567596	19.48075974	19.48075974
288.5	0.694677871	298.5	0.666666667	298.5	1	2	16.98528775	17.27715254	17.27715254
258.5	0.695652174	264.5	0.666666667	264.5	1	6	16.07793519	16.26345597	16.26345597
244.5	0.73015873	246.5	0.666666667	246.5	1	10	15.63649577	15.70031847	15.70031847
542	0.698060942	567.5	0.666666667	567.5	1	14	23.28089345	23.8222585	23.8222585
450	0.698060942	471.5	0.666666667	471.5	1	18	21.21320344	21.71405075	21.71405075
374	0.698060942	391.5	0.666666667	391.5	1	22	19.33907961	19.78635894	19.78635894
314	0.698060942	327.5	0.666666667	327.5	1	26	17.72004515	18.09696107	18.09696107
270	0.698060942	279.5	0.666666667	279.5	1	30	16.43167673	16.7182535	16.7182535
242	0.703703704	247.5	0.666666667	247.5	1	34	15.55634919	15.73213272	15.73213272
230	0.739837398	231.5	0.666666667	231.5	1	38	15.16575089	15.21512405	15.21512405
492.5	0.703296703	516.5	0.666666667	516.5	1	42	22.19234102	22.72663635	22.72663635
406.5	0.703296703	426.5	0.666666667	426.5	1	46	20.16184515	20.65187643	20.65187643
307.5	0.703296703	321.5	0.666666667	321.5	1	2	17.53567792	17.93042108	17.93042108
261.5	0.703296703	271.5	0.666666667	271.5	1	6	16.17096163	16.47725705	16.47725705
231.5	0.703703704	237.5	0.666666667	237.5	1	10	15.21512405	15.41103501	15.41103501
217.5	0.739837398	219.5	0.666666667	219.5	1	14	14.7478812	14.81553239	14.81553239
446	0.703296703	468.5	0.666666667	468.5	1	18	21.11871208	21.64486082	21.64486082
366	0.703296703	384.5	0.666666667	384.5	1	22	19.13112647	19.60867155	19.60867155
302	0.703296703	316.5	0.666666667	316.5	1	26	17.3781472	17.79044687	17.79044687
254	0.703296703	264.5	0.666666667	264.5	1	30	15.93737745	16.26345597	16.26345597
222	0.703703704	228.5	0.666666667	228.5	1	34	14.89966443	15.11621646	15.11621646
206	0.739837398	208.5	0.666666667	208.5	1	38	14.35270009	14.43952908	14.43952908
423.5	0.703296703	445.5	0.666666667	445.5	1	42	20.57911563	21.10687092	21.10687092
345.5	0.703296703	363.5	0.666666667	363.5	1	46	18.5876303	19.06567596	19.06567596
258.5	0.703296703	270.5	0.666666667	270.5	1	2	16.07793519	16.4468842	16.4468842
220.5	0.703296703	228.5	0.666666667	228.5	1	6	14.8492424	15.11621646	15.11621646
198.5	0.73015873	202.5	0.666666667	202.5	1	10	14.0890028	14.23024947	14.23024947
402	0.703296703	192.5	0.666666667	192.5	1	14	20.04993766	13.87443693	13.87443693
326	0.703296703	343.5	0.666666667	343.5	1	18	18.05547009	18.53375299	18.53375299
266	0.703296703	279.5	0.666666667	279.5	1	22	16.30950643	16.7182535	16.7182535
222	0.703296703	231.5	0.666666667	231.5	1	26	14.89966443	15.21512405	15.21512405
194	0.720930233	199.5	0.666666667	199.5	1	30	13.92838828	14.12444689	14.12444689
182	0.760683761	183.5	0.666666667	183.5	1	34	13.49073756	13.54621718	13.54621718
324.5	0.703296703	342.5	0.666666667	342.5	1	38	18.01388353	18.50675552	18.50675552
262.5	0.703296703	276.5	0.666666667	276.5	1	42	16.20185175	16.62828915	16.62828915
216.5	0.703296703	226.5	0.666666667	226.5	1	46	14.71393897	15.04991694	15.04991694
177.5	0.739837398	181.5	0.666666667	181.5	1	2	13.32291259	13.47219359	13.47219359
324	0.703296703	171.5	0.666666667	171.5	1	6	18	13.09580085	13.09580085
260	0.703296703	274.5	0.666666667	274.5	1	10	16.1245155	16.56804153	16.56804153
212	0.703296703	222.5	0.666666667	222.5	1	14	14.56021978	14.91643389	14.91643389
180	0.720930233	186.5	0.666666667	186.5	1	18	13.41640786	13.65650028	13.65650028
164	0.760683761	166.5	0.666666667	166.5	1	22	12.80624847	12.9034879	12.9034879
273.5	0.703296703	289.5	0.666666667	289.5	1	26	16.53783541	17.01469953	17.01469953
219.5	0.703296703	231.5	0.666666667	231.5	1	30	14.81553239	15.21512405	15.21512405
181.5	0.712121212	189.5	0.666666667	189.5	1	34	13.47219359	13.7658999	13.7658999
159.5	0.75	163.5	0.666666667	163.5	1	38	12.62933094	12.78671185	12.78671185
258	0.703296703	153.5	0.666666667	153.5	1	42	16.0623784	12.38951169	12.38951169
206	0.703296703	217.5	0.666666667	217.5	1	46	14.35270009	14.7478812	14.7478812
158	0.739837398	163.5	0.666666667	163.5	1	2	12.56980509	12.78671185	12.78671185
146	0.783783784	147.5	0.666666667	147.5	1	6	12.08304597	12.1449578	12.1449578
204.5	0.703296703	216.5	0.666666667	216.5	1	10	14.30034965	14.71393897	14.71393897
166.5	0.720930233	174.5	0.666666667	174.5	1	14	12.9034879	13.20984481	13.20984481
144.5	0.760683761	148.5	0.666666667	148.5	1	18	12.02081528	12.18605761	12.18605761
204	0.703296703	138.5	0.666666667	138.5	1	22	14.28285686	11.7686023	11.7686023
164	0.720930233	172.5	0.666666667	172.5	1	26	12.80624847	13.13392554	13.13392554
140	0.760683761	144.5	0.666666667	144.5	1	30	11.83215957	12.02081528	12.02081528
132	0.80952381	132.5	0.666666667	132.5	1	34	11.48912529	11.51086443	11.51086443
154.5	0.73015873	162.5	0.666666667	162.5	1	38	12.42980289	12.74754878	12.74754878
132.5	0.771929825	136.5	0.666666667	136.5	1	42	11.51086443	11.68332145	11.68332145
162	0.720930233	126.5	0.666666667	126.5	1	46	12.72792206	11.24722188	11.24722188
126	0.783783784	129.5	0.666666667	129.5	1	2	11.22497216	11.37980668	11.37980668
145.5	0.739837398	121.5	0.666666667	121.5	1	6	12.06233808	11.02270384	11.02270384
123.5	0.783783784	127.5	0.666666667	127.5	1	10	11.11305539	11.29158979	11.29158979
132	0.760683761	117.5	0.666666667	117.5	1	14	11.48912529	10.83974169	10.83974169
116	0.80952381	118.5	0.666666667	118.5	1	18	10.77032961	10.88577053	10.88577053
117.5	0.796296296	121.5	0.666666667	121.5	1	22	10.83974169	11.02270384	11.02270384
114	0.80952381	111.5	0.666666667	111.5	1	26	10.67707825	10.55935604	10.55935604
109.5	0.838383838	109.5	0.666666667	109.5	1	30	10.46422477	10.46422477	10.46422477
833.5	0.696696697	867	0.666666667	867	1	34	28.87040007	29.44486373	29.44486373
709.5	0.696696697	739	0.666666667	739	1	38	26.6364412	27.18455444	27.18455444
601.5	0.696696697	627	0.666666667	627	1	42	24.52549694	25.03996805	25.03996805
509.5	0.696696697	531	0.666666667	531	1	46	22.57210668	23.04343724	23.04343724
401.5	0.696696697	417	0.666666667	417	1	2	20.03746491	20.42057786	20.42057786
349.5	0.696696697	361	0.666666667	361	1	6	18.6949191	19	19
313.5	0.696696697	321	0.666666667	321	1	10	17.70593121	17.91647287	17.91647287
293.5	0.703703704	297	0.666666667	297	1	14	17.1318417	17.23368794	17.23368794
800.5	0.696696697	289	0.666666667	289	1	18	28.2931087	17	17
678.5	0.696696697	707.5	0.666666667	707.5	1	22	26.04803256	26.59887216	26.59887216
572.5	0.696696697	597.5	0.666666667	597.5	1	26	23.92697223	24.44381312	24.44381312
482.5	0.696696697	503.5	0.666666667	503.5	1	30	21.96588264	22.43880567	22.43880567
408.5	0.696696697	425.5	0.666666667	425.5	1	34	20.21138293	20.62765134	20.62765134
350.5	0.696696697	363.5	0.666666667	363.5	1	38	18.72164523	19.06567596	19.06567596
308.5	0.696696697	317.5	0.666666667	317.5	1	42	17.56416807	17.81852968	17.81852968
282.5	0.696696697	287.5	0.666666667	287.5	1	46	16.80773631	16.95582496	16.95582496
706.5	0.696696697	737	0.666666667	737	1	2	26.58006772	27.14774392	27.14774392
594.5	0.696696697	621	0.666666667	621	1	6	24.38237068	24.91987159	24.91987159
498.5	0.696696697	521	0.666666667	521	1	10	22.32711356	22.82542442	22.82542442
418.5	0.696696697	437	0.666666667	437	1	14	20.45727255	20.90454496	20.90454496
354.5	0.696696697	369	0.666666667	369	1	18	18.82817038	19.20937271	19.20937271
306.5	0.696696697	317	0.666666667	317	1	22	17.5071414	17.80449381	17.80449381
274.5	0.696696697	281	0.666666667	281	1	26	16.56804153	16.76305461	16.76305461
258.5	0.720930233	261	0.666666667	261	1	30	16.07793519	16.15549442	16.15549442
647.5	0.701149425	676.5	0.666666667	676.5	1	34	25.4460213	26.00961361	26.00961361
541.5	0.701149425	566.5	0.666666667	566.5	1	38	23.27015256	23.80126047	23.80126047
451.5	0.701149425	472.5	0.666666667	472.5	1	42	21.24852936	21.73706512	21.73706512
377.5	0.701149425	394.5	0.666666667	394.5	1	46	19.42935923	19.86202407	19.86202407
296.5	0.701149425	307.5	0.666666667	307.5	1	2	17.21917536	17.53567792	17.53567792
262.5	0.701149425	269.5	0.666666667	269.5	1	6	16.20185175	16.41645516	16.41645516
244.5	0.720930233	247.5	0.666666667	247.5	1	10	15.63649577	15.73213272	15.73213272
591.5	0.702549575	619	0.666666667	619	1	14	24.32077301	24.87971061	24.87971061
491.5	0.702549575	515	0.666666667	515	1	18	22.16979928	22.69361144	22.69361144
407.5	0.702549575	427	0.666666667	427	1	22	20.18662924	20.66397832	20.66397832
339.5	0.702549575	355	0.666666667	355	1	26	18.42552577	18.84144368	18.84144368
287.5	0.702549575	299	0.666666667	299	1	30	16.95582496	17.29161647	17.29161647
251.5	0.702549575	259	0.666666667	259	1	34	15.85875153	16.09347694	16.09347694
231.5	0.720930233	235	0.666666667	235	1	38	15.21512405	15.32970972	15.32970972
564.5	0.705882353	227	0.666666667	227	1	42	23.75920874	15.06651917	15.06651917
466.5	0.705882353	489.5	0.666666667	489.5	1	46	21.59861107	22.12464689	22.12464689
349.5	0.705882353	366.5	0.666666667	366.5	1	2	18.6949191	19.14418972	19.14418972
291.5	0.705882353	304.5	0.666666667	304.5	1	6	17.07337108	17.44992837	17.44992837
249.5	0.705882353	258.5	0.666666667	258.5	1	10	15.795569	16.07793519	16.07793519
223.5	0.712121212	228.5	0.666666667	228.5	1	14	14.94991639	15.11621646	15.11621646
213.5	0.75	214.5	0.666666667	214.5	1	18	14.6116392	14.64581852	14.64581852
442.5	0.711111111	465	0.666666667	465	1	22	21.03568397	21.56385865	21.56385865
362.5	0.711111111	381	0.666666667	381	1	26	19.03943276	19.5192213	19.5192213
298.5	0.711111111	313	0.666666667	313	1	30	17.27715254	17.69180601	17.69180601
250.5	0.711111111	261	0.666666667	261	1	34	15.82719179	16.15549442	16.15549442
218.5	0.711111111	225	0.666666667	225	1	38	14.7817455	15	15
202.5	0.739837398	205	0.666666667	205	1	42	14.23024947	14.31782106	14.31782106
441.5	0.711111111	464.5	0.666666667	464.5	1	46	21.01190139	21.55226206	21.55226206
324.5	0.711111111	341.5	0.666666667	341.5	1	2	18.01388353	18.47971861	18.47971861
266.5	0.711111111	279.5	0.666666667	279.5	1	6	16.32482772	16.7182535	16.7182535
224.5	0.711111111	233.5	0.666666667	233.5	1	10	14.98332406	15.28070679	15.28070679
198.5	0.720930233	203.5	0.666666667	203.5	1	14	14.0890028	14.26534262	14.26534262
188.5	0.760683761	189.5	0.666666667	189.5	1	18	13.72953022	13.7658999	13.7658999
357.5	0.711111111	377	0.666666667	377	1	22	18.9076704	19.41648784	19.41648784
289.5	0.711111111	305	0.666666667	305	1	26	17.01469953	17.4642492	17.4642492
237.5	0.711111111	249	0.666666667	249	1	30	15.41103501	15.77973384	15.77973384
201.5	0.711111111	209	0.666666667	209	1	34	14.19506957	14.45683229	14.45683229
181.5	0.739837398	185	0.666666667	185	1	38	13.47219359	13.60147051	13.60147051
376.5	0.711111111	177	0.666666667	177	1	42	19.40360791	13.3041347	13.3041347
302.5	0.711111111	319.5	0.666666667	319.5	1	46	17.39252713	17.87456293	17.87456293
221.5	0.711111111	232.5	0.666666667	232.5	1	2	14.88287607	15.24795068	15.24795068
187.5	0.712121212	194.5	0.666666667	194.5	1	6	13.69306394	13.94632568	13.94632568
169.5	0.75	172.5	0.666666667	172.5	1	10	13.01921657	13.13392554	13.13392554
318.5	0.711111111	337	0.666666667	337	1	14	17.8465683	18.35755975	18.35755975
254.5	0.711111111	269	0.666666667	269	1	18	15.95305613	16.40121947	16.40121947
206.5	0.711111111	217	0.666666667	217	1	22	14.37010786	14.73091986	14.73091986
174.5	0.720930233	181	0.666666667	181	1	26	13.20984481	13.45362405	13.45362405
158.5	0.760683761	161	0.666666667	161	1	30	12.58967831	12.68857754	12.68857754
283.5	0.711111111	300.5	0.666666667	300.5	1	34	16.83745824	17.33493582	17.33493582
225.5	0.711111111	238.5	0.666666667	238.5	1	38	15.01665742	15.44344521	15.44344521
183.5	0.711111111	192.5	0.666666667	192.5	1	42	13.54621718	13.87443693	13.87443693
157.5	0.739837398	162.5	0.666666667	162.5	1	46	12.5499004	12.74754878	12.74754878
251.5	0.711111111	267	0.666666667	267	1	2	15.85875153	16.34013464	16.34013464
199.5	0.711111111	211	0.666666667	211	1	6	14.12444689	14.52583905	14.52583905
163.5	0.720930233	171	0.666666667	171	1	10	12.78671185	13.07669683	13.07669683
143.5	0.760683761	147	0.666666667	147	1	14	11.97914855	12.12435565	12.12435565
236.5	0.711111111	139	0.666666667	139	1	18	15.3785565	11.78982612	11.78982612
186.5	0.711111111	197.5	0.666666667	197.5	1	22	13.65650028	14.05346932	14.05346932
152.5	0.73015873	159.5	0.666666667	159.5	1	26	12.34908904	12.62933094	12.62933094
134.5	0.771929825	137.5	0.666666667	137.5	1	30	11.5974135	11.7260394	11.7260394
196.5	0.711111111	209	0.666666667	209	1	34	14.01784577	14.45683229	14.45683229
156.5	0.720930233	165	0.666666667	165	1	38	12.509996	12.84523258	12.84523258
132.5	0.760683761	137	0.666666667	137	1	42	11.51086443	11.70469991	11.70469991
124.5	0.80952381	125	0.666666667	125	1	46	11.1579568	11.18033989	11.18033989
139.5	0.739837398	146.5	0.666666667	146.5	1	2	11.81101181	12.10371844	12.10371844
121.5	0.783783784	124.5	0.666666667	124.5	1	6	11.02270384	11.1579568	11.1579568
153.5	0.720930233	163	0.666666667	163	1	10	12.38951169	12.76714533	12.76714533
125.5	0.760683761	131	0.666666667	131	1	14	11.20267825	11.44552314	11.44552314
113.5	0.80952381	115	0.666666667	115	1	18	10.65363788	10.72380529	10.72380529
129.5	0.75	136.5	0.666666667	136.5	1	22	11.37980668	11.68332145	11.68332145
111.5	0.796296296	114.5	0.666666667	114.5	1	26	10.55935604	10.70046728	10.70046728
122.5	0.760683761	129	0.666666667	129	1	30	11.06797181	11.35781669	11.35781669
106.5	0.80952381	109	0.666666667	109	1	34	10.31988372	10.44030651	10.44030651
111.5	0.783783784	116.5	0.666666667	116.5	1	38	10.55935604	10.79351657	10.79351657
101.5	0.838383838	102.5	0.666666667	102.5	1	42	10.07472084	10.12422837	10.12422837
99.5	0.838383838	101	0.666666667	101	1	46	9.974968672	10.04987562	10.04987562
96.5	0.870967742	97	0.666666667	97	1	2	9.823441352	9.848857802	9.848857802
676.5	0.704477612	706	0.666666667	706	1	6	26.00961361	26.57066051	26.57066051
568.5	0.704477612	594	0.666666667	594	1	10	23.84323804	24.37211521	24.37211521
476.5	0.704477612	498	0.666666667	498	1	14	21.82887995	22.3159136	22.3159136
400.5	0.704477612	418	0.666666667	418	1	18	20.0124961	20.4450483	20.4450483
340.5	0.704477612	354	0.666666667	354	1	22	18.45264209	18.81488772	18.81488772
296.5	0.704477612	306	0.666666667	306	1	26	17.21917536	17.49285568	17.49285568
268.5	0.704477612	274	0.666666667	274	1	30	16.38596961	16.55294536	16.55294536
256.5	0.73015873	258	0.666666667	258	1	34	16.01561738	16.0623784	16.0623784
646.5	0.705882353	675.5	0.666666667	675.5	1	38	25.42636427	25.99038284	25.99038284
540.5	0.705882353	565.5	0.666666667	565.5	1	42	23.24865588	23.7802439	23.7802439
450.5	0.705882353	471.5	0.666666667	471.5	1	46	21.22498528	21.71405075	21.71405075
345.5	0.705882353	360.5	0.666666667	360.5	1	2	18.5876303	18.98683755	18.98683755
295.5	0.705882353	306.5	0.666666667	306.5	1	6	17.19011344	17.5071414	17.5071414
261.5	0.705882353	268.5	0.666666667	268.5	1	10	16.17096163	16.38596961	16.38596961
243.5	0.720930233	246.5	0.666666667	246.5	1	14	15.60448653	15.70031847	15.70031847
617.5	0.707246377	646	0.666666667	646	1	18	24.84954728	25.41653005	25.41653005
513.5	0.707246377	538	0.666666667	538	1	22	22.66053839	23.19482701	23.19482701
425.5	0.707246377	446	0.666666667	446	1	26	20.62765134	21.11871208	21.11871208
353.5	0.707246377	370	0.666666667	370	1	30	18.80159568	19.23538406	19.23538406
297.5	0.707246377	310	0.666666667	310	1	34	17.24818831	17.60681686	17.60681686
257.5	0.707246377	266	0.666666667	266	1	38	16.04680654	16.30950643	16.30950643
233.5	0.712121212	238	0.666666667	238	1	42	15.28070679	15.42724862	15.42724862
225.5	0.75	226	0.666666667	226	1	46	15.01665742	15.03329638	15.03329638
464.5	0.710601719	487.5	0.666666667	487.5	1	2	21.55226206	22.07940217	22.07940217
382.5	0.710601719	401.5	0.666666667	401.5	1	6	19.55760722	20.03746491	20.03746491
316.5	0.710601719	331.5	0.666666667	331.5	1	10	17.79044687	18.20714146	18.20714146
266.5	0.710601719	277.5	0.666666667	277.5	1	14	16.32482772	16.65833125	16.65833125
232.5	0.710601719	239.5	0.666666667	239.5	1	18	15.24795068	15.47578754	15.47578754
214.5	0.73015873	217.5	0.666666667	217.5	1	22	14.64581852	14.7478812	14.7478812
510.5	0.71388102	536	0.666666667	536	1	26	22.59424706	23.15167381	23.15167381
418.5	0.71388102	440	0.666666667	440	1	30	20.45727255	20.97617696	20.97617696
342.5	0.71388102	360	0.666666667	360	1	34	18.50675552	18.97366596	18.97366596
282.5	0.71388102	296	0.666666667	296	1	38	16.80773631	17.20465053	17.20465053
238.5	0.71388102	248	0.666666667	248	1	42	15.44344521	15.74801575	15.74801575
210.5	0.71388102	216	0.666666667	216	1	46	14.50861813	14.69693846	14.69693846
485.5	0.71388102	198	0.666666667	198	1	2	22.03406454	14.07124728	14.07124728
395.5	0.71388102	416.5	0.666666667	416.5	1	6	19.8871818	20.40833163	20.40833163
321.5	0.71388102	338.5	0.666666667	338.5	1	10	17.93042108	18.39836949	18.39836949
263.5	0.71388102	276.5	0.666666667	276.5	1	14	16.23268308	16.62828915	16.62828915
221.5	0.71388102	230.5	0.666666667	230.5	1	18	14.88287607	15.18222645	15.18222645
195.5	0.720930233	200.5	0.666666667	200.5	1	22	13.98213145	14.15980226	14.15980226
185.5	0.760683761	186.5	0.666666667	186.5	1	26	13.61983847	13.65650028	13.65650028
373.5	0.71388102	394	0.666666667	394	1	30	19.32614809	19.84943324	19.84943324
301.5	0.71388102	318	0.666666667	318	1	34	17.36375535	17.8325545	17.8325545
245.5	0.71388102	258	0.666666667	258	1	38	15.66843962	16.0623784	16.0623784
205.5	0.71388102	214	0.666666667	214	1	42	14.33527119	14.62873884	14.62873884
181.5	0.73015873	186	0.666666667	186	1	46	13.47219359	13.6381817	13.6381817
372.5	0.71388102	393.5	0.666666667	393.5	1	2	19.30025907	19.83683442	19.83683442
298.5	0.71388102	315.5	0.666666667	315.5	1	6	17.27715254	17.76231967	17.76231967
240.5	0.71388102	253.5	0.666666667	253.5	1	10	15.50806242	15.92168333	15.92168333
198.5	0.71388102	207.5	0.666666667	207.5	1	14	14.0890028	14.40486029	14.40486029
172.5	0.73015873	177.5	0.666666667	177.5	1	18	13.13392554	13.32291259	13.32291259
162.5	0.771929825	163.5	0.666666667	163.5	1	22	12.74754878	12.78671185	12.78671185
296.5	0.71388102	314	0.666666667	314	1	26	17.21917536	17.72004515	17.72004515
236.5	0.71388102	250	0.666666667	250	1	30	15.3785565	15.8113883	15.8113883
192.5	0.71388102	202	0.666666667	202	1	34	13.87443693	14.2126704	14.2126704
164.5	0.73015873	170	0.666666667	170	1	38	12.82575534	13.03840481	13.03840481
152.5	0.771929825	154	0.666666667	154	1	42	12.34908904	12.40967365	12.40967365
278.5	0.71388102	295.5	0.666666667	295.5	1	46	16.68831927	17.19011344	17.19011344
197.5	0.71388102	208.5	0.666666667	208.5	1	2	14.05346932	14.43952908	14.43952908
163.5	0.720930233	170.5	0.666666667	170.5	1	6	12.78671185	13.05756486	13.05756486
145.5	0.760683761	148.5	0.666666667	148.5	1	10	12.06233808	12.18605761	12.18605761
261.5	0.71388102	278	0.666666667	278	1	14	16.17096163	16.673332	16.673332
205.5	0.71388102	218	0.666666667	218	1	18	14.33527119	14.76482306	14.76482306
165.5	0.71388102	174	0.666666667	174	1	22	12.86468033	13.19090596	13.19090596
141.5	0.75	146	0.666666667	146	1	26	11.89537725	12.08304597	12.08304597
133.5	0.796296296	134	0.666666667	134	1	30	11.55422001	11.5758369	11.5758369
203.5	0.71388102	216.5	0.666666667	216.5	1	34	14.26534262	14.71393897	14.71393897
161.5	0.71388102	170.5	0.666666667	170.5	1	38	12.70826503	13.05756486	13.05756486
135.5	0.75	140.5	0.666666667	140.5	1	42	11.64044673	11.85326959	11.85326959
125.5	0.796296296	126.5	0.666666667	126.5	1	46	11.20267825	11.24722188	11.24722188
158.5	0.71388102	168	0.666666667	168	1	2	12.58967831	12.9614814	12.9614814
130.5	0.75	136	0.666666667	136	1	6	11.42365966	11.66190379	11.66190379
118.5	0.796296296	120	0.666666667	120	1	10	10.88577053	10.95445115	10.95445115
166.5	0.71388102	177.5	0.666666667	177.5	1	14	12.9034879	13.32291259	13.32291259
132.5	0.739837398	139.5	0.666666667	139.5	1	18	11.51086443	11.81101181	11.81101181
114.5	0.783783784	117.5	0.666666667	117.5	1	22	10.70046728	10.83974169	10.83974169
155.5	0.71388102	166	0.666666667	166	1	26	12.46996391	12.88409873	12.88409873
123.5	0.75	130	0.666666667	130	1	30	11.11305539	11.40175425	11.40175425
107.5	0.796296296	110	0.666666667	110	1	34	10.36822068	10.48808848	10.48808848
136.5	0.73015873	145.5	0.666666667	145.5	1	38	11.68332145	12.06233808	12.06233808
110.5	0.771929825	115.5	0.666666667	115.5	1	42	10.51189802	10.74709263	10.74709263
100.5	0.823529412	101.5	0.666666667	101.5	1	46	10.02496883	10.07472084	10.07472084
100.5	0.796296296	104	0.666666667	104	1	2	10.02496883	10.19803903	10.19803903
113.5	0.760683761	96	0.666666667	96	1	6	10.65363788	9.797958971	9.797958971
95.5	0.80952381	98.5	0.666666667	98.5	1	10	9.772410143	9.924716621	9.924716621
97.5	0.796296296	102	0.666666667	102	1	14	9.874208829	10.09950494	10.09950494
89.5	0.854166667	90	0.666666667	90	1	18	9.460443964	9.486832981	9.486832981
87.5	0.854166667	88.5	0.666666667	88.5	1	22	9.354143467	9.407443861	9.407443861
85.5	0.870967742	86	0.666666667	86	1	26	9.246621004	9.273618495	9.273618495
589.5	0.707246377	617	0.666666667	617	1	30	24.27962108	24.8394847	24.8394847
489.5	0.707246377	513	0.666666667	513	1	34	22.12464689	22.64950331	22.64950331
405.5	0.707246377	425	0.666666667	425	1	38	20.13703057	20.61552813	20.61552813
337.5	0.707246377	353	0.666666667	353	1	42	18.37117307	18.78829423	18.78829423
285.5	0.707246377	297	0.666666667	297	1	46	16.89674525	17.23368794	17.23368794
237.5	0.707246377	243	0.666666667	243	1	2	15.41103501	15.58845727	15.58845727
225.5	0.739837398	227	0.666666667	227	1	6	15.01665742	15.06651917	15.06651917
561.5	0.715542522	588.5	0.666666667	588.5	1	10	23.69599122	24.25901894	24.25901894
463.5	0.715542522	486.5	0.666666667	486.5	1	14	21.52905014	22.056745	22.056745
381.5	0.715542522	400.5	0.666666667	400.5	1	18	19.53202498	20.0124961	20.0124961
315.5	0.715542522	330.5	0.666666667	330.5	1	22	17.76231967	18.17965896	18.17965896
265.5	0.715542522	276.5	0.666666667	276.5	1	26	16.29417074	16.62828915	16.62828915
231.5	0.715542522	238.5	0.666666667	238.5	1	30	15.21512405	15.44344521	15.44344521
213.5	0.73015873	216.5	0.666666667	216.5	1	34	14.6116392	14.71393897	14.71393897
534.5	0.71884058	561	0.666666667	561	1	38	23.11925604	23.68543856	23.68543856
438.5	0.71884058	461	0.666666667	461	1	42	20.94039159	21.47091055	21.47091055
358.5	0.71884058	377	0.666666667	377	1	46	18.93409623	19.41648784	19.41648784
268.5	0.71884058	281	0.666666667	281	1	2	16.38596961	16.76305461	16.76305461
228.5	0.71884058	237	0.666666667	237	1	6	15.11621646	15.39480432	15.39480432
204.5	0.720930233	209	0.666666667	209	1	10	14.30034965	14.45683229	14.45683229
196.5	0.760683761	197	0.666666667	197	1	14	14.01784577	14.03566885	14.03566885
436.5	0.722063037	459.5	0.666666667	459.5	1	18	20.89258242	21.43595111	21.43595111
354.5	0.722063037	373.5	0.666666667	373.5	1	22	18.82817038	19.32614809	19.32614809
288.5	0.722063037	303.5	0.666666667	303.5	1	26	16.98528775	17.42125139	17.42125139
238.5	0.722063037	249.5	0.666666667	249.5	1	30	15.44344521	15.795569	15.795569
204.5	0.722063037	211.5	0.666666667	211.5	1	34	14.30034965	14.54303957	14.54303957
186.5	0.739837398	189.5	0.666666667	189.5	1	38	13.65650028	13.7658999	13.7658999
435.5	0.722063037	459	0.666666667	459	1	42	20.86863675	21.42428529	21.42428529
351.5	0.722063037	371	0.666666667	371	1	46	18.74833326	19.26136028	19.26136028
255.5	0.722063037	269	0.666666667	269	1	2	15.98436736	16.40121947	16.40121947
211.5	0.722063037	221	0.666666667	221	1	6	14.54303957	14.86606875	14.86606875
183.5	0.722063037	189	0.666666667	189	1	10	13.54621718	13.74772708	13.74772708
171.5	0.760683761	173	0.666666667	173	1	14	13.09580085	13.15294644	13.15294644
369.5	0.722063037	390.5	0.666666667	390.5	1	18	19.22238279	19.76107285	19.76107285
295.5	0.722063037	312.5	0.666666667	312.5	1	22	17.19011344	17.67766953	17.67766953
237.5	0.722063037	250.5	0.666666667	250.5	1	26	15.41103501	15.82719179	15.82719179
195.5	0.722063037	204.5	0.666666667	204.5	1	30	13.98213145	14.30034965	14.30034965
169.5	0.73015873	174.5	0.666666667	174.5	1	34	13.01921657	13.20984481	13.20984481
159.5	0.771929825	160.5	0.666666667	160.5	1	38	12.62933094	12.66885946	12.66885946
310.5	0.722063037	329	0.666666667	329	1	42	17.62101019	18.13835715	18.13835715
246.5	0.722063037	261	0.666666667	261	1	46	15.70031847	16.15549442	16.15549442
180.5	0.722063037	189	0.666666667	189	1	2	13.43502884	13.74772708	13.74772708
156.5	0.739837398	161	0.666666667	161	1	6	12.509996	12.68857754	12.68857754
148.5	0.783783784	149	0.666666667	149	1	10	12.18605761	12.20655562	12.20655562
274.5	0.722063037	291.5	0.666666667	291.5	1	14	16.56804153	17.07337108	17.07337108
216.5	0.722063037	229.5	0.666666667	229.5	1	18	14.71393897	15.14925741	15.14925741
174.5	0.722063037	183.5	0.666666667	183.5	1	22	13.20984481	13.54621718	13.54621718
148.5	0.739837398	153.5	0.666666667	153.5	1	26	12.18605761	12.38951169	12.38951169
138.5	0.783783784	139.5	0.666666667	139.5	1	30	11.7686023	11.81101181	11.81101181
241.5	0.722063037	257	0.666666667	257	1	34	15.54027027	16.03121954	16.03121954
189.5	0.722063037	201	0.666666667	201	1	38	13.7658999	14.17744688	14.17744688
153.5	0.722063037	161	0.666666667	161	1	42	12.38951169	12.68857754	12.68857754
133.5	0.760683761	137	0.666666667	137	1	46	11.55422001	11.70469991	11.70469991
225.5	0.722063037	240.5	0.666666667	240.5	1	2	15.01665742	15.50806242	15.50806242
175.5	0.722063037	186.5	0.666666667	186.5	1	6	13.2476413	13.65650028	13.65650028
141.5	0.73015873	148.5	0.666666667	148.5	1	10	11.89537725	12.18605761	12.18605761
123.5	0.771929825	126.5	0.666666667	126.5	1	14	11.11305539	11.24722188	11.24722188
210.5	0.722063037	225	0.666666667	225	1	18	14.50861813	15	15
162.5	0.722063037	173	0.666666667	173	1	22	12.74754878	13.15294644	13.15294644
130.5	0.739837398	137	0.666666667	137	1	26	11.42365966	11.70469991	11.70469991
114.5	0.783783784	117	0.666666667	117	1	30	10.70046728	10.81665383	10.81665383
183.5	0.722063037	196.5	0.666666667	196.5	1	34	13.54621718	14.01784577	14.01784577
141.5	0.722063037	150.5	0.666666667	150.5	1	38	11.89537725	12.26784415	12.26784415
115.5	0.760683761	120.5	0.666666667	120.5	1	42	10.74709263	10.9772492	10.9772492
105.5	0.80952381	106.5	0.666666667	106.5	1	46	10.27131929	10.31988372	10.31988372
123.5	0.739837398	131	0.666666667	131	1	2	11.11305539	11.44552314	11.44552314
103.5	0.783783784	107	0.666666667	107	1	6	10.17349497	10.34408043	10.34408043
148.5	0.722063037	99	0.666666667	99	1	10	12.18605761	9.949874371	9.949874371
114.5	0.75	121.5	0.666666667	121.5	1	14	10.70046728	11.02270384	11.02270384
96.5	0.796296296	99.5	0.666666667	99.5	1	18	9.823441352	9.974968672	9.974968672
120.5	0.739837398	129	0.666666667	129	1	22	10.9772492	11.35781669	11.35781669
96.5	0.783783784	101	0.666666667	101	1	26	9.823441352	10.04987562	10.04987562
88.5	0.838383838	89	0.666666667	89	1	30	9.407443861	9.433981132	9.433981132
94.5	0.783783784	99.5	0.666666667	99.5	1	34	9.721111048	9.974968672	9.974968672
84.5	0.838383838	85.5	0.666666667	85.5	1	38	9.192388155	9.246621004	9.246621004
85.5	0.80952381	89	0.666666667	89	1	42	9.246621004	9.433981132	9.433981132
88.5	0.796296296	81	0.666666667	81	1	46	9.407443861	9	9
78.5	0.838383838	81	0.666666667	81	1	2	8.860022573	9	9
75.5	0.870967742	76.5	0.666666667	76.5	1	6	8.689073598	8.746427842	8.746427842
534	0.724035608	560.5	0.666666667	560.5	1	10	23.10844002	23.6748812	23.6748812
438	0.724035608	460.5	0.666666667	460.5	1	14	20.92844954	21.45926373	21.45926373
358	0.724035608	376.5	0.666666667	376.5	1	18	18.92088793	19.40360791	19.40360791
294	0.724035608	308.5	0.666666667	308.5	1	22	17.1464282	17.56416807	17.56416807
246	0.724035608	256.5	0.666666667	256.5	1	26	15.68438714	16.01561738	16.01561738
214	0.724035608	220.5	0.666666667	220.5	1	30	14.62873884	14.8492424	14.8492424
198	0.739837398	200.5	0.666666667	200.5	1	34	14.07124728	14.15980226	14.15980226
507.5	0.725146199	533.5	0.666666667	533.5	1	38	22.52776065	23.09761892	23.09761892
413.5	0.725146199	435.5	0.666666667	435.5	1	42	20.33469941	20.86863675	20.86863675
335.5	0.725146199	353.5	0.666666667	353.5	1	46	18.31665908	18.80159568	18.80159568
248.5	0.725146199	260.5	0.666666667	260.5	1	2	15.76388277	16.14001239	16.14001239
210.5	0.725146199	218.5	0.666666667	218.5	1	6	14.50861813	14.7817455	14.7817455
188.5	0.73015873	192.5	0.666666667	192.5	1	10	13.72953022	13.87443693	13.87443693
482	0.730434783	182.5	0.666666667	182.5	1	14	21.9544984	13.50925609	13.50925609
390	0.730434783	411.5	0.666666667	411.5	1	18	19.74841766	20.28546278	20.28546278
314	0.730434783	331.5	0.666666667	331.5	1	22	17.72004515	18.20714146	18.20714146
254	0.730434783	267.5	0.666666667	267.5	1	26	15.93737745	16.35542723	16.35542723
210	0.730434783	219.5	0.666666667	219.5	1	30	14.49137675	14.81553239	14.81553239
182	0.730434783	187.5	0.666666667	187.5	1	34	13.49073756	13.69306394	13.69306394
170	0.760683761	171.5	0.666666667	171.5	1	38	13.03840481	13.09580085	13.09580085
388.5	0.730434783	410.5	0.666666667	410.5	1	42	19.71040334	20.26079959	20.26079959
310.5	0.730434783	328.5	0.666666667	328.5	1	46	17.62101019	18.12456896	18.12456896
223.5	0.730434783	235.5	0.666666667	235.5	1	2	14.94991639	15.34600925	15.34600925
185.5	0.730434783	193.5	0.666666667	193.5	1	6	13.61983847	13.91042774	13.91042774
163.5	0.739837398	167.5	0.666666667	167.5	1	10	12.78671185	12.94217911	12.94217911
388	0.730434783	157.5	0.666666667	157.5	1	14	19.6977156	12.5499004	12.5499004
308	0.730434783	326.5	0.666666667	326.5	1	18	17.54992877	18.069311	18.069311
244	0.730434783	258.5	0.666666667	258.5	1	22	15.62049935	16.07793519	16.07793519
196	0.730434783	206.5	0.666666667	206.5	1	26	14	14.37010786	14.37010786
164	0.730434783	170.5	0.666666667	170.5	1	30	12.80624847	13.05756486	13.05756486
148	0.760683761	150.5	0.666666667	150.5	1	34	12.16552506	12.26784415	12.26784415
325.5	0.730434783	345.5	0.666666667	345.5	1	38	18.04161855	18.5876303	18.5876303
255.5	0.730434783	271.5	0.666666667	271.5	1	42	15.98436736	16.47725705	16.47725705
201.5	0.730434783	213.5	0.666666667	213.5	1	46	14.19506957	14.6116392	14.6116392
150.5	0.730434783	156.5	0.666666667	156.5	1	2	12.26784415	12.509996	12.509996
136.5	0.771929825	138.5	0.666666667	138.5	1	6	11.68332145	11.7686023	11.7686023
270	0.730434783	287.5	0.666666667	287.5	1	10	16.43167673	16.95582496	16.95582496
210	0.730434783	223.5	0.666666667	223.5	1	14	14.49137675	14.94991639	14.94991639
166	0.730434783	175.5	0.666666667	175.5	1	18	12.88409873	13.2476413	13.2476413
138	0.739837398	143.5	0.666666667	143.5	1	22	11.74734012	11.97914855	11.97914855
126	0.783783784	127.5	0.666666667	127.5	1	26	11.22497216	11.29158979	11.29158979
236.5	0.730434783	252.5	0.666666667	252.5	1	30	15.3785565	15.89024858	15.89024858
182.5	0.730434783	194.5	0.666666667	194.5	1	34	13.50925609	13.94632568	13.94632568
144.5	0.730434783	152.5	0.666666667	152.5	1	38	12.02081528	12.34908904	12.34908904
122.5	0.760683761	126.5	0.666666667	126.5	1	42	11.06797181	11.24722188	11.24722188
236	0.730434783	116.5	0.666666667	116.5	1	46	15.3622915	10.79351657	10.79351657
158	0.730434783	168.5	0.666666667	168.5	1	2	12.56980509	12.98075499	12.98075499
126	0.739837398	132.5	0.666666667	132.5	1	6	11.22497216	11.51086443	11.51086443
110	0.783783784	112.5	0.666666667	112.5	1	10	10.48808848	10.60660172	10.60660172
191.5	0.730434783	205.5	0.666666667	205.5	1	14	13.8383525	14.33527119	14.33527119
145.5	0.730434783	155.5	0.666666667	155.5	1	18	12.06233808	12.46996391	12.46996391
115.5	0.75	121.5	0.666666667	121.5	1	22	10.74709263	11.02270384	11.02270384
101.5	0.796296296	103.5	0.666666667	103.5	1	26	10.07472084	10.17349497	10.17349497
154	0.730434783	165.5	0.666666667	165.5	1	30	12.40967365	12.86468033	12.86468033
118	0.739837398	125.5	0.666666667	125.5	1	34	10.86278049	11.20267825	11.20267825
98	0.783783784	101.5	0.666666667	101.5	1	38	9.899494937	10.07472084	10.07472084
153.5	0.730434783	93.5	0.666666667	93.5	1	42	12.38951169	9.669539803	9.669539803
115.5	0.739837398	123.5	0.666666667	123.5	1	46	10.74709263	11.11305539	11.11305539
88.5	0.80952381	90.5	0.666666667	90.5	1	2	9.407443861	9.513148795	9.513148795
114	0.739837398	122.5	0.666666667	122.5	1	6	10.67707825	11.06797181	11.06797181
90	0.783783784	94.5	0.666666667	94.5	1	10	9.486832981	9.721111048	9.721111048
82	0.838383838	82.5	0.666666667	82.5	1	14	9.055385138	9.082951062	9.082951062
92.5	0.771929825	98.5	0.666666667	98.5	1	18	9.617692031	9.924716621	9.924716621
78.5	0.823529412	80.5	0.666666667	80.5	1	22	8.860022573	8.972179222	8.972179222
86	0.783783784	91.5	0.666666667	91.5	1	26	9.273618495	9.565563235	9.565563235
74	0.838383838	75.5	0.666666667	75.5	1	30	8.602325267	8.689073598	8.689073598
76.5	0.80952381	80.5	0.666666667	80.5	1	34	8.746427842	8.972179222	8.972179222
76	0.80952381	70.5	0.666666667	70.5	1	38	8.717797887	8.396427812	8.396427812
68	0.870967742	68.5	0.666666667	68.5	1	42	8.246211251	8.276472679	8.276472679
66	0.870967742	66.5	0.666666667	66.5	1	46	8.124038405	8.154753215	8.154753215
411	0.733727811	433.5	0.666666667	433.5	1	2	20.27313493	20.82066281	20.82066281
331	0.733727811	349.5	0.666666667	349.5	1	6	18.1934054	18.6949191	18.6949191
267	0.733727811	281.5	0.666666667	281.5	1	10	16.34013464	16.77796174	16.77796174
219	0.733727811	229.5	0.666666667	229.5	1	14	14.79864859	15.14925741	15.14925741
187	0.733727811	193.5	0.666666667	193.5	1	18	13.67479433	13.91042774	13.91042774
171	0.75	173.5	0.666666667	173.5	1	22	13.07669683	13.17193987	13.17193987
432.5	0.733727811	456.5	0.666666667	456.5	1	26	20.79663434	21.36586062	21.36586062
346.5	0.733727811	366.5	0.666666667	366.5	1	30	18.61451047	19.14418972	19.14418972
276.5	0.733727811	292.5	0.666666667	292.5	1	34	16.62828915	17.10263138	17.10263138
222.5	0.733727811	234.5	0.666666667	234.5	1	38	14.91643389	15.31339283	15.31339283
184.5	0.733727811	192.5	0.666666667	192.5	1	42	13.58307771	13.87443693	13.87443693
162.5	0.739837398	166.5	0.666666667	166.5	1	46	12.74754878	12.9034879	12.9034879
365	0.733727811	386.5	0.666666667	386.5	1	2	19.10497317	19.65960325	19.65960325
289	0.733727811	306.5	0.666666667	306.5	1	6	17	17.5071414	17.5071414
229	0.733727811	242.5	0.666666667	242.5	1	10	15.13274595	15.5724115	15.5724115
185	0.733727811	194.5	0.666666667	194.5	1	14	13.60147051	13.94632568	13.94632568
157	0.733727811	162.5	0.666666667	162.5	1	18	12.52996409	12.74754878	12.74754878
145	0.771929825	146.5	0.666666667	146.5	1	22	12.04159458	12.10371844	12.10371844
323.5	0.733727811	343.5	0.666666667	343.5	1	26	17.98610575	18.53375299	18.53375299
253.5	0.733727811	269.5	0.666666667	269.5	1	30	15.92168333	16.41645516	16.41645516
199.5	0.733727811	211.5	0.666666667	211.5	1	34	14.12444689	14.54303957	14.54303957
161.5	0.733727811	169.5	0.666666667	169.5	1	38	12.70826503	13.01921657	13.01921657
139.5	0.75	143.5	0.666666667	143.5	1	42	11.81101181	11.97914855	11.97914855
323	0.733727811	133.5	0.666666667	133.5	1	46	17.97220076	11.55422001	11.55422001
221	0.733727811	235.5	0.666666667	235.5	1	2	14.86606875	15.34600925	15.34600925
173	0.733727811	183.5	0.666666667	183.5	1	6	13.15294644	13.54621718	13.54621718
141	0.733727811	147.5	0.666666667	147.5	1	10	11.87434209	12.1449578	12.1449578
125	0.771929825	127.5	0.666666667	127.5	1	14	11.18033989	11.29158979	11.29158979
266.5	0.733727811	284.5	0.666666667	284.5	1	18	16.32482772	16.86712779	16.86712779
204.5	0.733727811	218.5	0.666666667	218.5	1	22	14.30034965	14.7817455	14.7817455
158.5	0.733727811	168.5	0.666666667	168.5	1	26	12.58967831	12.98075499	12.98075499
128.5	0.739837398	134.5	0.666666667	134.5	1	30	11.33578405	11.5974135	11.5974135
114.5	0.783783784	116.5	0.666666667	116.5	1	34	10.70046728	10.79351657	10.79351657
217	0.733727811	232.5	0.666666667	232.5	1	38	14.73091986	15.24795068	15.24795068
165	0.733727811	176.5	0.666666667	176.5	1	42	12.84523258	13.28533026	13.28533026
129	0.733727811	136.5	0.666666667	136.5	1	46	11.35781669	11.68332145	11.68332145
105	0.796296296	106.5	0.666666667	106.5	1	2	10.24695077	10.31988372	10.31988372
187.5	0.733727811	201.5	0.666666667	201.5	1	6	13.69306394	14.19506957	14.19506957
141.5	0.733727811	151.5	0.666666667	151.5	1	10	11.89537725	12.30853363	12.30853363
111.5	0.75	117.5	0.666666667	117.5	1	14	10.55935604	10.83974169	10.83974169
97.5	0.796296296	99.5	0.666666667	99.5	1	18	9.874208829	9.974968672	9.974968672
161	0.733727811	173.5	0.666666667	173.5	1	22	12.68857754	13.17193987	13.17193987
121	0.733727811	129.5	0.666666667	129.5	1	26	11	11.37980668	11.37980668
97	0.771929825	101.5	0.666666667	101.5	1	30	9.848857802	10.07472084	10.07472084
89	0.823529412	89.5	0.666666667	89.5	1	34	9.433981132	9.460443964	9.460443964
127.5	0.733727811	137.5	0.666666667	137.5	1	38	11.29158979	11.7260394	11.7260394
97.5	0.760683761	103.5	0.666666667	103.5	1	42	9.874208829	10.17349497	10.17349497
83.5	0.80952381	85.5	0.666666667	85.5	1	46	9.137833441	9.246621004	9.246621004
101	0.75	108.5	0.666666667	108.5	1	2	10.04987562	10.41633333	10.41633333
81	0.796296296	84.5	0.666666667	84.5	1	6	9	9.192388155	9.192388155
116.5	0.733727811	76.5	0.666666667	76.5	1	10	10.79351657	8.746427842	8.746427842
86.5	0.771929825	92.5	0.666666667	92.5	1	14	9.300537619	9.617692031	9.617692031
72.5	0.823529412	74.5	0.666666667	74.5	1	18	8.514693183	8.631338251	8.631338251
85	0.771929825	91.5	0.666666667	91.5	1	22	9.219544457	9.565563235	9.565563235
69	0.823529412	71.5	0.666666667	71.5	1	26	8.306623863	8.455767263	8.455767263
78.5	0.783783784	84.5	0.666666667	84.5	1	30	8.860022573	9.192388155	9.192388155
64.5	0.838383838	66.5	0.666666667	66.5	1	34	8.031189202	8.154753215	8.154753215
65	0.823529412	68.5	0.666666667	68.5	1	38	8.062257748	8.276472679	8.276472679
64.5	0.823529412	60.5	0.666666667	60.5	1	42	8.031189202	7.778174593	7.778174593
59	0.854166667	58.5	0.666666667	58.5	1	46	7.681145748	7.64852927	7.64852927
386	0.733727811	408.5	0.666666667	408.5	1	2	19.6468827	20.21138293	20.21138293
306	0.733727811	324.5	0.666666667	324.5	1	6	17.49285568	18.01388353	18.01388353
242	0.733727811	256.5	0.666666667	256.5	1	10	15.55634919	16.01561738	16.01561738
194	0.733727811	204.5	0.666666667	204.5	1	14	13.92838828	14.30034965	14.30034965
162	0.733727811	168.5	0.666666667	168.5	1	18	12.72792206	12.98075499	12.98075499
146	0.760683761	148.5	0.666666667	148.5	1	22	12.08304597	12.18605761	12.18605761
363.5	0.733727811	385.5	0.666666667	385.5	1	26	19.06567596	19.63415392	19.63415392
285.5	0.733727811	303.5	0.666666667	303.5	1	30	16.89674525	17.42125139	17.42125139
223.5	0.733727811	237.5	0.666666667	237.5	1	34	14.94991639	15.41103501	15.41103501
177.5	0.733727811	187.5	0.666666667	187.5	1	38	13.32291259	13.69306394	13.69306394
147.5	0.733727811	153.5	0.666666667	153.5	1	42	12.1449578	12.38951169	12.38951169
133.5	0.771929825	135.5	0.666666667	135.5	1	46	11.55422001	11.64044673	11.64044673
266	0.733727811	283.5	0.666666667	283.5	1	2	16.30950643	16.83745824	16.83745824
206	0.733727811	219.5	0.666666667	219.5	1	6	14.35270009	14.81553239	14.81553239
162	0.733727811	171.5	0.666666667	171.5	1	10	12.72792206	13.09580085	13.09580085
134	0.739837398	139.5	0.666666667	139.5	1	14	11.5758369	11.81101181	11.81101181
122	0.783783784	123.5	0.666666667	123.5	1	18	11.04536102	11.11305539	11.11305539
264.5	0.733727811	282.5	0.666666667	282.5	1	22	16.26345597	16.80773631	16.80773631
202.5	0.733727811	216.5	0.666666667	216.5	1	26	14.23024947	14.71393897	14.71393897
156.5	0.733727811	166.5	0.666666667	166.5	1	30	12.509996	12.9034879	12.9034879
126.5	0.739837398	132.5	0.666666667	132.5	1	34	11.24722188	11.51086443	11.51086443
112.5	0.783783784	114.5	0.666666667	114.5	1	38	10.60660172	10.70046728	10.70046728
230	0.733727811	246.5	0.666666667	246.5	1	42	15.16575089	15.70031847	15.70031847
174	0.733727811	186.5	0.666666667	186.5	1	46	13.19090596	13.65650028	13.65650028
120	0.739837398	126.5	0.666666667	126.5	1	2	10.95445115	11.24722188	11.24722188
104	0.783783784	106.5	0.666666667	106.5	1	6	10.19803903	10.31988372	10.31988372
213.5	0.733727811	229.5	0.666666667	229.5	1	10	14.6116392	15.14925741	15.14925741
159.5	0.733727811	171.5	0.666666667	171.5	1	14	12.62933094	13.09580085	13.09580085
121.5	0.733727811	129.5	0.666666667	129.5	1	18	11.02270384	11.37980668	11.37980668
99.5	0.771929825	103.5	0.666666667	103.5	1	22	9.974968672	10.17349497	10.17349497
198	0.733727811	93.5	0.666666667	93.5	1	26	14.07124728	9.669539803	9.669539803
146	0.733727811	157.5	0.666666667	157.5	1	30	12.08304597	12.5499004	12.5499004
110	0.739837398	117.5	0.666666667	117.5	1	34	10.48808848	10.83974169	10.83974169
90	0.783783784	93.5	0.666666667	93.5	1	38	9.486832981	9.669539803	9.669539803
169.5	0.733727811	85.5	0.666666667	85.5	1	42	13.01921657	9.246621004	9.246621004
123.5	0.733727811	133.5	0.666666667	133.5	1	46	11.11305539	11.55422001	11.55422001
84.5	0.783783784	88.5	0.666666667	88.5	1	2	9.192388155	9.407443861	9.407443861
144	0.733727811	78.5	0.666666667	78.5	1	6	12	8.860022573	8.860022573
104	0.739837398	112.5	0.666666667	112.5	1	10	10.19803903	10.60660172	10.60660172
80	0.783783784	84.5	0.666666667	84.5	1	14	8.94427191	9.192388155	9.192388155
72	0.838383838	72.5	0.666666667	72.5	1	18	8.485281374	8.514693183	8.514693183
94.5	0.75	102.5	0.666666667	102.5	1	22	9.721111048	10.12422837	10.12422837
72.5	0.796296296	76.5	0.666666667	76.5	1	26	8.514693183	8.746427842	8.746427842
102	0.739837398	66.5	0.666666667	66.5	1	30	10.09950494	8.154753215	8.154753215
74	0.783783784	79.5	0.666666667	79.5	1	34	8.602325267	8.91627725	8.91627725
62	0.838383838	63.5	0.666666667	63.5	1	38	7.874007874	7.968688725	7.968688725
72.5	0.783783784	78.5	0.666666667	78.5	1	42	8.514693183	8.860022573	8.860022573
58.5	0.838383838	60.5	0.666666667	60.5	1	46	7.64852927	7.778174593	7.778174593
56	0.838383838	58.5	0.666666667	58.5	1	2	7.483314774	7.64852927	7.64852927
57.5	0.823529412	61.5	0.666666667	61.5	1	6	7.582875444	7.842193571	7.842193571
54	0.838383838	51.5	0.666666667	51.5	1	10	7.348469228	7.176350047	7.176350047
49.5	0.870967742	49.5	0.666666667	49.5	1	14	7.03562364	7.03562364	7.03562364
341.5	0.733727811	363	0.666666667	363	1	18	18.47971861	19.05255888	19.05255888
265.5	0.733727811	283	0.666666667	283	1	22	16.29417074	16.82260384	16.82260384
205.5	0.733727811	219	0.666666667	219	1	26	14.33527119	14.79864859	14.79864859
161.5	0.733727811	171	0.666666667	171	1	30	12.70826503	13.07669683	13.07669683
133.5	0.739837398	139	0.666666667	139	1	34	11.55422001	11.78982612	11.78982612
121.5	0.783783784	123	0.666666667	123	1	38	11.02270384	11.09053651	11.09053651
281.5	0.733727811	300.5	0.666666667	300.5	1	42	16.77796174	17.33493582	17.33493582
215.5	0.733727811	230.5	0.666666667	230.5	1	46	14.67991826	15.18222645	15.18222645
146.5	0.733727811	155.5	0.666666667	155.5	1	2	12.10371844	12.46996391	12.46996391
120.5	0.75	125.5	0.666666667	125.5	1	6	10.9772492	11.20267825	11.20267825
110.5	0.796296296	111.5	0.666666667	111.5	1	10	10.51189802	10.55935604	10.55935604
228.5	0.733727811	245	0.666666667	245	1	14	15.11621646	15.65247584	15.65247584
172.5	0.733727811	185	0.666666667	185	1	18	13.13392554	13.60147051	13.60147051
132.5	0.733727811	141	0.666666667	141	1	22	11.51086443	11.87434209	11.87434209
108.5	0.760683761	113	0.666666667	113	1	26	10.41633333	10.63014581	10.63014581
100.5	0.80952381	101	0.666666667	101	1	30	10.02496883	10.04987562	10.04987562
196.5	0.733727811	211.5	0.666666667	211.5	1	34	14.01784577	14.54303957	14.54303957
146.5	0.733727811	157.5	0.666666667	157.5	1	38	12.10371844	12.5499004	12.5499004
112.5	0.739837398	119.5	0.666666667	119.5	1	42	10.60660172	10.93160555	10.93160555
94.5	0.783783784	97.5	0.666666667	97.5	1	46	9.721111048	9.874208829	9.874208829
167.5	0.733727811	181	0.666666667	181	1	2	12.94217911	13.45362405	13.45362405
123.5	0.733727811	133	0.666666667	133	1	6	11.11305539	11.53256259	11.53256259
95.5	0.760683761	101	0.666666667	101	1	10	9.772410143	10.04987562	10.04987562
83.5	0.80952381	85	0.666666667	85	1	14	9.137833441	9.219544457	9.219544457
153.5	0.733727811	166.5	0.666666667	166.5	1	18	12.38951169	12.9034879	12.9034879
111.5	0.733727811	120.5	0.666666667	120.5	1	22	10.55935604	10.9772492	10.9772492
85.5	0.771929825	90.5	0.666666667	90.5	1	26	9.246621004	9.513148795	9.513148795
75.5	0.823529412	76.5	0.666666667	76.5	1	30	8.689073598	8.746427842	8.746427842
118.5	0.733727811	129	0.666666667	129	1	34	10.88577053	11.35781669	11.35781669
86.5	0.760683761	93	0.666666667	93	1	38	9.300537619	9.643650761	9.643650761
70.5	0.80952381	73	0.666666667	73	1	42	8.396427812	8.544003745	8.544003745
117.5	0.733727811	128.5	0.666666667	128.5	1	46	10.83974169	11.33578405	11.33578405
72.5	0.783783784	77.5	0.666666667	77.5	1	2	8.514693183	8.803408431	8.803408431
62.5	0.838383838	63.5	0.666666667	63.5	1	6	7.90569415	7.968688725	7.968688725
81.5	0.760683761	89	0.666666667	89	1	10	9.027735043	9.433981132	9.433981132
61.5	0.80952381	65	0.666666667	65	1	14	7.842193571	8.062257748	8.062257748
88.5	0.75	57	0.666666667	57	1	18	9.407443861	7.549834435	7.549834435
62.5	0.796296296	67.5	0.666666667	67.5	1	22	7.90569415	8.215838363	8.215838363
52.5	0.854166667	53.5	0.666666667	53.5	1	26	7.245688373	7.314369419	7.314369419
56.5	0.80952381	61	0.666666667	61	1	30	7.516648189	7.810249676	7.810249676
48.5	0.870967742	49	0.666666667	49	1	34	6.964194139	7	7
48.5	0.838383838	51.5	0.666666667	51.5	1	38	6.964194139	7.176350047	7.176350047
47.5	0.838383838	51	0.666666667	51	1	42	6.892024376	7.141428429	7.141428429
44.5	0.854166667	43	0.666666667	43	1	46	6.670832032	6.557438524	6.557438524
280.5	0.733727811	300	0.666666667	300	1	2	16.74813422	17.32050808	17.32050808
212.5	0.733727811	228	0.666666667	228	1	6	14.57737974	15.09966887	15.09966887
160.5	0.733727811	172	0.666666667	172	1	10	12.66885946	13.11487705	13.11487705
124.5	0.733727811	132	0.666666667	132	1	14	11.1579568	11.48912529	11.48912529
104.5	0.771929825	108	0.666666667	108	1	18	10.22252415	10.39230485	10.39230485
261.5	0.733727811	100	0.666666667	100	1	22	16.17096163	10	10
195.5	0.733727811	210.5	0.666666667	210.5	1	26	13.98213145	14.50861813	14.50861813
145.5	0.733727811	156.5	0.666666667	156.5	1	30	12.06233808	12.509996	12.509996
111.5	0.739837398	118.5	0.666666667	118.5	1	34	10.55935604	10.88577053	10.88577053
93.5	0.783783784	96.5	0.666666667	96.5	1	38	9.669539803	9.823441352	9.823441352
209.5	0.733727811	226	0.666666667	226	1	42	14.47411483	15.03329638	15.03329638
153.5	0.733727811	166	0.666666667	166	1	46	12.38951169	12.88409873	12.88409873
99.5	0.75	106	0.666666667	106	1	2	9.974968672	10.29563014	10.29563014
83.5	0.796296296	89.5	0.666666667	89.5	1	6	9.137833441	9.460443964	9.460443964
178.5	0.733727811	81.5	0.666666667	81.5	1	10	13.36038922	9.027735043	9.027735043
128.5	0.733727811	151.5	0.666666667	151.5	1	14	11.33578405	12.30853363	12.30853363
94.5	0.75	109.5	0.666666667	109.5	1	18	9.721111048	10.46422477	10.46422477
76.5	0.796296296	83.5	0.666666667	83.5	1	22	8.746427842	9.137833441	9.137833441
150.5	0.733727811	73.5	0.666666667	73.5	1	26	12.26784415	8.5732141	8.5732141
106.5	0.733727811	126.5	0.666666667	126.5	1	30	10.31988372	11.24722188	11.24722188
78.5	0.771929825	90.5	0.666666667	90.5	1	34	8.860022573	9.513148795	9.513148795
66.5	0.823529412	70.5	0.666666667	70.5	1	38	8.154753215	8.396427812	8.396427812
114.5	0.733727811	137.5	0.666666667	137.5	1	42	10.70046728	11.7260394	11.7260394
80.5	0.760683761	95.5	0.666666667	95.5	1	46	8.972179222	9.772410143	9.772410143
59.5	0.838383838	62.5	0.666666667	62.5	1	2	7.71362431	7.90569415	7.90569415
85.5	0.75	103.5	0.666666667	103.5	1	6	9.246621004	10.17349497	10.17349497
61.5	0.796296296	71.5	0.666666667	71.5	1	10	7.842193571	8.455767263	8.455767263
53.5	0.854166667	55.5	0.666666667	55.5	1	14	7.314369419	7.449832213	7.449832213
69.5	0.771929825	84.5	0.666666667	84.5	1	18	8.336666	9.192388155	9.192388155
51.5	0.823529412	58.5	0.666666667	58.5	1	22	7.176350047	7.64852927	7.64852927
68.5	0.771929825	48.5	0.666666667	48.5	1	26	8.276472679	6.964194139	6.964194139
48.5	0.823529412	56.5	0.666666667	56.5	1	30	6.964194139	7.516648189	7.516648189
61.5	0.783783784	44.5	0.666666667	44.5	1	34	7.842193571	6.670832032	6.670832032
43.5	0.838383838	50.5	0.666666667	50.5	1	38	6.595452979	7.106335202	7.106335202
45.5	0.823529412	40.5	0.666666667	40.5	1	42	6.745368782	6.363961031	6.363961031
37.5	0.888888889	39.5	0.666666667	39.5	1	46	6.123724357	6.284902545	6.284902545
34.5	0.888888889	35.5	0.666666667	35.5	1	2	5.873670062	5.958187644	5.958187644
225.5	0.733727811	33.5	0.666666667	33.5	1	6	15.01665742	5.787918451	5.787918451
165.5	0.733727811	193.5	0.666666667	193.5	1	10	12.86468033	13.91042774	13.91042774
121.5	0.733727811	141.5	0.666666667	141.5	1	14	11.02270384	11.89537725	11.89537725
93.5	0.760683761	105.5	0.666666667	105.5	1	18	9.669539803	10.27131929	10.27131929
81.5	0.80952381	85.5	0.666666667	85.5	1	22	9.027735043	9.246621004	9.246621004
177.5	0.733727811	208.5	0.666666667	208.5	1	26	13.32291259	14.43952908	14.43952908
127.5	0.733727811	150.5	0.666666667	150.5	1	30	11.29158979	12.26784415	12.26784415
93.5	0.75	108.5	0.666666667	108.5	1	34	9.669539803	10.41633333	10.41633333
75.5	0.796296296	82.5	0.666666667	82.5	1	38	8.689073598	9.082951062	9.082951062
162.5	0.733727811	72.5	0.666666667	72.5	1	42	12.74754878	8.514693183	8.514693183
114.5	0.733727811	136.5	0.666666667	136.5	1	46	10.70046728	11.68332145	11.68332145
72.5	0.783783784	82.5	0.666666667	82.5	1	2	8.514693183	9.082951062	9.082951062
64.5	0.838383838	66.5	0.666666667	66.5	1	6	8.031189202	8.154753215	8.154753215
112.5	0.733727811	135.5	0.666666667	135.5	1	10	10.60660172	11.64044673	11.64044673
78.5	0.760683761	93.5	0.666666667	93.5	1	14	8.860022573	9.669539803	9.669539803
60.5	0.80952381	67.5	0.666666667	67.5	1	18	7.778174593	8.215838363	8.215838363
111.5	0.733727811	57.5	0.666666667	57.5	1	22	10.55935604	7.582875444	7.582875444
75.5	0.760683761	91.5	0.666666667	91.5	1	26	8.689073598	9.565563235	9.565563235
55.5	0.80952381	63.5	0.666666667	63.5	1	30	7.449832213	7.968688725	7.968688725
100.5	0.733727811	51.5	0.666666667	51.5	1	34	10.02496883	7.176350047	7.176350047
66.5	0.771929825	81.5	0.666666667	81.5	1	38	8.154753215	9.027735043	9.027735043
48.5	0.823529412	55.5	0.666666667	55.5	1	42	6.964194139	7.449832213	7.449832213
72.5	0.760683761	45.5	0.666666667	45.5	1	46	8.514693183	6.745368782	6.745368782
42.5	0.838383838	48.5	0.666666667	48.5	1	2	6.519202405	6.964194139	6.964194139
57.5	0.783783784	40.5	0.666666667	40.5	1	6	7.582875444	6.363961031	6.363961031
39.5	0.838383838	46.5	0.666666667	46.5	1	10	6.284902545	6.819090848	6.819090848
45.5	0.80952381	36.5	0.666666667	36.5	1	14	6.745368782	6.041522987	6.041522987
33.5	0.870967742	37.5	0.666666667	37.5	1	18	5.787918451	6.123724357	6.123724357
33.5	0.854166667	40.5	0.666666667	40.5	1	22	5.787918451	6.363961031	6.363961031
30.5	0.870967742	30.5	0.666666667	30.5	1	26	5.522680509	5.522680509	5.522680509
27.5	0.908045977	28.5	0.666666667	28.5	1	30	5.244044241	5.338539126	5.338539126
162	0.733727811	192	0.666666667	192	1	34	12.72792206	13.85640646	13.85640646
114	0.733727811	136	0.666666667	136	1	38	10.67707825	11.66190379	11.66190379
82	0.760683761	96	0.666666667	96	1	42	9.055385138	9.797958971	9.797958971
66	0.80952381	72	0.666666667	72	1	46	8.124038405	8.485281374	8.485281374
122.5	0.733727811	147.5	0.666666667	147.5	1	2	11.06797181	12.1449578	12.1449578
84.5	0.75	101.5	0.666666667	101.5	1	6	9.192388155	10.07472084	10.07472084
62.5	0.796296296	71.5	0.666666667	71.5	1	10	7.90569415	8.455767263	8.455767263
134	0.733727811	57.5	0.666666667	57.5	1	14	11.5758369	7.582875444	7.582875444
90	0.739837398	110	0.666666667	110	1	18	9.486832981	10.48808848	10.48808848
62	0.783783784	74	0.666666667	74	1	22	7.874007874	8.602325267	8.602325267
50	0.838383838	54	0.666666667	54	1	26	7.071067812	7.348469228	7.348469228
88.5	0.739837398	109.5	0.666666667	109.5	1	30	9.407443861	10.46422477	10.46422477
58.5	0.783783784	71.5	0.666666667	71.5	1	34	7.64852927	8.455767263	8.455767263
44.5	0.838383838	49.5	0.666666667	49.5	1	38	6.670832032	7.03562364	7.03562364
70	0.760683761	88	0.666666667	88	1	42	8.366600265	9.38083152	9.38083152
46	0.80952381	56	0.666666667	56	1	46	6.782329983	7.483314774	7.483314774
61.5	0.771929825	38	0.666666667	38	1	2	7.842193571	6.164414003	6.164414003
39.5	0.823529412	48.5	0.666666667	48.5	1	6	6.284902545	6.964194139	6.964194139
54	0.783783784	34.5	0.666666667	34.5	1	10	7.348469228	5.873670062	5.873670062
34	0.838383838	42	0.666666667	42	1	14	5.830951895	6.480740698	6.480740698
41.5	0.80952381	30	0.666666667	30	1	18	6.442049363	5.477225575	5.477225575
27.5	0.870967742	32.5	0.666666667	32.5	1	22	5.244044241	5.700877125	5.700877125
26	0.870967742	32	0.666666667	32	1	26	5.099019514	5.656854249	5.656854249
23.5	0.888888889	24	0.666666667	24	1	30	4.847679857	4.898979486	4.898979486
147	0.733727811	22	0.666666667	22	1	34	12.12435565	4.69041576	4.69041576
99	0.733727811	121	0.666666667	121	1	38	9.949874371	11	11
67	0.771929825	81	0.666666667	81	1	42	8.185352772	9	9
51	0.823529412	57	0.666666667	57	1	46	7.141428429	7.549834435	7.549834435
87.5	0.739837398	108.5	0.666666667	108.5	1	2	9.354143467	10.41633333	10.41633333
57.5	0.783783784	70.5	0.666666667	70.5	1	6	7.582875444	8.396427812	8.396427812
43.5	0.838383838	48.5	0.666666667	48.5	1	10	6.595452979	6.964194139	6.964194139
77	0.75	97	0.666666667	97	1	14	8.774964387	9.848857802	9.848857802
49	0.796296296	61	0.666666667	61	1	18	7	7.810249676	7.810249676
37	0.854166667	41	0.666666667	41	1	22	6.08276253	6.403124237	6.403124237
59.5	0.771929825	76.5	0.666666667	76.5	1	26	7.71362431	8.746427842	8.746427842
37.5	0.823529412	46.5	0.666666667	46.5	1	30	6.123724357	6.819090848	6.819090848
59	0.771929825	32.5	0.666666667	32.5	1	34	7.681145748	5.700877125	5.700877125
35	0.823529412	45	0.666666667	45	1	38	5.916079783	6.708203932	6.708203932
27	0.888888889	29	0.666666667	29	1	42	5.196152423	5.385164807	5.385164807
29.5	0.838383838	38.5	0.666666667	38.5	1	46	5.431390246	6.204836823	6.204836823
25	0.854166667	33	0.666666667	33	1	2	5	5.744562647	5.744562647
24.5	0.854166667	21	0.666666667	21	1	6	4.949747468	4.582575695	4.582575695
19	0.888888889	19.5	0.666666667	19.5	1	10	4.358898944	4.415880433	4.415880433
108	0.733727811	17	0.666666667	17	1	14	10.39230485	4.123105626	4.123105626
68	0.760683761	86	0.666666667	86	1	18	8.246211251	9.273618495	9.273618495
44	0.80952381	54	0.666666667	54	1	22	6.633249581	7.348469228	7.348469228
36	0.870967742	38	0.666666667	38	1	26	6	6.164414003	6.164414003
58.5	0.771929825	75.5	0.666666667	75.5	1	30	7.64852927	8.689073598	8.689073598
36.5	0.823529412	45.5	0.666666667	45.5	1	34	6.041522987	6.745368782	6.745368782
66	0.760683761	31.5	0.666666667	31.5	1	38	8.124038405	5.61248608	5.61248608
38	0.80952381	50	0.666666667	50	1	42	6.164414003	7.071067812	7.071067812
26	0.870967742	30	0.666666667	30	1	46	5.099019514	5.477225575	5.477225575
27.5	0.838383838	36.5	0.666666667	36.5	1	2	5.244044241	6.041522987	6.041522987
36	0.80952381	22.5	0.666666667	22.5	1	6	6	4.74341649	4.74341649
20	0.870967742	26	0.666666667	26	1	10	4.472135955	5.099019514	5.099019514
21.5	0.854166667	18	0.666666667	18	1	14	4.636809248	4.242640687	4.242640687
18	0.870967742	16.5	0.666666667	16.5	1	18	4.242640687	4.062019202	4.062019202
13.5	0.908045977	14	0.666666667	14	1	22	3.674234614	3.741657387	3.741657387
65.5	0.760683761	12	0.666666667	12	1	26	8.093207028	3.464101615	3.464101615
37.5	0.80952381	49.5	0.666666667	49.5	1	30	6.123724357	7.03562364	7.03562364
25.5	0.870967742	29.5	0.666666667	29.5	1	34	5.049752469	5.431390246	5.431390246
41.5	0.796296296	56.5	0.666666667	56.5	1	38	6.442049363	7.516648189	7.516648189
23.5	0.854166667	30.5	0.666666667	30.5	1	42	4.847679857	5.522680509	5.522680509
34.5	0.80952381	20.5	0.666666667	20.5	1	46	5.873670062	4.527692569	4.527692569
16.5	0.908045977	18.5	0.666666667	18.5	1	2	4.062019202	4.301162634	4.301162634
16.5	0.870967742	23.5	0.666666667	23.5	1	6	4.062019202	4.847679857	4.847679857
15.5	0.870967742	13.5	0.666666667	13.5	1	10	3.937003937	3.674234614	3.674234614
12.5	0.888888889	11.5	0.666666667	11.5	1	14	3.535533906	3.391164992	3.391164992
8.5	0.950617284	9.5	0.666666667	9.5	1	18	2.915475947	3.082207001	3.082207001
28.5	0.823529412	40.5	0.666666667	40.5	1	22	5.338539126	6.363961031	6.363961031
16.5	0.888888889	20.5	0.666666667	20.5	1	26	4.062019202	4.527692569	4.527692569
22.5	0.838383838	33.5	0.666666667	33.5	1	30	4.74341649	5.787918451	5.787918451
12.5	0.908045977	15.5	0.666666667	15.5	1	34	3.535533906	3.937003937	3.937003937
11.5	0.888888889	17.5	0.666666667	17.5	1	38	3.391164992	4.183300133	4.183300133
10.5	0.888888889	9.5	0.666666667	9.5	1	42	3.240370349	3.082207001	3.082207001
6.5	0.928571429	7.5	0.666666667	7.5	1	46	2.549509757	2.738612788	2.738612788
13.5	0.870967742	21.5	0.666666667	21.5	1	2	3.674234614	4.636809248	4.636809248
16.5	0.854166667	9.5	0.666666667	9.5	1	6	4.062019202	3.082207001	3.082207001
6.5	0.928571429	9.5	0.666666667	9.5	1	10	2.549509757	3.082207001	3.082207001
4.5	0.950617284	6.5	0.666666667	6.5	1	14	2.121320344	2.549509757	2.549509757
12	0.870967742	3.5	0.666666667	3.5	1	18	3.464101615	1.870828693	1.870828693
4	0.950617284	6	0.666666667	6	1	22	2	2.449489743	2.449489743
2	0.950617284	3.5	0.666666667	3.5	1	26	1.414213562	1.870828693	1.870828693
1	0.974358974	3	0.666666667	3	1	30	1	1.732050808	1.732050808
1	0.974358974	1	0.666666667	1	1	34	1	1	1
0	1	0	0.666666667	0	1	35	0	0	0


==> Figs/DoFV_Data_2.tex <==
UCY	MCY	UCXSD	MCXSD
0.667	1	0	0
0.667	1	2	2
0.667	1	4	4
0.667	1	6	6
0.667	1	8	8
0.667	1	10	10
0.667	1	12	12
0.667	1	14	14
0.667	1	16	16
0.667	1	18	18
0.667	1	20	20
0.667	1	22	22
0.667	1	24	24
0.667	1	26	26
0.667	1	28	28
0.667	1	30	30
0.667	1	32	32
0.667	1	34	34
0.667	1	36	36
0.667	1	38	38
0.667	1	40	40
0.667	1	42	42


==> OldIntro.tex <==
Wireless networks are under continuous pressure to support increasing volumes of multimedia content~\cite{cisco2018cisco} and pave the way for the emergence of new applications such as wireless immersive viewing~\cite{mahmoodi2021non}. For the efficient delivery of such multimedia content, Maddah-Ali and Niesen proposed the idea of \emph{coded caching} for increasing the data rates by exploiting cache content across the network~\cite{maddah2014fundamental}. In a single-stream downlink network,
%of cache-enabled users,
%who can pre-fetch data into their cache memories, 
coded caching enables boosting the achievable rate by a multiplicative factor proportional to the cumulative cache size in the entire network. This speedup is achieved through
%The key to achieving this speedup lies in the 
multicasting of carefully created codewords to different groups of users, such that each user can use its cache content to remove unwanted parts 
%(i.e., the interference) 
from the received signal.
%
Motivated by the growing importance of multi-antenna communications~\cite{rajatheva2020white}, cache-aided \ac{MISO} setting was later explored in~\cite{shariatpanahi2016multi,shariatpanahi2018physical}, where it was revealed that the same coded caching gain could be achieved together with the spatial multiplexing gain. 
This cumulative gain was then shown in~\cite{lampiris2018resolving} to be optimal with the underlying assumptions of uncoded cache placement and one-shot linear data delivery.
%Of course, an even larger cache-aided \ac{DoF} can be achieved for the same setup using interference-alignment techniques such as in~\cite{naderializadeh2017fundamental}. However, such techniques are overly complex to implement in practice (cf.~\cite{maddah2014fundamental}), and hence, in this paper, we also aim at maximizing the \ac{DoF} with the underlying assumptions of uncoded cache placement and one-shot linear data delivery.

Following the introduction of \ac{MISO} coded caching, many later works in the literature addressed its important scaling and performance issues. Notably, in~\cite{tolli2017multi}, the authors showed that using optimized beamformers instead of zero-forcing, one could achieve a better rate for communications at the finite-SNR regime. %Also in the same paper, two interesting methods for adjusting the spatial \ac{DoF} and controlling the \ac{MAC} size were introduced for managing the optimized beamformer design complexity. 
Similarly, the exponentially growing subpacketization issue (i.e., the number of smaller parts each file should be split into) was addressed thoroughly in the literature.
Interestingly, while reducing subpacketization is challenging in single-antenna setups~\cite{yan2018placement},  
%
%for both single-antenna (cf.~\cite{yan2018placement,yan2017placement}) and multi-antenna 
%(cf.\cite{lampiris2018adding,salehi2020lowcomplexity,mohajer2020miso})
%setups. Most notably, for multi-antenna \ac{MISO} setups 
%and it was shown in~\cite{lampiris2018adding,salehi2020lowcomplexity}, 
\ac{MISO} setups allow reducing the subpacketization substantially without affecting the maximum achievable \ac{DoF}~\cite{lampiris2018adding}. %that one could substantially reduce the subpacketization requirement while achieving the same maximum \ac{DoF} value. 
Of course, this reduced subpacketization modestly decreases the achievable rate, especially at the finite-SNR regime~\cite{salehi2019subpacketization}. Nevertheless, it does not harm the achievable \ac{DoF} and yet enables a much simpler optimized beamformer design~\cite{salehi2020lowcomplexity}.

% -------------------------------------------------- %

There exists another critical obstacle preventing the practical implementation of coded caching schemes, especially in dynamic network setups. All the schemes mentioned so far are centralized, i.e., the cache contents of the users are dictated by a central server. However, the server needs prior knowledge of the number of users to indicate what data should be cached at each user during the placement phase. This makes it impossible to implement caching techniques in dynamic networks where the users are allowed to join/leave the network at any moment. One possible solution to this issue is to use fully decentralized schemes, such as~\cite{maddah2015decentralized}, where the cache contents of each user are assumed to be fully random and codewords are built to achieve the caching gain to the maximum possible extent. Unfortunately, the caching gain of such decentralized solutions is comparable with centralized schemes only asymptotically, i.e., when the number of users (or the size of each file) is very large. Hence, the problem remains largely unresolved for practical networks with a moderate number of users.

%Another important obstacle preventing practical implementation of coded caching schemes is their strict dependency on a well-performed cache placement phase. All the schemes mentioned so far are centralized, i.e., the cache contents of the users are dictated by a central server. Moreover, it is assumed that these contents are fully cached before the requests are revealed in the subsequent delivery phase. This makes it impossible to implement caching techniques in dynamic networks where the users are free to join/leave the network at any moment. One possible solution to this issue is to use fully decentralized schemes, such as~\cite{maddah2015decentralized}, where the cache contents of each user are assumed to be fully random, and codewords are built to achieve the caching gain to the maximum possible extent. Although decentralized schemes resolve the issue of dependency on a well-performed placement phase, they provide promising gains only asymptotically, i.e., when the number of users (or the size of each file) is very large. Hence, the problem remains largely unresolved for practical networks with a moderate number of users.

In this paper, we take a different approach to this problem by introducing a hybrid centralized/decentralized coded caching scheme. In this scheme, 
instead of defining cache contents for each user individually, the server assigns users with a limited set of \emph{caching profiles} that indicate the contents that should be cached at every assigned user.
%the cache contents of users are still dictated by a central server, but the users can join/leave the network at any time. Each user is assigned with a \emph{caching profile} that indicates which contents should be cached at its memory. 
Multiple users may be assigned with the same profile and cache the same contents, 
resulting in a shared-cache setup as studied in~\cite{parrinello2019fundamental}.
%making the resulting setup similar to shared-cache models where multiple users have access to the same cache storage (cf.~\cite{parrinello2019fundamental}). 
However, due to the dynamic nature of the network, the \emph{length} of each profile, defined as the number of users associated with that profile, can vary during the time and be independent from the length of other profiles. Then, we introduce a new delivery algorithm, inspired by the low-subpacketization scheme in~\cite{salehi2020lowcomplexity}, for enabling a combined caching and spatial multiplexing gain, comparable to a large extent with the ideal case of fully centralized schemes. Of course, this paper is not the first one introducing such a hybrid scheme; a similar approach is introduced in~\cite{jin2019new} for single-antenna setups. However, here, we extended the results to multi-antenna setups and do so with minor subpacketization and beamforming overheads. %introduce a multi-antenna scheme which also requires very low-subpacketization.

We emphasize that, this paper does \emph{not} aim at proposing an information-theoretic \ac{DoF}-optimal scheme for dynamic networks. Instead, the goal is to provide a practical scheme with an appropriate performance at the finite-SNR regime. In this regard, we leave most of the theoretical analyses of the proposed scheme to the extended version of this paper, and use numerical simulations here to investigate how our new scheme performs in comparison with centralized schemes applied to static network setups. Nevertheless, we provide helpful insights about the underlying reasons for any observation of an improved/deteriorated performance.

In this paper, we use boldface lower- and upper-case letters to denote vectors and matrices, respectively. Sets are shown with calligraphic letters. Similar to vectors, it is assumed that the order of members in a set is important and preserved. $\BA[i,j]$ is the element at row $i$ and column $j$ of matrix $\BA$, and $\Ba[i]$ and $\CA[i]$ are the $i$-th elements of vector $\Ba$ and set $\CA$, respectively.
$[K]$ represents the set of integers $\{1,2,...,K \}$, and $\CA \backslash \CB$ denotes the elements of set $\CA$ which are not in set $\CB$. Other notations are defined as they are used in the text.
